Inverse Dynamics with Rigid Contact and Friction

Inverse dynamics is used extensively in robotics and biomechanics applications. In manipulator and legged robots, it can form the basis of an effective nonlinear control strategy by providing a robot with both accurate positional tracking and active compliance. In biomechanics applications, inverse dynamics control can approximately determine the net torques applied at anatomical joints that correspond to an observed motion. In the context of robot control, using inverse dynamics requires knowledge of all contact forces acting on the robot; accurately perceiving external forces applied to the robot requires filtering and thus significant time delay. An alternative approach has been suggested in recent literature: predicting contact and actuator forces simultaneously under the assumptions of rigid body dynamics, rigid contact, and friction. Existing such inverse dynamics approaches have used approximations to the contact models, which permits use of fast numerical linear algebra algorithms. In contrast, we describe inverse dynamics algorithms that are derived only from first principles and use established phenomenological models like Coulomb friction. We assess these inverse dynamics algorithms in a control context using two virtual robots: a locomoting quadrupedal robot and a fixed-based manipulator gripping a box while using perfectly accurate sensor data from simulation. The data collected from these experiments gives an upper bound on the performance of such controllers in situ. For points of comparison, we assess performance on the same tasks with both error feedback control and inverse dynamics control with virtual contact force sensing.

==> tcbbreakable.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcbbreakable.code.tex: Code for breakable colorboxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.94}

\let\tcb@parboxrestore@true=\tcb@parboxrestore
\let\tcb@parboxrestore@false\tcb@parbox@false@settings

% total height for boxes smaller than 0.4375\maxdimen and 0.4375\maxdimen else (ca 2.5m)
\def\tcb@defToTotalHeightBreakable#1#2{%
  \ifnum\ht#2<0 %
    \edef#1{7168pt}%
  \else\ifnum\ht#2<469762048 %
    \tcbdimto#1{\ht#2+\dp#2}%
  \else%
    \edef#1{7168pt}%
  \fi\fi%
}

\newbox\tcb@testbox

% for oversized boxes height is detected as \textheight or larger
\def\tcb@defToTotalHeightUnlimited#1#2{%
  \tcb@defToTotalHeightBreakable#1#2%
  \ifdim\dimexpr#1<\textheight\relax%
    \edef\tcb@thevfuzz{\the\vfuzz}%
    \edef\tcb@thevbadness{\the\vbadness}%
    \vfuzz=\maxdimen\vbadness=10000%
    \splittopskip=0pt%
    \splitmaxdepth=0pt%
    \savingvdiscards=1%
    \setbox\tcb@testbox=\vsplit#2 to \textheight%
    \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
    \ifdim\wd#2=0pt\relax%
      \tcb@swap{#2}{\tcb@testbox}%
      \tcbdimto#1{\ht#2+\dp#2}%
    \else%
      \setbox#2=\vbox{%
        \unvbox\tcb@testbox%
        \splitdiscards%
        \unvbox#2}%
      \edef#1{7168pt}%
    \fi%
    \savingvdiscards=0%
  \fi%
}


\def\tcb@vbox#1#2{%
  \edef\reserved@a{%
    \endgroup%
    \setbox#1\vbox{\hsize=#2%
      \begingroup\aftergroup}%
      \def\noexpand\@currenvir{\@currenvir}%
      \def\noexpand\@currenvline{\on@line}}%
  \reserved@a%
  \@endpefalse%
  \color@begingroup%
  \textwidth\hsize%
  \columnwidth\hsize%
  \csname tcb@parboxrestore@\kvtcb@parbox\endcsname%
  \def\@mpfn{mpfootnote}%
  \def\thempfn{\thempfootnote}%
  \c@mpfootnote\z@%
  \let\@footnotetext\@mpfootnotetext%
  \let\@listdepth\@mplistdepth \@mplistdepth\z@%
  \@setminipage\tcb@hyph@fix%
  \let\tcb@drawcolorbox\tcb@drawcolorbox@standalone%
  \let\FN@pp@footnote\@empty% disable perpage mode of 'footmisc' package
  \ignorespaces%
}

\def\endtcb@vbox{%
  \par%
  \unskip%
  \ifvoid\@mpfootins\else%
    \vskip\skip\@mpfootins%
    \normalcolor%
    \footnoterule%
    \unvbox\@mpfootins%
  \fi%
  \@minipagefalse%
  \color@endgroup}

% remaining height
\def\tcb@comp@h@page{%
  \tcb@breakat@next%
  \ifdim\tcb@breakat@dim>0pt\relax%
    \tcbdimto\tcb@h@page{\tcb@breakat@dim-\kvtcb@shrinkbreakgoal}%
  \else%
    \ifx\kvtcb@float\@empty%
      \iftcb@multicol%
        \tcbdimto\tcb@h@page{\textheight-\kvtcb@shrinkbreakgoal}%
      \else%
        \ifdim\pagegoal=16383.99998pt
          \tcbdimto\tcb@h@page{\vsize-\kvtcb@shrinkbreakgoal}% detects floating objects
        \else%
          \tcb@comp@compress%
          \tcbdimto\tcb@h@page{\pagegoal-\pagetotal+\tcb@compress@height-\kvtcb@shrinkbreakgoal}%
        \fi%
      \fi%
    \else%
      \tcbdimto\tcb@h@page{\textheight-\kvtcb@shrinkbreakgoal}%
    \fi%
  \fi%
}

\def\tcb@comp@h@total@standalone{%
  \tcbdimto\tcb@h@padding{\kvtcb@bbtop@stand+\kvtcb@bbbottom@stand+\kvtcb@top@rule@stand+\kvtcb@bottom@rule@stand+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@total{\tcb@h@padding+\tcb@h@padtitle+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower}%
}


\newif\iftcb@final@box

\def\tcb@check@for@final@box{%
  \ifdim\tcb@h@total>\tcb@h@page\relax%
    \iftcb@multicol%
      \tcb@final@boxfalse%
    \else%
      \ifdim\tcb@h@total>\dimexpr\tcb@h@page+\kvtcb@enlargepage@flex\relax%
        \tcb@final@boxfalse%
      \else%
        \tcbdimto\tcb@temp{\tcb@h@total-\tcb@h@page}%
        \enlargethispage*{\tcb@temp}%
        \tcbdimto\tcb@h@page{\tcb@h@page+\tcb@temp}%
        \tcb@final@boxtrue%
      \fi%
    \fi%
  \else%
    \tcb@final@boxtrue%
  \fi%
}

\def\tcb@following@title{%
  \ifx\kvtcb@followingtitle\@empty%
    \tcb@hasTitlefalse%
    \let\tcb@h@title=\tcb@zpt%
    \let\tcb@h@padtitle=\tcb@zpt%
  \else%
    \tcb@hasTitletrue%
    \tcbdimto\tcb@w@title{\tcb@innerwidth-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle}%
    \begin{tcb@savebox}{\tcb@titlebox}{\tcb@w@title}\leavevmode\color{tcbcol@title}\kvtcb@fonttitle\kvtcb@followingtitle\end{tcb@savebox}%
    \tcbdimto\tcb@h@title{\ht\tcb@titlebox+\dp\tcb@titlebox}%
    \tcbdimto\tcb@h@padtitle{\kvtcb@title@rule+\kvtcb@boxsep*2+\kvtcb@toptitle+\kvtcb@bottomtitle+\tcb@h@title}%
  \fi%
}

\newbox\tcb@totalupperbox
\newbox\tcb@totallowerbox
\newif\iftcb@break@allowed

\def\tcb@enlbreak@next@final{%
  \ifdim\dimexpr\tcb@enlbreak@dim=0pt\relax
  \else%
    \iftcb@multicol\else\enlargethispage{\tcb@enlbreak@dim}\fi%
  \fi%
}

\def\tcb@enlbreak@next@scan#1/#2@{%
  \def\temp@a{#2}%
  \tcbdimto\tcb@enlbreak@dim{#1}%
  \ifx\temp@a\@empty%
    \let\tcb@enlbreak@next=\tcb@enlbreak@next@final%
  \else%
     \edef\tcb@enlbreak@seq{\temp@a @}%
  \fi%
  \tcb@enlbreak@next@final%
}

\def\tcb@enlbreak@next@step{%
  \edef\tcb@temp{\noexpand\tcb@enlbreak@next@scan\tcb@enlbreak@seq}%
  \tcb@temp%
}

\def\tcb@enlbreak@init{%
  \edef\tcb@enlbreak@seq{\kvtcb@enlargepage/@}%
  \let\tcb@enlbreak@next=\tcb@enlbreak@next@step%
  \tcb@enlbreak@next%
}


\def\tcb@breakat@next@scan#1/#2@{%
  \def\temp@a{#2}%
  \tcbdimto\tcb@breakat@dim{#1}%
  \ifx\temp@a\@empty%
    \let\tcb@breakat@next=\@empty%
  \else%
     \edef\tcb@breakat@seq{\temp@a @}%
  \fi%
}

\def\tcb@breakat@next@step{%
  \edef\tcb@temp{\noexpand\tcb@breakat@next@scan\tcb@breakat@seq}%
  \tcb@temp%
}

\def\tcb@breakat@init{%
  \edef\tcb@breakat@seq{\kvtcb@breakatdim/@}%
  \let\tcb@breakat@next=\tcb@breakat@next@step%
}


\newif\iftcb@multicol
\newif\iftcb@vfillbeforefirst

\def\tcb@do@nobreak@warning{%
  \iftcb@ignorenobreak%
    \tcb@warning{Using nobreak failed. You should set `ignore nobreak=false' to avoid this}%
  \else%
    \tcb@warning{Using nobreak failed. Try to enlarge `lines before break' or set page breaks manually}%
  \fi%
}

\def\tcb@handle@nobreak{%
  \tcb@enlbreak@init%
  \tcb@breakat@init%
  \tcb@comp@h@page%
  \tcbdimto\tcb@h@page{\tcb@h@page-1.5\baselineskip-\parskip-\lineskip}% security surcharge
  \tcb@comp@h@total@standalone%
  \tcb@check@for@final@box%
  \iftcb@final@box%
  \else%
    \ifdim\dimexpr\tcb@h@page-\tcb@h@padding-\tcb@h@padtitle<\kvtcb@breakminlines\baselineskip\relax%
      \tcbdimto\tcb@h@page{\tcb@h@page+3.5\baselineskip+\parskip+\lineskip}%
      \vspace{\tcb@h@page}%
      {\parskip\z@\nointerlineskip\noindent}%
      \vspace{-\tcb@h@page}%
      \par%
    \fi%
  \fi%
}

\def\tcb@prepare@break@operation{%
  \setcounter{tcbbreakpart}{0}%
  \let\tcb@nobreak@warning\@empty%
  \@ifundefined{columnbreak}{\tcb@multicolfalse}{%
    \ifnum\doublecol@number>\z@ %
      \tcb@multicoltrue%
    \else%
      \tcb@multicolfalse%
    \fi}%
  \ifx\kvtcb@float\@empty%
    \iftcb@nobreak{%
      \let\tcb@nobreak@warning\tcb@do@nobreak@warning%
      \iftcb@ignorenobreak%
        \kvtcb@beforebox%
      \else%
        \tcb@handle@nobreak%
      \fi%
    }{\kvtcb@beforebox}%
    \def\kvtcb@beforebox{\parskip\z@\nointerlineskip\noindent}%
    \noindent% applies parskip
    \vskip\lineskip{\parskip\z@\par\vskip\z@}\bgroup\@nobreakfalse\addpenalty\z@\egroup% force update vertical list
    \tcb@break@allowedtrue%
    \tcb@enlbreak@init%
  \else%
    \tcb@break@allowedfalse%
  \fi%
}

\def\tcb@height@fill@unbroken#1{%
  \ifnum\c@tcblayer<2\relax%
    \tcb@ignorenobreaktrue%
    \tcb@prepare@break@operation%
    \tcb@breakat@init%
    \tcbset{compress page=#1}%
    \tcb@comp@h@page%
    \tcbset{height=\tcb@h@page-\kvtcb@bbtop@stand-\kvtcb@bbbottom@stand}%
  \fi%
}

\def\tcb@height@fill@unbroken@normal{\tcb@height@fill@unbroken{none}}
\def\tcb@height@fill@unbroken@compressed{\tcb@height@fill@unbroken{all}}

\def\tcb@use@after@lastbox{\bgroup\tcb@after@lastbox\egroup}

\def\tcb@drawcolorbox@breakable{%
  \tcb@prepare@break@operation%
  \global\let\tcb@after@lastbox=\kvtcb@afterbox%
  \let\kvtcb@afterbox=\@empty%
  \begingroup%
    \parskip\z@%
    \parindent\z@%
    \lineskip\z@%
    \topskip\z@%
    \tcb@split@start%
  \endgroup%
  \color{.}% hack for some special cases
  \ifx\kvtcb@float\@empty%
    \aftergroup\tcb@use@after@lastbox%
  \fi%
}

\def\tcb@split@pagebreak{%
  \tcb@undo@before%
  \iftcb@multicol\columnbreak\else\pagebreak\fi%
  \tcb@nobreak@warning%
  \tcb@enlbreak@init\tcb@break@allowedfalse%
}

\def\tcb@split@start{%
  \tcb@breakat@init%
  \tcb@comp@h@page%
  % height calculation
  \tcb@comp@h@total@standalone%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@drawcolorbox@standalone%
  \else%
    \iftcb@break@allowed%
      \ifdim\dimexpr\tcb@h@page-\tcb@h@padding-\tcb@h@padtitle<\kvtcb@breakminlines\baselineskip\relax%
        \tcb@split@pagebreak%
        \tcb@comp@h@page%
        \tcb@check@for@final@box%
        \iftcb@final@box%
          \tcb@drawcolorbox@standalone%
        \else%
          \let\tcb@split@next=\tcb@split@first%
        \fi%
      \else%
        \let\tcb@split@next=\tcb@split@first%
      \fi%
    \else%
      \let\tcb@split@next=\tcb@split@first%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@setbox#1#2#3{%
  \setbox#1=\vbox{\unvbox#3}%
  \ifdim\dimexpr\ht#1+\dp#1>#2\relax%
    %\tcb@warning{Splitted box part too large by \the\dimexpr\ht#1+\dp#1-#2\relax}% switched off (99% useless/annoying)
    \setbox#1=\vbox to\the\dimexpr#2-\dp#1\relax{\unvbox#1}%
  \fi%
}


\def\tcb@setbox@upper#1#2{%
  \tcb@setbox\tcb@upperbox{#1}{#2}%
  \tcbdimto\tcb@h@upper{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcb@vsplit@upper{%
  \setbox\tcb@upperbox=\vsplit\tcb@totalupperbox to\tcb@split@dim%
  \edef\tcb@upper@box@badness{\the\badness}%
}

\def\tcb@split@upper@box@and@assemble{%
  \vfuzz=\maxdimen\vbadness=10000\savingvdiscards=1%
  \tcb@vsplit@upper%
  \ifnum\tcb@upper@box@badness=1000000\relax%
    \setbox\tcb@totalupperbox=\vbox{%
      \unvbox\tcb@upperbox%
      \splitdiscards%
      \unvbox\tcb@totalupperbox}%
  \else%
    \tcb@setbox@upper{\tcb@split@dim}{\tcb@upperbox}%
  \fi%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz\savingvdiscards=0%
}

\def\tcb@split@upper@box{%
  \vfuzz=\maxdimen\vbadness=10000%
  \tcb@vsplit@upper%
  \ifnum\tcb@upper@box@badness=1000000\relax%
    \tcb@warning{The upper box part has become overfull}%
  \fi%
  \tcb@setbox@upper{\tcb@split@dim}{\tcb@upperbox}%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
}

\def\tcb@setbox@lower#1#2{%
  \tcb@setbox\tcb@lowerbox{#1}{#2}%
  \tcbdimto\tcb@h@lower{\ht\tcb@lowerbox+\dp\tcb@lowerbox}%
}

\def\tcb@vsplit@lower{%
  \setbox\tcb@lowerbox=\vsplit\tcb@totallowerbox to\tcb@split@dim%
  \edef\tcb@lower@box@badness{\the\badness}%
}

\def\tcb@split@lower@box@and@assemble{%
  \vfuzz=\maxdimen\vbadness=10000\savingvdiscards=1%
  \tcb@vsplit@lower%
  \ifnum\tcb@lower@box@badness=1000000\relax%
    \setbox\tcb@totallowerbox=\vbox{%
      \unvbox\tcb@lowerbox%
      \splitdiscards%
      \unvbox\tcb@totallowerbox}%
  \else%
    \tcb@setbox@lower{\tcb@split@dim}{\tcb@lowerbox}%
  \fi%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz\savingvdiscards=0%
}


\def\tcb@split@lower@box{%
  \vfuzz=\maxdimen\vbadness=10000%
  \tcb@vsplit@lower%
  \ifnum\tcb@lower@box@badness=1000000\relax%
    \tcb@warning{The lower box part has become overfull}%
  \fi%
  \tcb@setbox@lower{\tcb@split@dim}{\tcb@lowerbox}%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
}

% patch for luatex 0.95 (thanks to Jeremy Engel)
\ifdefined\directlua
  \RequirePackage{ifluatex}
  \ifnum\luatexversion=95\relax
  \def\tcb@vsplit@upper{%
    \directlua{%
      tex.savingvdiscards = 1
      local vlist = tex.splitbox("tcb@totalupperbox", tex.sp("\tcb@split@dim"), "exactly")
      tex.setbox("tcb@upperbox", vlist)
      tex.savingvdiscards = 0
    }%
    \edef\tcb@upper@box@badness{\the\badness}%
  }
  \def\tcb@vsplit@lower{%
    \directlua{%
      tex.savingvdiscards = 1
      local vlist = tex.splitbox("tcb@totallowerbox", tex.sp("\tcb@split@dim"), "exactly")
      tex.setbox("tcb@lowerbox", vlist)
      tex.savingvdiscards = 0
    }%
    \edef\tcb@lower@box@badness{\the\badness}%
  }
\fi\fi

\def\tcb@split@setstate@first{%
  \edef\tcb@split@state{first}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@stand%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@break%
  \let\kvtcb@bbtop=\kvtcb@bbtop@stand%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@break%
  \let\tcb@break@topsep=\tcb@zpt%
  \let\tcb@break@bottomsep=\kvtcb@bottomsep%
}

\def\tcb@split@setstate@middle{%
  \edef\tcb@split@state{middle}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@break%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@break%
  \let\kvtcb@bbtop=\kvtcb@bbtop@break%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@break%
  \let\tcb@break@topsep=\kvtcb@topsep%
  \let\tcb@break@bottomsep=\kvtcb@bottomsep%
}

\def\tcb@split@setstate@last{%
  \edef\tcb@split@state{last}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@break%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@stand%
  \let\kvtcb@bbtop=\kvtcb@bbtop@break%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@stand%
  \let\tcb@break@topsep=\kvtcb@topsep%
  \let\tcb@break@bottomsep=\tcb@zpt%
}


\def\tcb@split@force@standalone{%
  \tcb@comp@h@total@standalone%
  \ifdim\tcb@h@total>\tcb@h@page\relax%
    \tcbdimto\kvtcb@bbbottom@stand{\kvtcb@bbbottom@stand+\tcb@h@page-\tcb@h@total}%
  \fi%
}


\def\tcb@split@break@to@start{%
  \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
  \tcb@swap{\tcb@totallowerbox}{\tcb@lowerbox}%
  \tcbdimto\tcb@h@upper{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \tcbdimto\tcb@h@lower{\ht\tcb@lowerbox+\dp\tcb@lowerbox}%
  \tcb@split@pagebreak%
  \let\tcb@split@next=\tcb@split@start%
}

\def\tcb@split@first{%
  \setcounter{tcbbreakpart}{1}%
  \ifx\kvtcb@float\@empty%
    \iftcb@vfillbeforefirst%
      \let\tcb@before@first=\vfill%
    \else%
    \let\tcb@before@first=\@empty%
    \fi%
    \let\tcb@before@middle=\@empty%
    \let\tcb@before@last=\@empty%
    \iftcb@multicol%
      \long\def\tcb@after@first{\par}% using \columnbreak here kills multicols' algortihm sometimes
      \long\def\tcb@after@middle{\par\vfill}%
    \else%
      \long\def\tcb@after@first{\par\pagebreak\tcb@enlbreak@next}%
      \long\def\tcb@after@middle{\par\vfill\eject\tcb@enlbreak@next}%
    \fi%
    \let\tcb@after@last=\par%
  \else%
    \edef\tcb@before@first{\noexpand\tcb@float@env@begin{tcbfloat}[\kvtcb@float]\noexpand\kvtcb@everyfloat}%
    \let\tcb@before@middle=\tcb@before@first%
    \let\tcb@before@last=\tcb@before@first%
    \let\tcb@after@first=\tcb@float@env@end%
    \let\tcb@after@middle=\tcb@float@env@end%
    \let\tcb@after@last=\tcb@float@env@end%
  \fi%
  %
  \edef\kvtcb@skin@@first{\kvtcb@skin@first}%
  \edef\kvtcb@skin@@middle{\kvtcb@skin@middle}%
  \edef\kvtcb@skin@@last{\kvtcb@skin@last}%
  %
  \let\tcb@h@breaksep@first=\kvtcb@bottomsep%
  \tcbdimto\tcb@h@breaksep@middle{\kvtcb@bottomsep+\kvtcb@topsep}%
  \let\tcb@h@breaksep@last=\kvtcb@topsep%
  \tcbdimto\tcb@h@padding@first{\kvtcb@bbtop@stand+\kvtcb@bbbottom@break+\kvtcb@top@rule@stand+\kvtcb@bottom@rule@break+\tcb@h@breaksep@first+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@padding@middle{\kvtcb@bbtop@break+\kvtcb@bbbottom@break+\kvtcb@top@rule@break+\kvtcb@bottom@rule@break+\tcb@h@breaksep@middle+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@padding@last{\kvtcb@bbtop@break+\kvtcb@bbbottom@stand+\kvtcb@top@rule@break+\kvtcb@bottom@rule@stand+\tcb@h@breaksep@last+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  %
  \tcb@split@setstate@first%
  %
  \splittopskip=0pt%
  \splitmaxdepth=0pt%
  \edef\tcb@thevfuzz{\the\vfuzz}%
  \edef\tcb@thevbadness{\the\vbadness}%
  %
  \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
  \tcb@swap{\tcb@totallowerbox}{\tcb@lowerbox}%
  %
  \let\tcb@split@next=\relax%
  \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@first-\tcb@h@padtitle}%
  \ifdim\tcb@split@dim<\tcb@h@upper\relax%
    %
    %
    \iftcb@break@allowed%
      \tcb@split@upper@box@and@assemble%
      \ifnum\tcb@upper@box@badness=1000000\relax%
        \tcb@split@break@to@start%
      \else%
        \ifdim\wd\tcb@totalupperbox=0pt\relax%
          \iftcb@lowerspace%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@SL%
          \else%
            \tcb@split@force@standalone%
            \tcb@drawcolorbox@standalone%
          \fi%
        \else%
          \ifdim\dimexpr\tcb@h@upper=0pt\relax%
            \tcb@split@break@to@start%
          \else%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@USL%
          \fi%
        \fi%
      \fi%
    \else%
      \tcb@split@upper@box%
      \ifdim\wd\tcb@totalupperbox=0pt\relax%
        \iftcb@lowerspace%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \tcb@split@force@standalone%
          \tcb@drawcolorbox@standalone%
        \fi%
      \else%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@USL%
      \fi%
    \fi%
  \else%
    \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
    \iftcb@lowerspace%
      \tcbdimto\tcb@split@dim{\tcb@split@dim-\tcb@h@upper-\tcb@h@segment}%
      \ifdim\tcb@split@dim<\kvtcb@breakminlines\baselineskip\relax%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@SL%
      \else
        \tcb@split@lower@box@and@assemble%
        \ifnum\tcb@lower@box@badness=1000000\relax%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \ifdim\wd\tcb@totallowerbox=0pt\relax%
            \tcb@split@force@standalone%
            \tcb@drawcolorbox@standalone%
          \else%
            \tcb@sdraw@USL%
            \let\tcb@split@next=\tcb@split@L%
          \fi%
        \fi%
      \fi%
    \else%
      \tcb@split@force@standalone%
      \tcb@drawcolorbox@standalone%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@force@last{%
  \tcb@split@setstate@last%
  \ifdim\tcb@h@total>\tcb@h@page%
    \tcbdimto\kvtcb@bbbottom{\kvtcb@bbbottom+\tcb@h@page-\tcb@h@total}%
  \fi%
}

\def\tcb@nextbreakpart{%
  \stepcounter{tcbbreakpart}%
  \tcb@count@boxes%
  \iftcb@checkpage%
    \tcb@phantom@savepage%
    \tcb@hasPhantomtrue%
    \sbox\tcb@phantombox{\kvtcb@phantom}%
    \let\kvtcb@phantom\@empty%
  \fi%
  \tcb@following@title%
}


\def\tcb@split@USL{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \tcb@defToTotalHeight\tcb@h@upper{\tcb@totalupperbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last+\tcb@h@padtitle+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@upper{\tcb@h@upper}{\tcb@totalupperbox}%
    \iftcb@lowerspace%
      \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
      \tcb@sdraw@USL%
    \else
      \tcb@sdraw@U%
    \fi%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle-\tcb@h@padtitle}%
    \ifdim\tcb@split@dim<\tcb@h@upper\relax%
      \tcb@split@upper@box%
      \ifdim\wd\tcb@totalupperbox=0pt\relax%
        \iftcb@lowerspace%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \tcb@split@force@last%
          \tcb@sdraw@U%
        \fi%
      \else%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@USL%
      \fi%
    \else%
      \tcb@setbox@upper{\tcb@h@upper}{\tcb@totalupperbox}%
      \iftcb@lowerspace%
        \tcbdimto\tcb@split@dim{\tcb@split@dim-\tcb@h@upper-\tcb@h@segment}
        \ifdim\tcb@split@dim<\kvtcb@breakminlines\baselineskip\relax%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else
          \tcb@split@lower@box@and@assemble%
          \ifnum\tcb@lower@box@badness=1000000\relax%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@SL%
          \else%
            \ifdim\wd\tcb@totallowerbox=0pt\relax%
              \tcb@split@force@last%
              \tcb@sdraw@USL%
            \else%
              \tcb@sdraw@USL%
              \let\tcb@split@next=\tcb@split@L%
            \fi%
          \fi%
        \fi%
      \else%
        \tcb@split@force@last%
        \tcb@sdraw@U%
      \fi%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@SL{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \let\tcb@h@upper=\tcb@zpt%
  \tcb@defToTotalHeight\tcb@h@lower{\tcb@totallowerbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last-\kvtcb@top-\kvtcb@boxsep+\tcb@h@padtitle+\tcb@h@segment+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
    \tcb@sdraw@SL%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle+\kvtcb@top+\kvtcb@boxsep-\tcb@h@padtitle-\tcb@h@segment}%
    \tcb@split@lower@box%
    \ifdim\wd\tcb@totallowerbox=0pt\relax%
      \tcb@split@force@last%
      \tcb@sdraw@SL%
    \else
      \tcb@sdraw@SL%
      \let\tcb@split@next=\tcb@split@L%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@L{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \let\tcb@h@upper=\tcb@zpt%
  \tcb@defToTotalHeight\tcb@h@lower{\tcb@totallowerbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last+\tcb@h@padtitle+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
    \tcb@sdraw@L%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle-\tcb@h@padtitle}%
    \tcb@split@lower@box%
    \ifdim\wd\tcb@totallowerbox=0pt\relax%
      \tcb@split@force@last%
      \tcb@sdraw@L%
    \else
      \tcb@sdraw@L%
      \let\tcb@split@next=\tcb@split@L%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@break@ch@fixed{%
  \ifdim\tcb@natheight<\tcb@h@page\relax%
    \tcbdimto\kvtcb@height@fixed{\tcb@h@page-\kvtcb@bbtop-\kvtcb@bbbottom}%
    \tcb@ch@fixed%
  \else%
    \tcb@ch@natural%
  \fi%
}


\def\tcb@sdraw@USL{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{1}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcbdimto\tcbtextheight{\tcb@innerheight-\kvtcb@boxsep*2-\kvtcb@top-\kvtcb@bottom}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
     % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \iftcb@lowerseparated%
      \tcb@segmentation@code%
    \fi%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@upper%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@U{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{0}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\tcb@h@upper+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcbdimto\tcbtextheight{\tcb@innerheight-\kvtcb@boxsep*2-\kvtcb@top-\kvtcb@bottom}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@upper%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@SL{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{1}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@bottom+\kvtcb@boxsep+\tcb@h@segment+\tcb@h@lower+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcbdimto\tcbtextheight{\tcb@innerheight-\kvtcb@boxsep*2-\kvtcb@top-\kvtcb@bottom}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \iftcb@lowerseparated%
      \tcb@segmentation@code%
    \fi%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@L{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{2}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\ht\tcb@lowerbox+\dp\tcb@lowerbox+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcbdimto\tcbtextheight{\tcb@innerheight-\kvtcb@boxsep*2-\kvtcb@top-\kvtcb@bottom}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}



\tcbset{%
  breakable@true/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightBreakable%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  breakable@unlimited/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightUnlimited%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  breakable/.style={breakable@#1},
  breakable/.default=true,%
  unbreakable/.style={breakable=false},%
  enforce breakable/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightBreakable%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  title after break/.store in=\kvtcb@followingtitle,%
  notitle after break/.style={title after break=},%
  adjusted title after break/.style={title after break={#1\vphantom{\kvtcb@adjusttext}}},%
  lines before break/.store in=\kvtcb@breakminlines,%
  shrink break goal/.store in=\kvtcb@shrinkbreakgoal,%
  toprule at break/.store in=\kvtcb@top@rule@break,
  bottomrule at break/.store in=\kvtcb@bottom@rule@break,
  topsep at break/.store in=\kvtcb@topsep,%
  bottomsep at break/.store in=\kvtcb@bottomsep,%
  pad before break/.code={\let\kvtcb@bottom@rule@break=\tcb@zpt%
    \tcbdimto\kvtcb@bottomsep{#1-\kvtcb@bottom-\kvtcb@boxsep}},%
  pad before break*/.style={pad before break={#1},%
    code={\tcbdimto\tcb@temp{\kvtcb@bottom@rule@stand-\kvtcb@bottomsep}%
      \ifdim\tcb@temp>0pt\relax%
        \tcbdimto\kvtcb@enlargepage@flex{\kvtcb@enlargepage@flex+\tcb@temp}\fi}},%
  pad after break/.code={\let\kvtcb@top@rule@break=\tcb@zpt%
    \tcbdimto\kvtcb@topsep{#1-\kvtcb@top-\kvtcb@boxsep}},%
  pad at break/.style={pad before break={#1},pad after break={#1}},%
  pad at break*/.style={pad before break*={#1},pad after break={#1}},%
  enlargepage/.store in=\kvtcb@enlargepage,%
  enlargepage flexible/.store in=\kvtcb@enlargepage@flex,%
  break at/.store in=\kvtcb@breakatdim,%
  height fixed for/.is choice,%
  height fixed for/none/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/first/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/middle/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/last/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  height fixed for/first and middle/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/middle and last/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  height fixed for/all/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  vfill before first/.is if=tcb@vfillbeforefirst,%
  height fill/true/.code={\let\tcb@height@adjust\tcb@height@fill@unbroken@normal},%
  height fill/maximum/.code={\let\tcb@height@adjust\tcb@height@fill@unbroken@compressed},%
  height fill/.default=true,%
  compress page/.is choice,%
  compress page/all/.code={\def\tcb@comp@compress{\def\tcb@compress@height{\pageshrink-1sp}}},%
  compress page/none/.code={\def\tcb@comp@compress{\let\tcb@compress@height\tcb@zpt}},%
  compress page/baselineskip/.code={\def\tcb@comp@compress{%
    \ifdim\pageshrink>\baselineskip%
      \let\tcb@compress@height\baselineskip%
    \else%
      \def\tcb@compress@height{\pageshrink-1sp}%
    \fi}},%
  compress page/.default=all,%
  compress page=baselineskip,% global setting
  extras unbroken/.code={\appto\tcb@extras@unbroken{\tcbset{#1}}},%
  extras first/.code={\appto\tcb@extras@first{\tcbset{#1}}},%
  extras middle/.code={\appto\tcb@extras@middle{\tcbset{#1}}},%
  extras last/.code={\appto\tcb@extras@last{\tcbset{#1}}},%
  extras/.style={extras unbroken={#1},extras first={#1},extras middle={#1},extras last={#1}},%
  extras broken/.style={extras first={#1},extras middle={#1},extras last={#1}},%
  extras unbroken and first/.style={extras unbroken={#1},extras first={#1}},%
  extras unbroken and last/.style={extras unbroken={#1},extras last={#1}},%
  extras middle and last/.style={extras middle={#1},extras last={#1}},%
  extras first and middle/.style={extras first={#1},extras middle={#1}},%
  no extras unbroken/.code={\let\tcb@extras@unbroken\@empty},%
  no extras first/.code={\let\tcb@extras@first\@empty},%
  no extras middle/.code={\let\tcb@extras@middle\@empty},%
  no extras last/.code={\let\tcb@extras@last\@empty},%
  no extras/.code={\let\tcb@extras@unbroken\@empty\let\tcb@extras@first\@empty\let\tcb@extras@middle\@empty\let\tcb@extras@last\@empty},%
  if odd page*/.style 2 args={check odd page,extras={if odd page={#1}{#2}}},%
}


\tcbset{%
  reset@breakable/.style={%
    unbreakable,notitle after break,
    shrink break goal=0pt,
    lines before break=2,
    topsep at break=0pt,
    bottomsep at break=0pt,
    enlargepage=0pt,enlargepage flexible=0pt,
    break at=0pt,
    height fixed for=none,
    vfill before first=false,
    no extras,
  },
  initialize@reset=reset@breakable,
}


==> tcbdocumentation.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcbdocumentation.code.tex: Code for LaTeX documentations
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.94}

\tcbuselibrary{listings,skins,xparse,external}

\RequirePackage{pifont}[2005/04/12]
\RequirePackage{marvosym}[2011/07/20]
\ifdefined\printindex\else\RequirePackage{makeidx}[2000/03/29]\fi
\RequirePackage{refcount}[2011/10/16]
\RequirePackage{hyperref}[2012/02/06]
\ifdefined\marginnote\else\RequirePackage{marginnote}[2012/03/29]\fi

\definecolor{Option}{rgb}{0.118,0.546,0.222}
\definecolor{Definition}{rgb}{0.784,0.06,0.176}
\definecolor{ExampleFrame}{rgb}{0.628,0.705,0.942}
\definecolor{ExampleBack}{rgb}{0.963,0.971,0.994}
\definecolor{Hyperlink}{rgb}{0.281,0.275,0.485}

\def\colDef#1{\textcolor{\kvtcb@col@command}{#1}}
\def\colOpt#1{\textcolor{\kvtcb@col@opt}{#1}}

\lstdefinestyle{tcbdocumentation}{language={[LaTeX]TeX},
    aboveskip={0\p@ \@plus 6\p@},
    belowskip={0\p@ \@plus 6\p@},
    columns=fullflexible,
    keepspaces=true,
    breaklines=true,
    prebreak={\Righttorque},
    postbreak={\space\Lefttorque},
    breakatwhitespace=true,
    basicstyle=\ttfamily\footnotesize,
    extendedchars=true,
    moredelim={[is][\itshape\rmfamily]{^^a7}{^^a7}},
    nolol,inputencoding=\kvtcb@listingencoding}

% The following macros are taken from ltxdoc
\DeclareRobustCommand\cs[1]{\texttt{\char`\\#1}}
\def\meta@font@select{\rmfamily\itshape}

\AtEndPreamble{%
  \@ifpackageloaded{doc}{%
  }{% code taken from doc.sty
    \ifx\l@nohyphenation\undefined
      \newlanguage\l@nohyphenation
    \fi
    \DeclareRobustCommand\meta[1]{%
         \ensuremath\langle
         \ifmmode \expandafter \nfss@text \fi
         {%
          \meta@font@select
          \edef\meta@hyphen@restore
            {\hyphenchar\the\font\the\hyphenchar\font}%
          \hyphenchar\font\m@ne
          \language\l@nohyphenation
          #1\/%
          \meta@hyphen@restore
         }\ensuremath\rangle
    }%
  }%
}%

\def\marg#1{%
  {\ttfamily\char`\{}\meta{#1}{\ttfamily\char`\}}}
\def\oarg#1{%
  \colOpt{{\ttfamily[}\meta{#1}{\ttfamily]}}}

\newrobustcmd\tcb@cs[1]{{\catcode`\_=12\relax\catcode`\@11\relax\ttfamily\char`\\\scantokens{#1}\unskip}}
\newrobustcmd\tcb@scantokens[1]{{\catcode`\_=12\relax\catcode`\@11\relax\ttfamily\scantokens{#1}\unskip}}

\newif\iftcb@doc@toindex
\newif\iftcb@doc@colorize
\newif\iftcb@doc@annotate

% language specific texts
\tcbset{
  doclang/.cd,
  color/.store in=\kvtcb@text@color,
  colors/.store in=\kvtcb@text@colors,
  counter/.store in=\kvtcb@text@counter,
  counters/.store in=\kvtcb@text@counters,
  environment content/.store in=\kvtcb@text@envcontent,
  environment/.store in=\kvtcb@text@env,
  environments/.store in=\kvtcb@text@envs,
  index/.store in=\kvtcb@text@index,
  key/.store in=\kvtcb@text@key,
  keys/.store in=\kvtcb@text@keys,
  length/.store in=\kvtcb@text@length,
  lengths/.store in=\kvtcb@text@lengths,
  new/.store in=\kvtcb@text@new,
  pageshort/.store in=\kvtcb@text@pageshort,
  updated/.store in=\kvtcb@text@updated,
  value/.store in=\kvtcb@text@value,
  values/.store in=\kvtcb@text@values,
}

% documentation options
\tcbset{
  documentation listing options/.store in=\kvtcb@doclistingoptions,%
  documentation listing style/.style={documentation listing options={style=#1}},%
  documentation minted style/.store in=\kvtcb@docmintstyle,
  documentation minted options/.store in=\kvtcb@docmintoptions,
  color command/.store in=\kvtcb@col@command,
  color environment/.store in=\kvtcb@col@environment,
  color key/.store in=\kvtcb@col@key,
  color value/.store in=\kvtcb@col@value,
  color counter/.store in=\kvtcb@col@counter,
  color length/.store in=\kvtcb@col@length,
  color color/.store in=\kvtcb@col@color,
  color definition/.style={color command={#1},color environment={#1},color key={#1},
    color value={#1},color color={#1},color counter={#1},color length={#1}},
  color option/.store in=\kvtcb@col@opt,
  color hyperlink/.store in=\kvtcb@colhyper,
  color frame/.store in=\kvtcb@colhyper,
  index actual/.store in=\idx@actual,
  index quote/.store in=\idx@quote,
  index level/.store in=\idx@level,
  index format/.store in=\idx@format,
  index colorize/.is if=tcb@doc@colorize,%
  index annotate/.is if=tcb@doc@annotate,%
  index command/.code={\def\kvtcb@index@command##1{#1{##1}}},%
  index command name/.code={\def\kvtcb@index@command##1{\index[#1]{##1}}},%
  doc left/.dimstore in=\kvtcb@doc@left,
  doc right/.dimstore in=\kvtcb@doc@right,
  doc left indent/.dimstore in=\kvtcb@doc@indentleft,
  doc right indent/.dimstore in=\kvtcb@doc@indentright,
  doc head command/.style={doc@head@command/.style={#1}},
  doc head environment/.style={doc@head@environment/.style={#1}},
  doc head key/.style={doc@head@key/.style={#1}},
  doc head/.style={doc head command={#1},doc head environment={#1},doc head key={#1}},
  before doc body command/.store in=\kvtcb@doc@body@command@before,
  after doc body command/.store in=\kvtcb@doc@body@command@after,
  before doc body environment/.store in=\kvtcb@doc@body@environment@before,
  after doc body environment/.store in=\kvtcb@doc@body@environment@after,
  before doc body key/.store in=\kvtcb@doc@body@key@before,
  after doc body key/.store in=\kvtcb@doc@body@key@after,
  before doc body/.style={before doc body command={#1},before doc body environment={#1},before doc body key={#1}},
  after doc body/.style={after doc body command={#1},after doc body environment={#1},after doc body key={#1}},
  doc description/.store in=\kvtcb@doc@description,%
  doc into index/.is if=tcb@doc@toindex,%
  doc updated/.style={before upper={\tcbdocmarginnote{\tcbdocupdated{#1}}}},
  doc new/.style={before upper={\tcbdocmarginnote{\tcbdocnew{#1}}}},
  doc new and updated/.style 2 args={before upper={\tcbdocmarginnote{\tcbdocnew{#1}\\\tcbdocupdated{#2}}}},
  doc marginnote/.style={doc@marginnote/.style={#1}},
}


% styles
\tcbset{
  docexample/.style={colframe=ExampleFrame,colback=ExampleBack,
    before skip=\medskipamount,after skip=\medskipamount,
    fontlower=\footnotesize},
  documentation minted style=,
  documentation minted options={tabsize=2,fontsize=\small},
  index default settings/.style={index actual={@},index quote={"},index level={!}},
  index german settings/.style={index actual={=},index quote={!},index level={>}},
  english language/.code={\tcbset{doclang/.cd,
    color=color,colors=Colors,
    counter=counter,counters=Counters,
    environment content=environment content,
    environment=environment,environments=Environments,
    index=Index,
    key=key,keys=Keys,
    length=length,lengths=Lengths,
    new=New,
    pageshort={P.},
    updated=Updated,
    value=value,values=Values}},
}

\AtBeginDocument{%
  \csname tcb@doc@index@\idx@format\endcsname%
  \hypersetup{
  citecolor=\kvtcb@colhyper,
  linkcolor=\kvtcb@colhyper,
  urlcolor=\kvtcb@colhyper,
  filecolor=\kvtcb@colhyper,
  menucolor=\kvtcb@colhyper
}}

\def\dispExample{\tcb@layer@pushup\tcbset{docexample}\begingroup\tcbwritetemp}

\def\enddispExample{%
  \endtcbwritetemp\endgroup%
  \begin{tcolorbox}%
  \tcb@doc@usetemplisting%
  \tcblower%
  \tcbusetemp%
  \end{tcolorbox}%
}

\newenvironment{dispExample*}[1]{%
  \tcb@layer@pushup\tcbset{docexample,#1}\begingroup\tcbwritetemp%
  }{\enddispExample}

\def\dispListing{\tcb@layer@pushup\tcbset{docexample}\begingroup\tcbwritetemp}

\def\enddispListing{%
  \endtcbwritetemp\endgroup%
  \begin{tcolorbox}%
  \tcb@doc@usetemplisting%
  \end{tcolorbox}%
}

\newenvironment{dispListing*}[1]{%
  \tcb@layer@pushup\tcbset{docexample,#1}\begingroup\tcbwritetemp%
  }{\enddispListing}

% index auxiliary macros
\def\tcb@Index@Print@CA#1#2#3{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@scantokens{#1}}\else\tcb@scantokens{#1}\fi%
  \iftcb@doc@annotate\ #3\fi%
}

\def\tcb@Index@Print@C#1#2{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@scantokens{#1}}\else\tcb@scantokens{#1}\fi%
}

\def\tcb@Index@Print@ComCA#1#2#3{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@cs{#1}}\else\tcb@cs{#1}\fi%
  \iftcb@doc@annotate\ #3\fi%
}

\def\tcb@Index@Print@ComC#1#2{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@cs{#1}}\else\tcb@cs{#1}\fi%
}

\newrobustcmd{\tcbIndexPrintComC}[1]{\tcb@Index@Print@ComC{#1}{\kvtcb@col@command}}
\def\tcb@Print@Com#1{\textcolor{\kvtcb@col@command}{\bfseries\tcb@cs{#1}}}

\newrobustcmd{\tcbIndexPrintEnvCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@environment}{\kvtcb@text@env}}
\newrobustcmd{\tcbIndexPrintEnvC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@environment}}
\def\tcb@Print@Env#1{\textcolor{\kvtcb@col@environment}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintKeyCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@key}{\kvtcb@text@key}}
\newrobustcmd{\tcbIndexPrintKeyC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@key}}
\def\tcb@Print@Key#1{\textcolor{\kvtcb@col@key}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintValCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@value}{\kvtcb@text@value}}
\newrobustcmd{\tcbIndexPrintValC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@value}}
\def\tcb@Print@Val#1{\textcolor{\kvtcb@col@value}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintColCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@color}{\kvtcb@text@color}}
\newrobustcmd{\tcbIndexPrintColC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@color}}
\def\tcb@Print@Col#1{\textcolor{\kvtcb@col@color}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintCountCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@counter}{\kvtcb@text@counter}}
\newrobustcmd{\tcbIndexPrintCountC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@counter}}
\def\tcb@Print@Count#1{\textcolor{\kvtcb@col@counter}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintLenCA}[1]{\tcb@Index@Print@ComCA{#1}{\kvtcb@col@length}{\kvtcb@text@length}}
\newrobustcmd{\tcbIndexPrintLenC}[1]{\tcb@Index@Print@ComC{#1}{\kvtcb@col@length}}
\def\tcb@Print@Len#1{\textcolor{\kvtcb@col@length}{\bfseries\tcb@cs{#1}}}

\def\tcb@index@Com#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintComC{#1}}\fi}
\def\tcb@index@Env#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintEnvCA{#1}}\kvtcb@index@command{\kvtcb@text@envs\idx@level#1\idx@actual\tcbIndexPrintEnvC{#1}}\fi}
\def\tcb@index@Key#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintKeyCA{#1}}\kvtcb@index@command{\kvtcb@text@keys\idx@level#1\idx@actual\tcbIndexPrintKeyC{#1}}\fi}%
\def\tcb@index@KeyPath#1#2{\iftcb@doc@toindex\kvtcb@index@command{#2\idx@actual\tcbIndexPrintKeyCA{#2}}\kvtcb@index@command{\kvtcb@text@keys\idx@level#1\idx@actual\tcbIndexPrintKeyC{/#1/}\idx@level#2\idx@actual\tcbIndexPrintKeyC{#2}}\fi}%
\def\tcb@index@Val#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintValCA{#1}}\kvtcb@index@command{\kvtcb@text@values\idx@level#1\idx@actual\tcbIndexPrintValC{#1}}\fi}
\def\tcb@index@Col#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintColCA{#1}}\kvtcb@index@command{\kvtcb@text@colors\idx@level#1\idx@actual\tcbIndexPrintColC{#1}}\fi}
\def\tcb@index@Count#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintCountCA{#1}}\kvtcb@index@command{\kvtcb@text@counters\idx@level#1\idx@actual\tcbIndexPrintCountC{#1}}\fi}
\def\tcb@index@Len#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintLenCA{#1}}\kvtcb@index@command{\kvtcb@text@lengths\idx@level#1\idx@actual\tcbIndexPrintLenC{#1}}\fi}

\def\brackets#1{{\ttfamily\char`\{}#1{\ttfamily\char`\}}}

\newenvironment{tcb@manual@entry}{\begin{list}{}{%
  \setlength{\leftmargin}{\kvtcb@doc@left}%
  \setlength{\itemindent}{0pt}%
  \setlength{\itemsep}{0pt}%
  \setlength{\parsep}{0pt}%
  \setlength{\rightmargin}{\kvtcb@doc@right}%
  }\item}{\end{list}}

\def\tcb@manual@top#1{\itemsep=0pt\parskip=0pt\item\strut{#1}\par\topsep=0pt}

\def\tcb@doc@do@description{%
  \ifx\kvtcb@doc@description\@empty\else\tcblower\raggedleft(\kvtcb@doc@description)\fi%
}

\newtcolorbox{tcb@doc@head}[1]{blank,colback=white,colframe=white,
  code={\tcbdimto\tcb@temp@grow@left{-\kvtcb@doc@indentleft}%
        \tcbdimto\tcb@temp@grow@right{-\kvtcb@doc@indentright}},
  grow to left by=\tcb@temp@grow@left,%
  grow to right by=\tcb@temp@grow@right,
  sidebyside,sidebyside align=top,
  sidebyside gap=-\tcb@w@upper@real,
  phantom=\phantomsection,%
  enlarge bottom by=-0.2\baselineskip,#1}

% main documentation environments
\newenvironment{docCommand}[3][]{\tcbset{#1}%
  \begin{tcb@manual@entry}%
  \begin{tcb@doc@head}{doc@head@command}%
  \tcb@Print@Com{#2}\tcb@index@Com{#2}\protected@edef\@currentlabel{\noexpand\tcb@cs{#2}}\label{com:#2}{\ttfamily #3}%
  \tcb@doc@do@description%
  \end{tcb@doc@head}\nobreak\tcbset{before upper=}\kvtcb@doc@body@command@before\ignorespaces}%
  {\ifvmode\else\unskip\fi\kvtcb@doc@body@command@after\end{tcb@manual@entry}}

\newenvironment{docCommand*}{\bgroup\tcb@doc@toindexfalse\begin{docCommand}}{\end{docCommand}\egroup}

\newenvironment{docEnvironment}[3][]{\tcbset{#1}%
  \begin{tcb@manual@entry}%
  \begin{tcb@doc@head}{doc@head@environment}%
  \strut\cs{begin}\brackets{\tcb@Print@Env{#2}}\tcb@index@Env{#2}\protected@edef\@currentlabel{#2}\label{env:#2}{\ttfamily #3}\par%
  \strut~~\meta{\kvtcb@text@envcontent}\par%
  \strut\cs{end}\brackets{\tcb@Print@Env{#2}}%
  \tcb@doc@do@description%
  \end{tcb@doc@head}\nobreak\tcbset{before upper=}\kvtcb@doc@body@environment@before\ignorespaces}%
  {\ifvmode\else\unskip\fi\kvtcb@doc@body@environment@after\end{tcb@manual@entry}}

\newenvironment{docEnvironment*}{\bgroup\tcb@doc@toindexfalse\begin{docEnvironment}}{\end{docEnvironment}\egroup}

\NewDocumentEnvironment{docKey}{ O{} +O{} m m +m }{\tcbset{#2,doc description={#5}}%
  \begin{tcb@manual@entry}%
  \begin{tcb@doc@head}{doc@head@key}%
  \ifblank{#1}{%
    \tcb@Print@Key{#3}\tcb@index@Key{#3}\protected@edef\@currentlabel{#3}\label{key:#3}{\ttfamily #4}%
  }{%
    \tcb@Print@Key{/#1/#3}%
    \tcb@index@KeyPath{#1}{#3}\protected@edef\@currentlabel{/#1/#3}\label{key:/#1/#3}{\ttfamily #4}%
  }%
  \tcb@doc@do@description%
  \end{tcb@doc@head}\nobreak\tcbset{before upper=}\kvtcb@doc@body@key@before\ignorespaces}%
  {\ifvmode\else\unskip\fi\kvtcb@doc@body@key@after\end{tcb@manual@entry}}

\newenvironment{docKey*}{\bgroup\tcb@doc@toindexfalse\begin{docKey}}{\end{docKey}\egroup}

\def\tcbmakedocSubKey#1#2{%
  \NewDocumentEnvironment{#1}{ O{} +O{} m m +m }{%
    \ifblank{##1}{\def\tcb@key@path{#2}}{\def\tcb@key@path{#2/##1}}%
    \begin{docKey}[\tcb@key@path][##2]{##3}{##4}{##5}}%
      {\end{docKey}}%
  \newenvironment{#1*}{\bgroup\tcb@doc@toindexfalse\begin{#1}}{\end{#1}\egroup}%
}

\DeclareDocumentCommand\docAuxCommand{sm}{%
  \tcb@Print@Com{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Com{#2}}%
}

\DeclareDocumentCommand\docAuxEnvironment{sm}{%
  \tcb@Print@Env{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Env{#2}}%
}

\DeclareDocumentCommand\docAuxKey{sO{}m}{%
  \ifblank{#2}{%
    \tcb@Print@Key{#3}%
    \IfBooleanTF{#1}{}{\tcb@index@Key{#3}}%
  }{%
    \tcb@Print@Key{/#2/#3}%
    \IfBooleanTF{#1}{}{\tcb@index@KeyPath{#2}{#3}}%
}}

\DeclareDocumentCommand\docColor{sm}{%
  \tcb@Print@Col{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Col{#2}}%
}

\DeclareDocumentCommand\docCounter{sm}{%
  \tcb@Print@Count{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Count{#2}}%
}

\DeclareDocumentCommand\docLength{sm}{%
  \tcb@Print@Len{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Len{#2}}%
}

\DeclareDocumentCommand\docValue{sm}{%
  \tcb@Print@Val{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Val{#2}}%
}

\setrefcountdefault{-1}
\DeclareDocumentCommand\tcb@ref@doc{msm}{%
  \hyperref[#1:#3]{\texttt{\ref*{#1:#3}}%
  \IfBooleanTF{#2}{}{%
    \ifnum\getpagerefnumber{#1:#3}=\thepage%
    \else%
      \textsuperscript{\ding{213}\,\kvtcb@text@pageshort\,\pageref*{#1:#3}}%
    \fi}}%
}

\def\refCom{\tcb@ref@doc{com}}
\def\refEnv{\tcb@ref@doc{env}}
\def\refKey{\tcb@ref@doc{key}}

\def\refAux#1{\textcolor{\kvtcb@colhyper}{\tcb@scantokens{#1}}}
\def\refAuxcs#1{\textcolor{\kvtcb@colhyper}{\tcb@cs{#1}}}

\newenvironment{absquote}
               {\list{}{\leftmargin2cm\rightmargin\leftmargin}%
                \item\relax\footnotesize}
               {\endlist}

\newcommand{\tcbdocmarginnote}[2][]{%
  \marginnote{%
  \begin{tcolorbox}[enhanced jigsaw,size=fbox,boxrule=1pt,leftrule=0pt,rightrule=0pt,
    arc=0pt,outer arc=1pt,boxsep=1pt,top=1pt,bottom=1pt,
    nobeforeafter,width=\marginparwidth,
    colframe=red!50!white,colback=red!25!yellow!5!white,fontupper=\scriptsize,before upper=\flushright,
    doc@marginnote,#1]#2\end{tcolorbox}}}

\newcommand*{\tcbdocnew}[1]{\kvtcb@text@new: #1}
\newcommand*{\tcbdocupdated}[1]{\kvtcb@text@updated: #1}

%--- index macros taken from pgfmanual-en-macros
\def\tcb@doc@index@pgf@{%
  \ifdefined\c@IndexColumns%
    \c@IndexColumns=2%
  \fi%
  \def\theindex{\@restonecoltrue
    \columnseprule \z@  \columnsep 29\p@
    \twocolumn[\index@prologue]%
    \parindent -30pt%
    \columnsep 15pt%
    \parskip 0pt plus 1pt%
    \leftskip 30pt%
    \rightskip 0pt plus 2cm%
    \small%
    \def\@idxitem{\par}%
    \let\item\@idxitem\ignorespaces}
  \def\endtheindex{\onecolumn}%
  \def\noindexing{\let\index=\@gobble}%
}

\def\tcb@doc@index@pgfsection{%
  \def\index@prologue{\section*{\kvtcb@text@index}\addcontentsline{toc}{section}{\kvtcb@text@index}%
    \par\noindent%
  }%
  \tcb@doc@index@pgf@%
}

\def\tcb@doc@index@pgfchapter{%
  \def\index@prologue{\ifdefined\phantomsection\phantomsection\fi\@makeschapterhead{\kvtcb@text@index}\addcontentsline{toc}{chapter}{\kvtcb@text@index}}%
  \tcb@doc@index@pgf@%
}

\let\tcb@doc@index@pgf=\tcb@doc@index@pgfsection%

\def\tcb@doc@index@doc{%
  \let\tcb@index@Com=\SpecialMainIndex%%
  \let\tcb@index@Env=\SpecialMainEnvIndex%
  \tcbset{index german settings}%
  \EnableCrossrefs%
  \PageIndex%
}

\def\tcb@doc@index@off{}%

\tcbset{%
  reset@documentation/.style={%
    index command=\index,%
    index format=pgf,
    english language,
    documentation listing style=tcbdocumentation,
    index default settings,
    color option=Option,
    color definition=Definition,
    color hyperlink=Hyperlink,
    doc left=2em,
    doc right=0pt,
    doc left indent=-2em,
    doc right indent=0pt,
    doc head=,
    before doc body=,
    after doc body=,
    doc description=,
    doc into index=true,
    index colorize=false,
    index annotate=true,
    doc marginnote=,
    },
  initialize@reset=reset@documentation,
}

% deprecated
\tcbset{
  before example/.store in=\kvtcb@beforeexample,
  after example/.store in=\kvtcb@afterexample,
    before example=\par\smallskip,
    after example=,
}


==> tcbexternal.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcbexternal.code.tex: Code for externalization
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.94}



{
\catcode`\"=12
\xdef\tcbexternal@normal@dq{"}
\catcode`\"=13
\gdef\tcbexternal@activate@normal@dq{\let"=\tcbexternal@normal@dq}
}

\long\def\tcbifexternal#1#2{%
  \ifdefined\TCBEXTERNALINPUT%
    #1%
  \else%
    #2%
  \fi%
}

\tcbifexternal{%
  \def\tcbEXTERNALIZE{%
    \RequirePackage{incgraph}%
    \TCBEXTERNALPREAMBLE%
    \begin{document}%
    \begin{inctext}[border=\TCBEXTERNALSAFETY]%
    \input{\TCBEXTERNALINPUT}%
    \end{inctext}%
    \end{document}%
  }%
}{%
  \def\tcbEXTERNALIZE{%
    \tcbset{
      external/.cd,
      externalize/.is if=tcb@externalize,
      externalize=true,
    }%
  }%
}

\@onlypreamble\tcbEXTERNALIZE

\def\tcbexternal@setbasename#1{%
  \edef\tcbexternal@job@name{\expandonce{\tcbexternal@prefix}\expandonce{#1}}%
  \edef\tcbexternal@job@mdfive{\expandonce{\tcbexternal@job@name.md5}}%
  \edef\tcbexternal@job@source{\expandonce{\tcbexternal@job@name.tex}}%
  \edef\tcbexternal@job@pdf{\expandonce{\tcbexternal@job@name.pdf}}%
}

\def\tcbexternal@corecompile{%
  \begingroup%
  \ifnum\the\catcode`\"=13 \tcbexternal@activate@normal@dq\fi%
  \message{=== Compile external '\tcbexternal@job@name': }%
  \immediate\openout\tcb@out="\tcbexternal@run@tex"
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALINPUT{"\tcbexternal@job@source"}}%
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALSAFETY{\tcbexternal@safety}}%
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALPREAMBLE{\expandonce{\tcbexternal@preamble}}}%
  \ifdefempty{\tcbexternal@preclass}{}{\immediate\write\tcb@out{\expandonce{\tcbexternal@preclass}}}%
  \immediate\write\tcb@out{\string\input{"\jobname.tex"}}%
  \immediate\closeout\tcb@out%
  \foreach \n in {1,...,\tcbexternal@runs}
  {%
    \ShellEscape{%
      \tcbexternal@compiler\space
      -shell-escape
      -halt-on-error
      -interaction=batchmode
      -jobname="\tcbexternal@job@name"
      "\tcbexternal@run@tex"
    }%
  }%
  \endgroup%
}

\def\tcbexternal@compile#1{%
  \tcbiffileprocess{#1}%
    {\tcbexternal@job@source}{\tcbexternal@job@mdfive}{\tcbexternal@job@pdf}%
    {\tcbexternal@corecompile}{}%
}

\def\tcbexternal@inputsource{%
  \IfFileExists{\tcbexternal@job@source}%
    {\input{\tcbexternal@job@source}}%
    {\tcb@error{File '\tcbexternal@job@source' missing.}{}}%
}

\def\tcbexternal@pdfmissing@warning{%
  \tcb@warning{File '\tcbexternal@job@pdf' missing.
    Compilation error or shell-escape wasn't enabled or a subdirectory could'nt be generated}%
  \message{Load '\tcbexternal@job@source' instead}%
  \tcbexternal@inputsource%
}

\def\tcbexternal@pdfmissing@error{%
  \tcb@error{File '\tcbexternal@job@pdf' missing.
    Compilation error or shell-escape wasn't enabled or a subdirectory could'nt be generated}{}%
}

\def\tcbexternal@inputpdf{%
  \IfFileExists{\tcbexternal@job@pdf}%
    {%
      \begingroup\edef\x{\endgroup%
        \noexpand\includegraphics[trim=\tcbexternal@safety\space\tcbexternal@safety%
        \space\tcbexternal@safety\space\tcbexternal@safety]{\expandonce{\tcbexternal@job@pdf}}}%
      \x%
    }%
    {\tcbexternal@pdfmissing}%
}

\newif\iftcb@externalize
\tcb@externalizefalse

\def\tcb@useexternal{%
  \iftcb@externalize%
    \tcbexternal@compile{\tcbexternal@condition}%
    \tcbexternal@inputpdf%
  \else%
    \tcbexternal@compile{2}%
    \tcbexternal@inputsource%
  \fi%
}

\newenvironment{tcbexternal}[2][]{%
  \tcbset{external/.cd,#1,name=#2}%
  \@ifundefined{@tcbexternal@JN@\tcbexternal@job@name}{%
      \global\@namedef{@tcbexternal@JN@\tcbexternal@job@name}{}%
    }{%
      \tcb@error{External job name '\tcbexternal@job@name' already used}%
        {Give a new unique name to the current external job.}%
    }%
  \begingroup%
  \let\tcb@verbatim@begin@hook=\tcbexternal@out@begin%
  \let\tcb@verbatim@end@hook=\tcbexternal@out@end%
  \tcbverbatimwrite{\tcbexternal@job@source}}%
{%
  \endtcbverbatimwrite\endgroup%
  \tcb@useexternal%
}

\long\def\new@tcb@externalizeenvironment#1#2#3#4#5{%
  \tcb@newenvironment{#1}[2][]{%
    #4%
    \begingroup%
    \tcbexternal[#3,##1,environment=#2]{##2}%
  }{%
    \endtcbexternal%
    \endgroup%
    #5%
  }%
}

\def\newtcbexternalizeenvironment{%
  \let\tcb@newenvironment\newenvironment%
  \new@tcb@externalizeenvironment%
}

\def\renewtcbexternalizeenvironment{%
  \let\tcb@newenvironment\renewenvironment%
  \new@tcb@externalizeenvironment%
}

\long\def\new@tcb@externalizetcolorbox#1#2#3#4{%
  \new@tcb@externalizeenvironment{#1}{#2}%
    {preamble tcbset={force nobeforeafter},#3}%
    {\tcb@layer@pushup\tcb@apply@box@options{#4}\tcb@set@normal@unbroken@beforeafter\tcb@before@unbroken}%
    {\tcb@after@unbroken}%
}

\def\newtcbexternalizetcolorbox{%
  \let\tcb@newenvironment\newenvironment%
  \new@tcb@externalizetcolorbox%
}

\def\renewtcbexternalizetcolorbox{%
  \let\tcb@newenvironment\renewenvironment%
  \new@tcb@externalizetcolorbox%
}


\newtcbexternalizeenvironment{extikzpicture}{tikzpicture}{}{}{}

\newtcbexternalizetcolorbox{extcolorbox}{tcolorbox}{}{}


\tcbset{
  external/.cd,
  %
  runner/.code={%
    \edef\tcbexternal@run@tex{\expandonce{#1}}%
  },
  %
  prefix/.store in=\tcbexternal@prefix,
  compiler/.store in=\tcbexternal@compiler,
  runs/.code={\numdef\tcbexternal@runs{#1}},
  name/.code={\tcbexternal@setbasename{#1}},
  safety/.store in=\tcbexternal@safety,
  preamble/.code={\appto\tcbexternal@preamble{#1}},
  preamble tcbset/.code={\appto\tcbexternal@preamble{\tcbset{#1}}},
  clear preamble/.code={\def\tcbexternal@preamble{}},
  preclass/.code={\appto\tcbexternal@preclass{#1}},
  clear preclass/.code={\def\tcbexternal@preclass{}},
  PassOptionsToPackage/.code 2 args={\appto\tcbexternal@preclass{\PassOptionsToPackage{#1}{#2}}},
  PassOptionsToClass/.code 2 args={\appto\tcbexternal@preclass{\PassOptionsToClass{#1}{#2}}},
  externalize/.code={},
  -/.style={externalize=false},
  %
  force remake/.is choice,
  force remake/true/.code={\def\tcbexternal@condition{0}},
  force remake/false/.code={\def\tcbexternal@condition{1}},
  force remake/.default=true,
  !/.style=force remake,
  %
  input source on error/.is choice,
  input source on error/true/.code={\let\tcbexternal@pdfmissing=\tcbexternal@pdfmissing@warning},
  input source on error/false/.code={\let\tcbexternal@pdfmissing=\tcbexternal@pdfmissing@error},
  input source on error/.default=true,
  %
  plain/.code={%
    \let\tcbexternal@out@begin=\@empty%
    \let\tcbexternal@out@end=\@empty%
  },
  minipage/.code={%
    \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{minipage}{\the\dimexpr#1\relax}\string\ignorespaces\@percentchar}}%
    \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{minipage}\@percentchar}}%
  },
  minipage/.default=\linewidth,
  %
  environment with percent/.is choice,
  environment with percent/true/.style={%
    /tcb/external/environment/.code={%
      \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{##1}\@percentchar}}%
      \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{##1}\@percentchar}}%
    }
  },
  environment with percent/false/.style={%
    /tcb/external/environment/.code={%
      \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{##1}}}%
      \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{##1}}}%
    }
  },
  environment with percent/.default=true,
  %
  runner=\jobname_run.tex,
  prefix={external/},
  compiler=pdflatex,
  runs=1,
  name=unnamed,
  safety=2mm,
  clear preamble,
  clear preclass,
  force remake=false,
  input source on error,
  environment with percent,
  plain
}

\tcbset{%
  externalize example/.style={%
    external/name=#1,tempfile=\tcbexternal@job@source,
    code={\let\tcbusetemp=\tcb@useexternal}%
  },
  externalize example!/.style={externalize example=#1,external/force remake},
  externalize listing/.style={%
    external/name=#1,listing file=\tcbexternal@job@source,
    code={\let\tcbuselistingtext@input=\tcb@useexternal}%
  },
  externalize listing!/.style={externalize listing=#1,external/force remake},
}


==> tcbfitting.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcbfitting.code.tex: Code for fit boxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.94}

\newdimen\tcbfitdim
\newdimen\tcb@lowerfitdim
\newdimen\tcb@upperfitdim
\newif\iftcb@continue

\tcbset{%
  fit/.style={capture=fitbox},%
  fit to/.style args={#1 and #2}{capture=fitbox,width=#1,height=#2},%
  fit to height/.style={capture=fitbox,height=#1},%
  fit basedim/.code={\def\kvtcb@fit@basedim{#1}\tcbfitdim\kvtcb@fit@basedim},%
  fit skip/.store in=\kvtcb@fit@skip,%
  fit fontsize macros/.code={%
    \renewcommand\tiny{\tcb@setfontsize\tiny{0.5}}%
    \renewcommand\scriptsize{\tcb@setfontsize\scriptsize{0.7}}%
    \renewcommand\footnotesize{\tcb@setfontsize\footnotesize{0.8}}%
    \renewcommand\small{\tcb@setfontsize\small{0.9}}%
    \renewcommand\normalsize{\tcb@setfontsize\normalsize{1}}%
    \renewcommand\large{\tcb@setfontsize\large{1.2}}%
    \renewcommand\Large{\tcb@setfontsize\Large{1.44}}%
    \renewcommand\LARGE{\tcb@setfontsize\LARGE{1.728}}%
    \renewcommand\huge{\tcb@setfontsize\huge{2.0736}}%
    \renewcommand\Huge{\tcb@setfontsize\Huge{2.48832}}},%
  fit height plus/.style={fit,height plus=#1},%
  fit width plus/.dimstore in=\kvtcb@fit@plus@width,%
  fit height from/.style args={#1 to #2}{fit,height from={#1} to {#2}},
  fit width from/.style args={#1 to #2}{fit,width={#1},fit width plus={#2-#1}},
  fit maxstep/.store in=\kvtcb@fit@maxstep,%
  fit maxfontdiff/.store in=\kvtcb@fit@maxfontdiff,%
  fit maxfontdiffgap/.store in=\kvtcb@fit@maxfontdiffgap,%
  fit maxwidthdiff/.store in=\kvtcb@fit@maxwidthdiff,%
  fit maxwidthdiffgap/.store in=\kvtcb@fit@maxwidthdiffgap,%
  fit warning/.is choice,
  fit warning/on/.code={\let\tcb@fit@warn@begin=\@empty%
    \let\tcb@fit@warn@end=\@empty},
  fit warning/off/.code={\def\tcb@fit@warn@begin{\hbadness=10000\relax}%
    \let\tcb@fit@warn@end=\@empty},
  fit warning/final/.code={\tcb@cur@hbadness=\hbadness\def\tcb@fit@warn@begin{\hbadness=10000\relax}%
    \def\tcb@fit@warn@end{\hbadness=\tcb@cur@hbadness\relax\tcb@fit@@box}},
  fit algorithm/.is choice,
  fit algorithm/fontsize/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@fontsize},
  fit algorithm/fontsize*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@fontsize@star},
  fit algorithm/areasize/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@areasize},
  fit algorithm/areasize*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@areasize@star},
  fit algorithm/hybrid/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@hybrid},
  fit algorithm/hybrid*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@hybrid@star},
  fit algorithm/squeeze/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@squeeze},
  spartan@fit/.style={fit algorithm=squeeze},
}

\def\tcb@@capture@fitbox{%
  \let\endtcolorbox=\relax%
  \Collect@Body\tcbox@inner@fitbox@collected%
}

\def\tcbfontsize#1{\fontsize{#1\tcbfitdim}{#1\dimexpr\kvtcb@fit@skip\tcbfitdim}\selectfont}

\def\tcb@setfontsize#1#2{\@setfontsize#1{#2\tcbfitdim}{#2\dimexpr\kvtcb@fit@skip\tcbfitdim}}

\long\def\tcbox@inner@fitbox@collected#1{%
  \tcbox@inner@fitbox{#1}%
  \tcb@finalize@environment%
}

\newcount\tcb@cur@hbadness

\def\tcbox@fitalgorithm@fontsize{%
  \tcb@continuetrue%
  \loop%
    \tcbfitdim.5\tcbfitdim%
    \tcb@fit@@box%
    \ifnum\count@=\kvtcb@fit@maxstep\relax%
      \tcb@continuefalse%
    \else%
      \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \ifdim\tcbfitdim<18000sp\relax%
          \count@\kvtcb@fit@maxstep\relax%
          \tcb@continuefalse%
        \fi%
      \else%
        \tcb@continuefalse%
      \fi%
    \fi%
  \iftcb@continue \repeat%
  \ifnum\count@<\kvtcb@fit@maxstep\relax%
    \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
    \tcb@lowerfitdim\tcbfitdim%
    \tcb@upperfitdim2\tcbfitdim%
    \tcbfitdim1.5\tcbfitdim%
    \loop%
      \tcb@fit@@box%
      \tcb@continuetrue%
      \ifnum\count@<\kvtcb@fit@maxstep\relax%
        \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxfontdiff\relax%
          \tcb@continuefalse%
        \else%
          \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxfontdiffgap\relax%
            \ifdim\dimexpr\tcb@fit@@gap<\tcb@fit@@line\relax%
              \tcb@continuefalse%
            \fi%
          \fi%
        \fi%
      \else%
        \tcb@continuefalse%
      \fi%
      \iftcb@continue%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
          \tcb@upperfitdim\tcbfitdim%
          \advance\tcbfitdim\tcb@lowerfitdim%
          \tcbfitdim0.5\tcbfitdim%
        \else%
          \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
          \tcb@lowerfitdim\tcbfitdim%
          \advance\tcbfitdim\tcb@upperfitdim%
          \tcbfitdim0.5\tcbfitdim%
        \fi%
      \else%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
          \tcbfitdim\tcb@lowerfitdim%
          \tcb@fit@@box%
        \fi%
      \fi%
    \iftcb@continue \repeat%
  \fi%
}

\def\tcbox@fitalgorithm@fontsize@star{%
  \tcbox@fitalgorithm@fontsize%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize@core{%
  \pgfmathdivide{\tcb@fit@@h}{\tcb@fit@@target}%
  \pgfmathsqrt{\pgfmathresult}%
  \let\tcb@temp=\pgfmathresult%
  \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper}%
  \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \pgfmathdivide{\tcb@fit@@h}{\tcb@fit@@target}%
  \pgfmathdivide{\pgfmathresult}{\tcb@temp}%
  \pgfmathsqrt{\pgfmathresult}%
  \ifdim\dimexpr\pgfmathresult pt<0.98pt\relax
    \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper@temp}%
    \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  \else\ifdim\dimexpr\pgfmathresult pt>1.02pt\relax
    \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper@temp}%
    \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  \fi\fi%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize{%
  \tcbox@fitalgorithm@areasize@core%
  \pgfmathdivide{\tcb@w@upper}{\tcb@w@upper@temp}%
  \tcbdimto\tcb@fit@@h{\pgfmathresult\dimexpr\tcb@fit@@h}%
  \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
    \let\tcb@fit@@h=\tcb@fit@@target%
  \fi
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@h}%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize@star{%
  \tcbox@fitalgorithm@areasize@core%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@squeeze{%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@hybrid@core{%
  \pgfmathdivide{\tcb@fit@@target}{\tcb@fit@@h}%
  \pgfmathsqrt{\pgfmathresult}%
  \tcbfitdim=\pgfmathresult\tcbfitdim%
  \tcb@fit@@box%
  %
  \pgfmathdivide{\tcb@fit@@target}{\tcb@fit@@h}%
  \pgfmathsqrt{\pgfmathresult}%
  \ifdim\dimexpr\pgfmathresult pt<0.85pt\relax
    \tcbfitdim=\pgfmathresult\tcbfitdim%
    \tcb@fit@@box%
  \else\ifdim\dimexpr\pgfmathresult pt>1.15pt\relax
    \tcbfitdim=\pgfmathresult\tcbfitdim%
    \tcb@fit@@box%
  \fi\fi%
}

\def\tcbox@fitalgorithm@hybrid{%
  \tcbox@fitalgorithm@hybrid@core%
  \tcbox@fitalgorithm@areasize%
}

\def\tcbox@fitalgorithm@hybrid@star{%
  \tcbox@fitalgorithm@hybrid@core%
  \tcbox@fitalgorithm@areasize@star%
}

\def\tcb@fit@@box{%
  \iftcb@hasTitle%
    \tcbdimto\tcb@w@title{\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)}%
    \begin{tcb@savebox}{\tcb@titlebox}{\tcb@w@title}\color{tcbcol@title}\kvtcb@fonttitle\kvtcb@haligntitle\kvtcb@before@title\kvtcb@title\kvtcb@after@title\end{tcb@savebox}%
    \tcbdimto\tcb@h@titletotal{\ht\tcb@titlebox+\dp\tcb@titlebox+\kvtcb@title@rule+(\kvtcb@boxsep)*2+\kvtcb@toptitle+\kvtcb@bottomtitle}%
  \else%
    \let\tcb@h@titletotal=\tcb@zpt%
  \fi%
  \tcbdimto\tcb@fit@@line{\kvtcb@fit@skip\tcbfitdim}%
  \tcbdimto\tcb@w@upper{\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@leftupper)-(\kvtcb@rightupper)}%
  \tcb@fit@@boxsave{\tcb@w@upper}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \tcbdimto\tcb@fit@@target{\kvtcb@height@fixed-(\kvtcb@top@rule@stand)-(\kvtcb@bottom@rule@stand)-(\kvtcb@top)-(\kvtcb@bottom)-(\kvtcb@boxsep)*2-\tcb@h@titletotal}%
}%

\long\def\tcbox@inner@fitbox#1{%
  \tcbset{breakable@false,sidebyside=false}%
  \let\tcb@space\tcb@zpt%
  \let\tcb@val@raisebase=\tcb@zpt%
  \unless\ifdefined\kvtcb@height@fixed%
    \tcbset{height=\kvtcb@width}%
  \fi%
  \tcb@hasLowerfalse%
  %
  \count@\z@%
  \tcbfitdim\kvtcb@fit@basedim%
  \tcb@fit@warn@begin%
  %
  \def\tcb@fit@@boxsave##1{%
    \tcbdimto\tcb@innerwidth{\kvtcb@width-\kvtcb@left@rule-\kvtcb@right@rule}%
    \colorlet{tcbcol@origin}{.}%
    \tcb@set@color{tcbcol@upper}%
    \begin{tcb@savebox}{\tcb@upperbox}{##1}%
      \kvtcb@fontupper\fontsize{\tcbfitdim}{\tcb@fit@@line}\selectfont%
%      \kvtcb@halignupper\kvtcb@before@upper\ignorespaces#1\unskip\kvtcb@after@upper%
      \kvtcb@halignupper\kvtcb@before@upper\ignorespaces#1\kvtcb@after@upper%
    \end{tcb@savebox}%
    \tcb@reset@color%
    \advance\count@ 1\relax%
  }%
  %
  \tcb@set@@phantom%
  \tcb@set@@title%
  \tcb@fit@@box%
  %
  % height fit
  \ifdim\kvtcb@height@fixed@plus>0pt\relax%
    \let\tcb@fit@@minheight=\kvtcb@height@fixed%
    \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
      \ifdim\dimexpr\tcb@fit@@h>\dimexpr\tcb@fit@@target+\kvtcb@height@fixed@plus\relax%
        \tcbdimto\kvtcb@height@fixed{\kvtcb@height@fixed+\kvtcb@height@fixed@plus}%
        \tcbdimto\tcb@fit@@target{\tcb@fit@@target+\kvtcb@height@fixed@plus}%
      \else%
        \tcbdimto\kvtcb@height@fixed{\kvtcb@height@fixed+\tcb@fit@@h-\tcb@fit@@target}%
        \let\tcb@fit@@target=\tcb@fit@@h%
      \fi%
    \fi%
  \fi%
  %
  % width fit
  \ifdim\kvtcb@fit@plus@width>0pt\relax%
    \ifnum\count@<\kvtcb@fit@maxstep\relax%
      \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \tcb@lowerfitdim\dimexpr\kvtcb@width\relax%
        \tcb@upperfitdim\dimexpr\kvtcb@width+\kvtcb@fit@plus@width\relax%
        \tcbdimto\kvtcb@width{\tcb@upperfitdim}%
        \tcb@fit@@box%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \else%
          \ifnum\count@<\kvtcb@fit@maxstep\relax%
            \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
            \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
            \loop%
              \tcb@fit@@box%
              \tcb@continuetrue%
              \ifnum\count@<\kvtcb@fit@maxstep\relax%
                \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxwidthdiff\relax%
                  \tcb@continuefalse%
                \else%
                  \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxwidthdiffgap\relax%
                    \ifdim\dimexpr\tcb@fit@@gap<\tcb@fit@@line\relax%
                      \tcb@continuefalse%
                    \fi%
                  \fi%
                \fi%
              \else%
                \tcb@continuefalse%
              \fi%
              \iftcb@continue%
                \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
                  \tcb@lowerfitdim\dimexpr\kvtcb@width\relax%
                  \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
                \else%
                  \tcb@upperfitdim\dimexpr\kvtcb@width\relax%
                  \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
                  \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
                \fi%
              \else%
                \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
                  \tcbdimto\kvtcb@width{\tcb@upperfitdim}%
                  \tcb@fit@@box%
                \fi%
              \fi%
            \iftcb@continue \repeat%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  %
  % (font) fit
  \ifnum\count@<\kvtcb@fit@maxstep\relax%
    \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
    \tcbox@fitalgorithm%
    \fi%
  \fi%
  %
  \tcb@fit@warn@end%
  %
  % last height fit
  \ifdim\kvtcb@height@fixed@plus>0pt\relax%
    \ifdim\dimexpr\tcb@fit@@h<\tcb@fit@@target\relax%
      \tcbdimto\tcb@temp{\kvtcb@height@fixed+\tcb@fit@@h-\tcb@fit@@target}%
      \ifdim\dimexpr\tcb@temp<\tcb@fit@@minheight\relax%
      \else%
        \let\kvtcb@height@fixed=\tcb@temp%
      \fi%
    \fi%
  \fi%
  %
  \edef\tcbfitsteps{\the\count@}%
  \tcb@set@@dimensions%
  \tcb@draw@color@box%
}

\newcommand{\tcboxfit}[2][]{%
  \tcb@ox{capture=fitbox,#1}{#2}%
}

\long\def\tcb@newtcboxfit#1#2{\expandafter\tcb@newcommand\csname#1\endcsname{\tcboxfit[#2,options@for=#1]}}

\long\def\tcb@newtcboxfit@#1[#2]#3{\expandafter\tcb@newcommand\csname#1\endcsname[#2]{\tcboxfit[#3,options@for=#1]}}

\long\def\tcb@newtcboxfit@@#1[#2][#3]#4{\expandafter\tcb@newcommand\csname#1\endcsname[#2][#3]{\tcboxfit[#4,options@for=#1]}}

\long\def\tcb@new@tcboxfit@#1[#2]{%
  \@ifnextchar[{\tcb@newtcboxfit@@{#1}[#2]}{\tcb@newtcboxfit@{#1}[#2]}}

\long\def\tcb@new@tcboxfit#1{%
  \@ifnextchar[{\tcb@new@tcboxfit@{#1}}{\tcb@newtcboxfit{#1}}}

\def\newtcboxfit{%
  \let\tcb@newcommand\newcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcboxfit%
  \tcb@process@newcommand}

\def\renewtcboxfit{%
  \let\tcb@newcommand\renewcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcboxfit%
  \tcb@process@newcommand}

\tcbset{%
  reset@fitting/.style={%
    fit algorithm=fontsize,%
    fit basedim=10pt,fit skip=1.2,
    height plus=0pt,fit width plus=0pt,
    fit maxstep=20,fit maxfontdiff=0.1pt,fit maxfontdiffgap=1pt,
    fit maxwidthdiff=1pt,fit maxwidthdiffgap=10pt,
    fit warning=off
  },
  initialize@reset=reset@fitting,
}



==> tcbhooks.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcbhooks.code.tex: Code for adding hooks
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.94}

\tcbset{%
  before upper app/.code={\appto\kvtcb@before@upper{#1}},%
  before upper pre/.code={\preto\kvtcb@before@upper{#1}},%
  after upper app/.code={\appto\kvtcb@after@upper{#1}},%
  after upper pre/.code={\preto\kvtcb@after@upper{#1}},%
  before lower app/.code={\appto\kvtcb@before@lower{#1}},%
  before lower pre/.code={\preto\kvtcb@before@lower{#1}},%
  after lower app/.code={\appto\kvtcb@after@lower{#1}},%
  after lower pre/.code={\preto\kvtcb@after@lower{#1}},%
  before title app/.code={\appto\kvtcb@before@title{#1}},%
  before title pre/.code={\preto\kvtcb@before@title{#1}},%
  after title app/.code={\appto\kvtcb@after@title{#1}},%
  after title pre/.code={\preto\kvtcb@after@title{#1}},%
  %
  % usable inside the document or in the preamble after setting before / after
  before app/.code={\appto\kvtcb@beforebox{#1}},%
  before pre/.code={\preto\kvtcb@beforebox{#1}},%
  after app/.code={\appto\kvtcb@afterbox{#1}},%
  after pre/.code={\preto\kvtcb@afterbox{#1}},%
  %
  overlay unbroken app/.code={\appto\tcb@overlay@unbroken{#1}},%
  overlay unbroken pre/.code={\preto\tcb@overlay@unbroken{#1}},%
  overlay first app/.code={\appto\tcb@overlay@first{#1}},%
  overlay first pre/.code={\preto\tcb@overlay@first{#1}},%
  overlay middle app/.code={\appto\tcb@overlay@middle{#1}},%
  overlay middle pre/.code={\preto\tcb@overlay@middle{#1}},%
  overlay last app/.code={\appto\tcb@overlay@last{#1}},%
  overlay last pre/.code={\preto\tcb@overlay@last{#1}},%
  %
  overlay app/.style={overlay unbroken app={#1},overlay first app={#1},overlay middle app={#1},overlay last app={#1}},%
  overlay pre/.style={overlay unbroken pre={#1},overlay first pre={#1},overlay middle pre={#1},overlay last pre={#1}},%
  overlay broken app/.style={overlay first app={#1},overlay middle app={#1},overlay last app={#1}},%
  overlay broken pre/.style={overlay first pre={#1},overlay middle pre={#1},overlay last pre={#1}},%
  overlay unbroken and first app/.style={overlay unbroken app={#1},overlay first app={#1}},%
  overlay unbroken and first pre/.style={overlay unbroken pre={#1},overlay first pre={#1}},%
  overlay unbroken and last app/.style={overlay unbroken app={#1},overlay last app={#1}},%
  overlay unbroken and last pre/.style={overlay unbroken pre={#1},overlay last pre={#1}},%
  overlay middle and last app/.style={overlay middle app={#1},overlay last app={#1}},%
  overlay middle and last pre/.style={overlay middle pre={#1},overlay last pre={#1}},%
  overlay first and middle app/.style={overlay first app={#1},overlay middle app={#1}},%
  overlay first and middle pre/.style={overlay first pre={#1},overlay middle pre={#1}},%
  %
  % skins:
  frame code app/.code={\appto\tcb@frame@code{#1}},%
  frame code pre/.code={\preto\tcb@frame@code{#1}},%
  interior titled code app/.code={\appto\tcb@interiortitled@code{#1}},%
  interior titled code pre/.code={\preto\tcb@interiortitled@code{#1}},%
  interior code app/.code={\appto\tcb@interior@code{#1}},%
  interior code pre/.code={\preto\tcb@interior@code{#1}},%
  segmentation code app/.code={\appto\tcb@segmentation@code{#1}},%
  segmentation code pre/.code={\preto\tcb@segmentation@code{#1}},%
  title code app/.code={\appto\tcb@title@code{#1}},%
  title code pre/.code={\preto\tcb@title@code{#1}},%
  %
  extras unbroken pre/.code={\preto\tcb@extras@unbroken{#1}},%
  extras first pre/.code={\preto\tcb@extras@first{#1}},%
  extras middle pre/.code={\preto\tcb@extras@middle{#1}},%
  extras last pre/.code={\preto\tcb@extras@last{#1}},%
  extras pre/.style={extras unbroken pre={#1},extras first pre={#1},extras middle pre={#1},extras last pre={#1}},%
  extras broken pre/.style={extras first pre={#1},extras middle pre={#1},extras last pre={#1}},%
  extras unbroken and first pre/.style={extras unbroken pre={#1},extras first pre={#1}},%
  extras unbroken and last pre/.style={extras unbroken pre={#1},extras last pre={#1}},%
  extras middle and last pre/.style={extras middle pre={#1},extras last pre={#1}},%
  extras first and middle pre/.style={extras first pre={#1},extras middle pre={#1}},%
  %
  underlay unbroken pre/.code={\preto\tcb@underlay@unbroken{#1}},%
  underlay first pre/.code={\preto\tcb@underlay@first{#1}},%
  underlay middle pre/.code={\preto\tcb@underlay@middle{#1}},%
  underlay last pre/.code={\preto\tcb@underlay@last{#1}},%
  underlay boxed title pre/.code={\preto\tcb@underlay@boxedtitle{#1}},%
  underlay pre/.style={underlay unbroken pre={#1},underlay first pre={#1},underlay middle pre={#1},underlay last pre={#1}},%
  underlay broken pre/.style={underlay first pre={#1},underlay middle pre={#1},underlay last pre={#1}},%
  underlay unbroken and first pre/.style={underlay unbroken pre={#1},underlay first pre={#1}},%
  underlay unbroken and last pre/.style={underlay unbroken pre={#1},underlay last pre={#1}},%
  underlay middle and last pre/.style={underlay middle pre={#1},underlay last pre={#1}},%
  underlay first and middle pre/.style={underlay first pre={#1},underlay middle pre={#1}},%
  finish unbroken pre/.code={\preto\tcb@finish@unbroken{#1}},%
  finish first pre/.code={\preto\tcb@finish@first{#1}},%
  finish middle pre/.code={\preto\tcb@finish@middle{#1}},%
  finish last pre/.code={\preto\tcb@finish@last{#1}},%
  finish pre/.style={finish unbroken pre={#1},finish first pre={#1},finish middle pre={#1},finish last pre={#1}},%
  finish broken pre/.style={finish first pre={#1},finish middle pre={#1},finish last pre={#1}},%
  finish unbroken and first pre/.style={finish unbroken pre={#1},finish first pre={#1}},%
  finish unbroken and last pre/.style={finish unbroken pre={#1},finish last pre={#1}},%
  finish middle and last pre/.style={finish middle pre={#1},finish last pre={#1}},%
  finish first and middle pre/.style={finish first pre={#1},finish middle pre={#1}},%
  %
  watermark tikz app/.style={overlay app={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz pre/.style={overlay pre={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark tikz pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark graphics app/.style={overlay app={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics pre/.style={overlay pre={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@graphics{#2}}},
  watermark graphics pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@graphics{#2}}},
  watermark text app/.style={overlay app={\tcb@drawspec@watermark@text{#1}}},
  watermark text pre/.style={overlay pre={\tcb@drawspec@watermark@text{#1}}},
  watermark text app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@text{#2}}},
  watermark text pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@text{#2}}},
}



==> tcblistings.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcblistings.code.tex: Code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.94}

\RequirePackage{listings}[2007/02/22]

\tcbuselibrary{listings@core}

\let\tcb@listing@MakeCaption@org=\lst@MakeCaption

\def\tcb@listing@set@MakeCaption@org{%
  \let\lst@MakeCaption\tcb@listing@MakeCaption@org}
\def\tcb@listing@set@MakeCaption@empty{%
  \lst@HRefStepCounter{lstlisting}%
  \let\lst@MakeCaption\@gobble}

\lstdefinestyle{tcblatex}{language={[LaTeX]TeX},
     aboveskip={0\p@ \@plus 6\p@}, belowskip={0\p@ \@plus 6\p@},
     columns=fullflexible, keepspaces=true,
     breaklines=true, breakatwhitespace=true,
     basicstyle=\ttfamily\small, extendedchars=true, nolol,
     inputencoding=\kvtcb@listingencoding}

\def\tcb@listing@input@listing#1#2{%
  \begingroup%
  \toks@=\expandafter{#1}%
  \edef\tcb@temp{\noexpand\lstinputlisting[nolol,\the\toks@]}%
  \tcb@listing@set@MakeCaption%
  \tcb@temp{#2}%
  \endgroup%
}%


\def\tcb@listing@uselistinglisting{%
  \tcb@listing@input@listing{\kvtcb@listingoptions}{\kvtcb@listingfile}%
}%

\def\tcb@listing@usetemplisting{%
  \tcb@listing@input@listing{\kvtcb@listingoptions}{\kvtcb@tempfile}%
}%

\def\tcb@listing@doc@usetemplisting{%
  \tcb@listing@input@listing{\kvtcb@doclistingoptions}{\kvtcb@tempfile}%
}

\tcbset{%
  listing options/.store in=\kvtcb@listingoptions,%
  listing style/.style={listing options={style=#1}},%
  no listing options/.style={listing options=},%
  listing inputencoding/.store in=\kvtcb@listingencoding,%
  listing remove caption/.is choice,
  listing remove caption/true/.code={\let\tcb@listing@set@MakeCaption\tcb@listing@set@MakeCaption@empty},
  listing remove caption/false/.code={\let\tcb@listing@set@MakeCaption\tcb@listing@set@MakeCaption@org},
  listing remove caption/.default=true,
  listing engine/listings/.code={\let\tcbuselistinglisting\tcb@listing@uselistinglisting%
    \let\tcbusetemplisting\tcb@listing@usetemplisting%
    \let\tcb@doc@usetemplisting\tcb@listing@doc@usetemplisting},
  every listing line/.code={%
    \def\lst@NewLine{%
      \ifx\lst@OutputBox\@gobble\else
          \par\noindent \hbox{}#1%
      \fi
      \global\advance\lst@newlines\m@ne
      \lst@newlinetrue}},%
  every listing line*/.style={every listing line={#1},%
    code={\setbox\z@=\hbox{#1}\tcbdimto\kvtcb@rightupper{\kvtcb@rightupper+\wd\z@}}},%
}


\tcbset{%
  reset@listings/.style={%
    listing style=tcblatex,
    listing inputencoding=\inputencodingname,
    listing remove caption,
    listing engine=listings,
  },
  initialize@reset=reset@listings,
}



==> tcblistingscore.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcblistingscode.code.tex: Auxiliary code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.94}

\def\tcbuselistingtext@input{\input{\kvtcb@listingfile}}%
\def\tcbuselistingtext{\tcbuselistingtext@input}%
\def\tcbuselistingcomment{\kvtcb@listingcomment}%
\def\tcb@listing@listing{\tcbuselistinglisting}

\def\tcb@listing@listingAndOther{%
   \tcbuselistinglisting%
   \tcblower%
   \tcb@use@listing@other%
}

\def\tcb@listing@otherAndListing{%
   \tcb@use@listing@other%
   \tcblower%
   \tcbuselistinglisting%
}

\newenvironment{tcb@lower@outside}[1]{%
  \tcbset{savedelimiter=tcb@lower@outside}\tcb@minipage{#1}%
  \color{tcbcol@lower}\kvtcb@fontlower\kvtcb@halignlower\kvtcb@before@lower\ignorespaces}%
  {\kvtcb@after@lower\endminipage}

\def\tcb@use@listing@other@reset{%
  \tcbset{every box on layer 1/.style={reset,every box}}%
  \tcb@use@listing@other}

\def\tcb@use@lower@outside#1{%
  \setbox\z@=\hbox{\begin{tcb@lower@outside}{#1}%
    \tcb@use@listing@other@reset%
  \end{tcb@lower@outside}}%
  \tcbdimto{\tcb@temp@wd}{\wd\z@}%
  \unhbox\z@%
}

\def\tcb@inputlisting@out@otherAboveListing{%
  {\kvtcb@beforebox}\noindent%
  \iftcb@lowervisible%
    \tcb@use@lower@outside{\kvtcb@width}%
    \par\vskip-\parskip\vspace*{\kvtcb@middle}\noindent%
  \fi%
  \begin{tcolorbox}[before=,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
}

\def\tcb@inputlisting@out@otherAboveListing@Decoupled{%
  \iftcb@lowervisible%
    {\par\tcb@use@listing@other@reset\par}%
  \fi%
  \begin{tcolorbox}[savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
}

\def\tcb@inputlisting@out@listingAboveOther{%
  \begin{tcolorbox}[after=,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \iftcb@lowervisible\par\vskip-\parskip\vspace*{\kvtcb@middle}\noindent%
    \tcb@use@lower@outside{\kvtcb@width}%
  \fi%
  {\kvtcb@afterbox}%
}

\def\tcb@inputlisting@out@listingAboveOther@Decoupled{%
  \begin{tcolorbox}[savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \iftcb@lowervisible%
    {\par\tcb@use@listing@other@reset\par}%
  \fi%
}


\newenvironment{tcb@outside@environment}{%
  \tcb@before@unbroken%
  \begin{minipage}{\tcb@width}}%
{%
  \end{minipage}%
  \tcb@after@unbroken}

\def\tcb@inputlisting@out@prepare{%
  \tcbdimto\tcb@width{\kvtcb@width}%
  \tcbdimto\tcb@innerwidth{\tcb@width-\kvtcb@left@rule-\kvtcb@right@rule}%
  \tcbdimto\tcb@temp{\tcb@innerwidth-\kvtcb@boxsep*2}%
  \tcbdimto\tcb@w@upper{\tcb@temp-\kvtcb@leftupper-\kvtcb@rightupper}%
  \tcbset{breakable@false}%
  \def\tcb@minipage{\csname tcb@minipage@\kvtcb@sbs@align\endcsname}%
  \tcbdimto\tcb@w@upper@real{\tcb@w@upper}%
  \tcbdimto\tcb@w@sbs{\tcb@w@upper@real-\kvtcb@sbs@gap}%
  \tcb@sbs@quota%
  \ifx\kvtcb@float\@empty%
    \let\tcb@before@unbroken=\kvtcb@beforebox%
    \let\tcb@after@unbroken=\kvtcb@afterbox%
  \else%
    \edef\tcb@before@unbroken{\noexpand\tcb@float@env@begin{tcbfloat}[\kvtcb@float]}%
    \let\tcb@after@unbroken=\tcb@float@env@end%
  \fi%
}

\def\tcb@use@lower@outside@side#1{%
  \setbox\z@=\hbox{\begin{tcb@lower@outside}{#1}%
    \tcb@use@listing@other@reset%
  \end{tcb@lower@outside}}%
  \tcb@box@align\z@%
  \tcbdimto{\tcb@temp@wd}{\wd\z@}%
  \unhbox\z@%
}

\def\tcb@inputlisting@out@listingAndOther{%
  \tcb@inputlisting@out@prepare%
  \tcbdimto\tcb@w@outside{\tcb@w@lower}%
  \tcbdimto\tcb@w@inside{\tcb@width-\tcb@w@lower-\kvtcb@sbs@gap}%
  \begin{tcb@outside@environment}%
  \setbox\z@=\hbox{\tcb@minipage{\tcb@w@inside}%
  \begin{tcolorbox}[width=\tcb@w@inside,nobeforeafter,nofloat,sidebyside=false,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \endminipage}%
  \tcb@box@align\z@%
  \unhbox\z@%
  \kern\kvtcb@sbs@gap%
  \iftcb@lowervisible%
    \tcb@use@lower@outside@side{\tcb@w@outside}%
  \fi%
  \end{tcb@outside@environment}%
}

\def\tcb@inputlisting@out@otherAndListing{%
  \tcb@inputlisting@out@prepare%
  \tcbdimto\tcb@w@outside{\tcb@w@upper}%
  \tcbdimto\tcb@w@inside{\tcb@width-\tcb@w@upper-\kvtcb@sbs@gap}%
  \begin{tcb@outside@environment}%
  \iftcb@lowervisible%
    \tcb@use@lower@outside@side{\tcb@w@outside}%
    \tcbdimto{\tcb@temp@wd}{\tcb@w@outside-\tcb@temp@wd+\kvtcb@sbs@gap}%
  \else%
    \tcbdimto{\tcb@temp@wd}{\tcb@w@outside+\kvtcb@sbs@gap}%
  \fi%
  \kern\tcb@temp@wd%
  \setbox\z@=\hbox{\tcb@minipage{\tcb@w@inside}%
  \begin{tcolorbox}[width=\tcb@w@inside,nobeforeafter,nofloat,sidebyside=false,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \endminipage}%
  \tcb@box@align\z@%
  \unhbox\z@%
  \end{tcb@outside@environment}%
}

\def\tcb@inputlisting@inside{%
  \begin{tcolorbox}[capture=\tcb@listing@capture,savedelimiter=tcolorbox]\tcb@listing@process\end{tcolorbox}%
}

\long\def\tcb@run@system@command#1{%
  \ifcase\pdf@shellescape\relax
    \tcb@error{You must invoke LaTeX with the -shell-escape flag}{Pass the -shell-escape flag to LaTeX.}%
  \or\or
    \tcb@warning{System call with restricted shell escape may fail}%
  \fi%
  \ShellEscape{#1}%
  \relax%
}


\tcbset{%
  listing file/.store in=\kvtcb@listingfile,%
  comment/.store in=\kvtcb@listingcomment,%
  listing@process@inside/.code 2 args={%
    \let\tcb@inputlisting\tcb@inputlisting@inside%
    \let\tcb@listing@process=#1%
    \let\tcb@use@listing@other=#2},%
  listing@process@outside/.code 2 args={%
    \let\tcb@inputlisting=#1%
    \let\tcb@use@listing@other=#2},%
  listing only/.style={listing@process@inside={\tcb@listing@listing}{\tcbuselistingtext}},%
  text only/.style={listing@process@inside={\tcbuselistingtext}{\tcbuselistingtext}},%
  comment only/.style={listing@process@inside={\tcbuselistingcomment}{\tcbuselistingcomment}},%
  listing and text/.style={listing@process@inside={\tcb@listing@listingAndOther}{\tcbuselistingtext}},%
  text and listing/.style={listing@process@inside={\tcb@listing@otherAndListing}{\tcbuselistingtext}},%
  text above listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing}{\tcbuselistingtext}},%
  text above* listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing@Decoupled}{\tcbuselistingtext}},%
  listing above text/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther}{\tcbuselistingtext}},%
  listing above* text/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther@Decoupled}{\tcbuselistingtext}},%
  text outside listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAndListing}{\tcbuselistingtext}},%
  listing outside text/.style={listing@process@outside={\tcb@inputlisting@out@listingAndOther}{\tcbuselistingtext}},%
  text side listing/.style={sidebyside,text and listing},%
  listing side text/.style={sidebyside,listing and text},%
  listing and comment/.style={listing@process@inside={\tcb@listing@listingAndOther}{\tcbuselistingcomment}},%
  comment and listing/.style={listing@process@inside={\tcb@listing@otherAndListing}{\tcbuselistingcomment}},%
  comment above listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing}{\tcbuselistingcomment}},%
  comment above* listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing@Decoupled}{\tcbuselistingcomment}},%
  listing above comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther}{\tcbuselistingcomment}},%
  listing above* comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther@Decoupled}{\tcbuselistingcomment}},%
  comment outside listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAndListing}{\tcbuselistingcomment}},%
  listing outside comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAndOther}{\tcbuselistingcomment}},%
  comment side listing/.style={sidebyside,comment and listing},%
  listing side comment/.style={sidebyside,listing and comment},%
  listing engine/.is choice,%
  image comment/.style 2 args={comment={\includegraphics[#1]{#2}}},%
  comment style/.store in=\kvtcb@commentstyle,%
  tcbimage comment/.style={comment={\let\tcb@trans@commentstyle\kvtcb@commentstyle\tcbincludegraphics[code={\pgfkeysalsofrom\tcb@trans@commentstyle}]{#1}}},
  pdf extension/.store in=\kvtcb@pdf@extension,%
  pdf comment/.style={comment={\let\tcb@trans@commentstyle\kvtcb@commentstyle\filename@parse{#1}\edef\tcb@trans@commentfile{\filename@area\filename@base.\kvtcb@pdf@extension}%
    \begin{tcbraster}[raster halign=center,sharp corners,size=tight,colback=white,code={\pgfkeysalsofrom\tcb@trans@commentstyle}]\tcbincludepdf{\tcb@trans@commentfile}\end{tcbraster}}},
  pdf comment/.default={\kvtcb@listingfile},
  process code/.code={\appto\tcb@listing@process@hook{#1}},%
  no process/.code={\def\tcb@listing@process@hook{}},%
  compilable listing/.style={listing file={\jobname-listing-\thetcblistingcount.tex}},
  run system command/.style={process code={\tcb@run@system@command{#1}}},%
  run@system@command/.style 2 args={run system command={#1\space#2\space\filename@area\filename@base}},%
  run pdflatex/.style={run@system@command={pdflatex}{#1}},%
  run xelatex/.style={run@system@command={xelatex}{#1}},%
  run lualatex/.style={run@system@command={lualatex}{#1}},%
  run makeindex/.style={run@system@command={makeindex}{#1}},%
  run bibtex/.style={run@system@command={bibtex}{#1}},%
  run biber/.style={run@system@command={biber}{#1}},%
  run arara/.style={run@system@command={arara}{#1}},%
  run latex/.style={run@system@command={latex}{#1}},%
  run dvips/.style={run@system@command={dvips}{#1}},%
  run ps2pdf/.style={run system command={ps2pdf\space#1\space\filename@area\filename@base.ps}},%
  freeze file/.code={\def\tcbprocess@condition{1}\def\tcbprocess@target{#1}},%
  freeze none/.code={\def\tcbprocess@condition{0}\def\tcbprocess@target{}},%
  freeze extension/.style={freeze file={\filename@area\filename@base#1}},%
  freeze pdf/.style={freeze extension={.pdf}},
  freeze png/.style={freeze extension={.png}},
  freeze jpg/.style={freeze extension={.jpg}},
}

\def\tcb@listing@process@core{%
  \filename@parse{\kvtcb@listingfile}%
  \tcbiffileprocess{\tcbprocess@condition}%
    {\kvtcb@listingfile}{\filename@area\filename@base.md5}{\tcbprocess@target}%
    {\tcb@listing@process@hook}{}%
}

\def\tcbinputlisting@core{%
  \ifdefempty\tcb@listing@process@hook{}{\tcb@listing@process@core}%
  \let\tcb@listing@capture=\kvtcb@capture%
  \tcb@inputlisting%
}

\newcounter{tcblisting}

\newenvironment{tcblisting}[1]{%
  \stepcounter{tcblisting}\edef\thetcblistingcount{\thetcblisting}%
  \tcb@layer@pushup%
  \tcb@apply@box@options{capture=minipage,#1}%
  \begingroup\tcbverbatimwrite{\kvtcb@listingfile}%
}{\endtcbverbatimwrite\endgroup%
  \tcbinputlisting@core%
}

\long\def\tcbinputlisting#1{%
  \begingroup%
  \stepcounter{tcblisting}\edef\thetcblistingcount{\thetcblisting}%
  \tcb@layer@pushup%
  \tcb@apply@box@options{capture=minipage,#1}%
  \tcbinputlisting@core%
  \endgroup%
}

\newenvironment{tcboutputlisting}{%
  \begingroup\tcbverbatimwrite{\kvtcb@listingfile}%
}{\endtcbverbatimwrite\endgroup}

\long\def\tcb@newtcblisting#1#2{\tcb@newenvironment{#1}{\tcblisting{#2,options@for=#1}}{\endtcblisting}}

\long\def\tcb@newtcblisting@#1[#2]#3{\tcb@newenvironment{#1}[#2]{\tcblisting{#3,options@for=#1}}{\endtcblisting}}

\long\def\tcb@newtcblisting@@#1[#2][#3]#4{\tcb@newenvironment{#1}[#2][#3]{\tcblisting{#4,options@for=#1}}{\endtcblisting}}

\long\def\tcb@new@tcblisting@#1[#2]{%
  \@ifnextchar[{\tcb@newtcblisting@@{#1}[#2]}{\tcb@newtcblisting@{#1}[#2]}}

\def\tcb@new@tcblisting#1{%
  \@ifnextchar[{\tcb@new@tcblisting@{#1}}{\tcb@newtcblisting{#1}}}

\def\newtcblisting{%
  \let\tcb@newenvironment\newenvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcblisting%
  \tcb@process@newenvironment}

\def\renewtcblisting{%
  \let\tcb@newenvironment\renewenvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcblisting%
  \tcb@process@newenvironment}

\long\def\tcb@newtcbinputlisting#1#2{\expandafter\tcb@newcommand\csname#1\endcsname{\tcbinputlisting{#2,options@for=#1}}}

\long\def\tcb@newtcbinputlisting@#1[#2]#3{\expandafter\tcb@newcommand\csname#1\endcsname[#2]{\tcbinputlisting{#3,options@for=#1}}}

\long\def\tcb@newtcbinputlisting@@#1[#2][#3]#4{\expandafter\tcb@newcommand\csname#1\endcsname[#2][#3]{\tcbinputlisting{#4,options@for=#1}}}

\long\def\tcb@new@tcbinputlisting@#1[#2]{%
  \@ifnextchar[{\tcb@newtcbinputlisting@@{#1}[#2]}{\tcb@newtcbinputlisting@{#1}[#2]}}

\def\tcb@new@tcbinputlisting#1{%
  \@ifnextchar[{\tcb@new@tcbinputlisting@{#1}}{\tcb@newtcbinputlisting{#1}}}

\def\newtcbinputlisting{%
  \let\tcb@newcommand\newcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcbinputlisting%
  \tcb@process@newcommand}

\def\renewtcbinputlisting{%
  \let\tcb@newcommand\renewcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcbinputlisting%
  \tcb@process@newcommand}

\tcbset{%
  reset@listingscore/.style={%
    listing file=\jobname.listing,
    comment=, listing and text,
    no process,freeze none,
    comment style=,pdf extension=pdf,
  },
  initialize@reset=reset@listingscore,
}



==> tcblistingsutf8.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcblistingsutf8.code.tex: Code for colorboxes with listings in UTF-8
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.94}

\RequirePackage{listingsutf8}[2011/11/10]
\tcbuselibrary{listings}

\tcbset{
  listing utf8/.style={listing inputencoding=utf8/#1},
}

\tcbset{%
  reset@listingsutf8/.style={listing utf8=latin1},
  initialize@reset=reset@listingsutf8,
}



==> tcbmagazine.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcbmagazine.code.tex: Code for box sets and magazine styles
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.94}

\tcbuselibrary{breakable}

\def\newboxarray#1{%
  \ifcsdef{tcb@boxarray@#1@allocated}{%
    \tcb@warning{box array '#1' is allocated again by \string\newboxarray. Memory and registers are wasted}%
  }{}%
  \global\csdef{tcb@boxarray@#1@size}{0}%
  \global\csdef{tcb@boxarray@#1@allocated}{0}%
}

\newboxarray{default}

\newrobustcmd*{\boxarraygetsize}[2][default]{%
  \letcs#2{tcb@boxarray@#1@size}%
  \ifdef{#2}{}{%
    \tcb@error{undefined box array '#1'}%
    {You have to say \string\newboxarray{#1}, before '#1' can be used as box array.}%
  }%
}

\newrobustcmd*{\boxarrayreset}[1][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \global\csdef{tcb@boxarray@#1@size}{0}%
}

\newrobustcmd*{\boxarrayclear}[1][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \global\csdef{tcb@boxarray@#1@size}{0}%
  \letcs\tcb@box@array@allocated{tcb@boxarray@#1@allocated}%
  \begingroup%
    \count@=0%
    \loop%
    \ifnum\count@<\tcb@box@array@allocated\relax%
      \advance\count@ 1\relax%
      \letcs\tcb@box@array@box{tcb@boxarray@#1@\number\count@ @box}%
      \setbox0=\box\tcb@box@array@box%
    \repeat%
  \endgroup%
}

\newrobustcmd*{\boxarraygetbox}[3][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \let#2\@undefined%
  \ifnum\numexpr#3>0\relax%
    \ifnum\numexpr#3>\tcb@box@array@size\relax%
    \else%
      \letcs#2{tcb@boxarray@#1@#3@box}%
    \fi%
  \fi%
}

\newrobustcmd*{\boxarraygetwidth}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\wd\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygetheight}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\ht\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygetdepth}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\dp\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygettotalheight}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\ht\tcb@box@array@box+\dp\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\useboxarray}[2][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \usebox{\tcb@box@array@box}%
  \fi%
}

\newrobustcmd{\usetcboxarray}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \tcbox[#3]{\usebox{\tcb@box@array@box}}%
  \fi%
}

\newrobustcmd*{\consumeboxarray}[2][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \leavevmode\box\tcb@box@array@box\relax%
  \fi%
}

\newrobustcmd{\consumetcboxarray}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \tcbox[#3]{\leavevmode\box\tcb@box@array@box\relax}%
  \fi%
}

\def\boxarraystore#1{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \numdef\tcb@box@array@size{\tcb@box@array@size+1}%
  \global\cslet{tcb@boxarray@#1@size}{\tcb@box@array@size}%
  \letcs\tcb@box@array@allocated{tcb@boxarray@#1@allocated}%
  \ifnum\tcb@box@array@allocated<\tcb@box@array@size\relax%
    \newbox\tcb@box@array@box\csxdef{tcb@boxarray@#1@\tcb@box@array@size @box}{\the\tcb@box@array@box}%
    \global\cslet{tcb@boxarray@#1@allocated}{\tcb@box@array@size}%
  \else%
    \letcs\tcb@box@array@box{tcb@boxarray@#1@\tcb@box@array@size @box}%
  \fi%
  \edef\reserved@a{%
    \endgroup
    \global\setbox\tcb@box@array@box\hbox{%
      \begingroup\aftergroup}%
        \def\noexpand\@currenvir{\@currenvir}%
        \def\noexpand\@currenvline{\on@line}}%
  \reserved@a
    \@endpefalse
    \color@setgroup
      \ignorespaces}

\def\endboxarraystore{\unskip\color@endgroup}

\def\tcb@storetoboxarray@begin#1#2[#3]{\begin{boxarraystore}{#1}}
\def\tcb@storetoboxarray@end{\end{boxarraystore}}

\tcbset{
  store to box array/.code={%
    \def\kvtcb@float{S}\def\tcb@float@env@begin{\tcb@storetoboxarray@begin{#1}}\def\tcb@float@env@end{\tcb@storetoboxarray@end}},
  store to box array/.default=default,
  reset box array/.code={\boxarrayreset[#1]},
  reset box array/.default=default,
  reset and store to box array/.style={reset box array={#1},store to box array={#1}},%
  reset and store to box array/.default=default,
  do not store to box array/.style={nofloat},
}



==> tcbminted.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcbminted.code.tex: Code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.94}

\RequirePackage{minted}[2011/09/17]

\tcbuselibrary{listings@core}

\def\tcb@minted@input@listing#1#2#3#4{%
  \edef\temp@a{#4}%
  \ifx\temp@a\@empty%
  \else%
    \toks@=\expandafter{#4}%
    \edef\tcb@temp{\noexpand\usemintedstyle{\the\toks@}}%
    \tcb@temp%
  \fi%
  \toks@=\expandafter{#1}%
  \edef\tcb@temp{\noexpand\inputminted[\the\toks@]}%
  \tcb@temp{#2}{\minted@outputdir#3}%
}

\def\tcb@minted@uselistinglisting{%
  \tcb@minted@input@listing{\kvtcb@minted@options}{\kvtcb@minted@language}{\kvtcb@listingfile}{\kvtcb@minted@style}%
}%

\def\tcb@minted@usetemplisting{%
  \tcb@minted@input@listing{\kvtcb@minted@options}{\kvtcb@minted@language}{\kvtcb@tempfile}{\kvtcb@minted@style}%
}%

\def\tcb@minted@doc@usetemplisting{%
  \tcb@minted@input@listing{\kvtcb@docmintoptions}{latex}{\kvtcb@tempfile}{\kvtcb@docmintstyle}%
}

\tcbset{%
  minted language/.store in=\kvtcb@minted@language,
  minted options/.store in=\kvtcb@minted@options,
  minted style/.store in=\kvtcb@minted@style,
  listing engine/minted/.code={\let\tcbuselistinglisting\tcb@minted@uselistinglisting%
    \let\tcbusetemplisting\tcb@minted@usetemplisting%
    \let\tcb@doc@usetemplisting\tcb@minted@doc@usetemplisting},
}


\tcbset{%
  reset@minted/.style={%
    minted language=latex,
    minted options={tabsize=2,fontsize=\small},
    minted style=,
    listing engine=minted,
  },
  initialize@reset=reset@minted,
}



==> tcbraster.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcbskinsjigsaw.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.94}

\newcounter{tcbrastercolumn}
\newcounter{tcbrasterrow}
\newcounter{tcbraster}

\newrobustcmd{\thetcbrasternum}{\the\numexpr(\c@tcbrasterrow-1)*\kvtcb@raster@columns+\c@tcbrastercolumn\relax}

\def\tcb@raster@ehg@all{%
  \tcbset{equal height group={\kvtcb@raster@ehgid}}%
}

\def\tcb@raster@ehg@row{%
  \tcbset{equal height group={\kvtcb@raster@ehgid @\number\c@tcbrasterrow}}%
}


\tcbset{%
  raster columns/.store in=\kvtcb@raster@columns,
  raster rows/.store in=\kvtcb@raster@rows,
  raster width/.store in=\kvtcb@raster@width,
  raster height/.store in=\kvtcb@raster@height,
  %
  raster before skip/.store in=\kvtcb@raster@skip@before,
  raster after skip/.store in=\kvtcb@raster@skip@after,
  raster left skip/.store in=\kvtcb@raster@skip@left,
  raster right skip/.store in=\kvtcb@raster@skip@right,
  %
  raster column skip/.store in=\kvtcb@raster@xskip,
  raster row skip/.store in=\kvtcb@raster@yskip,
  %
  raster equal skip/.style={raster before skip=#1,raster after skip=#1,
    raster column skip=#1,raster row skip=#1},
  %
  raster@halign/.store in=\kvtcb@raster@halign,
  raster halign/.is choice,
  raster halign/center/.style={raster@halign=\centering},
  raster halign/left/.style={raster@halign=\raggedright},
  raster halign/right/.style={raster@halign=\raggedleft},
  %
  raster valign/.store in=\kvtcb@raster@valign,
  %
  raster equal height group/.store in=\kvtcb@raster@ehgid,%
  raster equal height/.is choice,
  raster equal height/.default=all,
  raster equal height/none/.code={\let\tcb@raster@ehg@start\@empty%
    \let\tcb@raster@ehg@continue\@empty},%
  raster equal height/rows/.code={\let\tcb@raster@ehg@start\tcb@raster@ehg@row%
    \let\tcb@raster@ehg@continue\tcb@raster@ehg@row},%
  raster equal height/all/.code={\let\tcb@raster@ehg@start\tcb@raster@ehg@all%
    \let\tcb@raster@ehg@continue\@empty},%
  %
  raster force size/.is choice,%
  raster force size/.default=true,%
  raster force size/true/.code={\let\tcb@raster@set@size\tcbset@late@options},%
  raster force size/false/.code={\let\tcb@raster@set@size\tcbset},%
  raster multicolumn/.code={%
    \ifnum\numexpr\c@tcbrastercolumn+#1>\numexpr\kvtcb@raster@columns+1\relax
      \tcb@warning{'raster multicolumn' combined too much columns}%
    \else%
      \tcbset@late@options{%
        code={\preto\kvtcb@afterbox{\addtocounter{tcbrastercolumn}{\numexpr#1-1}}},
        width=(\tcb@raster@box@width+\kvtcb@raster@xskip)*#1-\kvtcb@raster@xskip}%
    \fi%
  },
  raster multirow/.code={%
    \ifdefined\tcb@raster@box@height%
      \tcbset@late@options{%
        height=(\tcb@raster@box@height+\kvtcb@raster@yskip)*#1-\kvtcb@raster@yskip}%
    \else%
      \tcb@warning{'raster multirow' needs a fixed 'raster height'}%
    \fi%
  },
}

\tcbset{
  raster reset/.style={
    raster width=\linewidth,raster height=0pt,
    raster equal skip=2mm,
    raster columns=2,raster rows=2,
    raster left skip=0pt,raster right skip=0pt,
    raster halign=left,raster valign=center,
    raster equal height=none,
    raster equal height group={REG@\tcb@raster@number},
    raster force size,},
  raster reset
}

\setcounter{tcbraster}{0}

\let\tcb@raster@change@minipage\@empty
\let\tcb@raster@change@fitbox\@empty
\def\tcb@raster@change@hbox{\tcbset{capture=minipage}}

\def\tcb@height@fill@unbroken@raster#1{%
  \ifnum\c@tcblayer<2\relax%
    \kvtcb@beforebox%
    \def\kvtcb@beforebox{}%
    \tcb@breakat@init%
    \tcbset{compress page=#1}%
    \tcb@comp@h@page%
    \ifdim\tcb@h@page<0pt\relax\unkern\pagebreak\tcb@comp@h@page\kern\kvtcb@raster@skip@left\fi%
    \tcbset{height=\tcb@h@page-\kvtcb@bbtop@stand-\kvtcb@bbbottom@stand}%
  \fi%
}

\newenvironment{tcbraster}[1][]{%
  \tcb@layer@pushup%
  \stepcounter{tcbraster}%
  \edef\tcb@raster@number{\number\c@tcbraster}%
  \edef\tcb@raster@save@column{\number\c@tcbrastercolumn}%
  \edef\tcb@raster@save@row{\number\c@tcbrasterrow}%
  \let\tcb@raster@change@fitbox\@empty%
  \setcounter{tcbrastercolumn}{1}%
  \setcounter{tcbrasterrow}{1}%
  \let\tcb@height@fill@unbroken\tcb@height@fill@unbroken@raster%
  \tcbset{every box on layer \the\numexpr\number\c@tcblayer+1\relax/.code={%
    \tcbset{raster every box/.try}%
    \ifodd\c@tcbrastercolumn\relax%
      \tcbset{raster odd column/.try}%
    \else%
      \tcbset{raster even column/.try}%
    \fi%
    \tcbset{raster column \number\c@tcbrastercolumn/.try}%
    \ifodd\c@tcbrasterrow\relax%
      \tcbset{raster odd row/.try}%
    \else%
      \tcbset{raster even row/.try}%
    \fi%
    \tcbset{raster row \number\c@tcbrasterrow/.try}%
    \ifodd\thetcbrasternum\relax%
      \tcbset{raster odd number/.try}%
    \else%
      \tcbset{raster even number/.try}%
    \fi%
    \tcbset{raster row \number\c@tcbrasterrow\space column \number\c@tcbrastercolumn/.try}%
    \tcbset{raster number \thetcbrasternum/.try}%
  }}%
  \tcbset{#1}%
  \tcbset@late@options{%
    before={\ifhmode\unskip\fi\ifnum\c@tcbrastercolumn>1 \kern\kvtcb@raster@xskip\else%
      \ifnum\c@tcbrasterrow>1 \parindent\z@\parskip\z@\par\nointerlineskip\addvspace{\the\dimexpr\kvtcb@raster@yskip\relax}\noindent\fi%
      \kern\kvtcb@raster@skip@left\fi},
    after={%
      \ifnum\c@tcbrastercolumn=\kvtcb@raster@columns\relax%
        \kern\kvtcb@raster@skip@right%
        \setcounter{tcbrastercolumn}{1}\addtocounter{tcbrasterrow}{1}%
        \aftergroup\tcb@raster@ehg@continue%
      \else%
        \stepcounter{tcbrastercolumn}%
      \fi},%
    box align=\kvtcb@raster@valign,%
  }%
  \tcbdimto\tcb@raster@box@width{(\kvtcb@raster@width+\kvtcb@raster@xskip-\kvtcb@raster@skip@left-\kvtcb@raster@skip@right)/\kvtcb@raster@columns-\kvtcb@raster@xskip}%
  \tcb@raster@set@size{%
    code={\csuse{tcb@raster@change@\kvtcb@capture}},
    width=\tcb@raster@box@width,
  }%
  \ifdim\dimexpr\kvtcb@raster@height>0pt\relax%
    \tcbdimto\tcb@raster@box@height{(\kvtcb@raster@height+\kvtcb@raster@yskip-0.001pt)/\kvtcb@raster@rows-\kvtcb@raster@yskip}%
    \tcb@raster@set@size{height=\tcb@raster@box@height}%
  \fi%
  \tcb@raster@ehg@start%
  \let\tcb@end@raster\@empty%
  \ifinner\ifhmode%
    \color@vbox%
    \hsize=\kvtcb@raster@width%
    \let\tcb@end@raster\color@endbox%
  \fi\fi%&
  \if@nobreak%
    \iftcb@ignorenobreak%
      {\par\nointerlineskip%
      \addvspace{\glueexpr\kvtcb@raster@skip@before-\parskip}}%
    \fi%
  \else%
    {\par\nointerlineskip%
    \addvspace{\glueexpr\kvtcb@raster@skip@before-\parskip}}%
  \fi%
  \kvtcb@raster@halign\noindent%
}{%
  \ifhmode\unskip\fi%
  \ifnum\c@tcbrastercolumn>1 %
    \kern\kvtcb@raster@skip@right%
  \fi%
  \begingroup%
  \par\nointerlineskip%
  \addvspace{\glueexpr\kvtcb@raster@skip@after-\parskip}%
  \endgroup%
  \tcb@end@raster%
  \setcounter{tcbrastercolumn}{\tcb@raster@save@column}%
  \setcounter{tcbrasterrow}{\tcb@raster@save@row}%
}

\newcommand{\tcbitem@following}[1][]{%
  \end{tcolorbox}\begin{tcolorbox}[#1]%
}

\newcommand{\tcbitem@first}[1][]{%
  \let\tcbitem=\tcbitem@following%
  \begin{tcolorbox}[#1]%
}

\newenvironment{tcbitemize}[1][]{%
  \begin{tcbraster}[#1]%
  \let\tcb@raster@change@fitbox=\tcb@raster@change@hbox%
  \let\tcbitem=\tcbitem@first%
}{\end{tcolorbox}\end{tcbraster}}

\newenvironment{tcboxedraster}[2][]{%
  \tcolorbox[#2]\tcbraster[#1]}%
  {\endtcbraster\endtcolorbox}

\newenvironment{tcboxeditemize}[2][]{%
  \tcolorbox[#2]\tcbitemize[#1]}%
  {\endtcbitemize\endtcolorbox}


==> tcbskins.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcbskins.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.94}

\RequirePackage{tikz}[2010/10/13]

\newenvironment{tikzpicture@tcb@hooked}{%
  \edef\tcb@tikzpicture@begin{\noexpand\tikzpicture[\expandonce\tcb@tikz@option@hook]}%
  \tcb@tikzpicture@begin\tcb@tikz@begin@hook}{\tcb@tikz@end@hook\endtikzpicture}

\def\tcb@creategeonodes@true{%
  \begin{scope}[every node/.style={line width=0mm,inner sep=0mm,outer sep=0mm,draw=none,fill=none,rectangle}]
    \node[name=frame,at={(0,0)},above right,minimum width=\tcb@width,minimum height=\tcb@height]{};
    \node[name=interior,at={({\kvtcb@left@rule},{\kvtcb@bottom@rule})},above right,minimum width=\tcb@innerwidth,minimum height=\tcb@innerheight]{};
    \ifnum\tcb@segment@state=1%
    \node[name=segmentation,at={({\kvtcb@left@rule},{\the\dimexpr\kvtcb@bottom@rule+\kvtcb@boxsep*2+\tcb@break@bottomsep+\kvtcb@bottom+\tcb@height@lower\relax})},above right,
       minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\kvtcb@middle*2\relax]{};
    \else\iftcb@sidebyside%
    \node[name=segmentation,at={({\the\dimexpr\kvtcb@left@rule+\kvtcb@boxsep+\kvtcb@leftupper+\tcb@w@upper\relax},{\the\dimexpr\kvtcb@bottom@rule\relax})},above right,
       minimum width=\the\dimexpr\kvtcb@sbs@gap\relax,minimum height=\tcb@innerheight]{};
    \fi\fi%
    \iftcb@hasTitle%
    \node[name=title,at={({\kvtcb@left@rule},{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule\relax})},above right,
       minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\tcb@h@title+\kvtcb@toptitle+\kvtcb@bottomtitle+\kvtcb@boxsep*2\relax]{};
    \fi%
    \tcb@specialgeonodes@hook%
  \end{scope}%
}

\def\tcbsettowidthofnode#1#2{%
  \pgfpointanchor{#2}{east}\unskip%
  #1\pgf@x%
  \pgfpointanchor{#2}{west}\unskip%
  \advance #1 by -\pgf@x\relax%
}

\def\tcbsetmacrotowidthofnode#1#2{%
  \tcbsettowidthofnode\pgf@xa{#2}%
  \edef#1{\the\pgf@xa}%
}

\def\tcbsettoheightofnode#1#2{%
  \pgfpointanchor{#2}{north}\unskip%
  #1\pgf@y%
  \pgfpointanchor{#2}{south}\unskip%
  \advance #1 by -\pgf@y\relax%
}

\def\tcbsetmacrotoheightofnode#1#2{%
  \tcbsettoheightofnode\pgf@ya{#2}%
  \edef#1{\the\pgf@ya}%
}

\def\tcb@spec#1{\tikzset{tcb@spec/.style={#1}}}

\def\tcb@gettikzxy#1#2#3{%
  \tikz@scan@one@point\pgfutil@firstofone#1\relax%
  \edef#2{\the\pgf@x}%
  \edef#3{\the\pgf@y}%
}

\def\tcb@boundary@tikzbase#1#2#3#4#5#6{%
  \tcb@gettikzxy{(#1)}{\tcb@xa}{\tcb@ya}%
  \tcb@gettikzxy{(#2)}{\tcb@xb}{\tcb@yb}%
  \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  #4\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
  #5\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  #6\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  #3\pgfpathclose%
}

\def\tcb@pathboundary#1#2{\path[#1]\pgfextra{#2};}

\def\tcb@pathbase#1#2#3#4#5#6#7{\tcb@pathboundary{#1}{\tcb@boundary@tikzbase{#2}{#3}{#4}{#5}{#6}{#7}}}

\def\tcb@boundaryframe@pathfirst{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@zpt}{\tcb@arc@out@NW}{\tcb@arc@out@NE}{\tcb@arc@zpt}%
}

\def\tcb@boundaryframe@pathmiddle{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@boundaryframe@pathlast{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@out@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@out@SE}%
}

\tikzset{%
  tcb fill frame/.style={fill=tcbcol@frame,fill opacity=\kvtcb@opacityframe,tcb@spec,frame@style},%
  tcb fill interior/.style={fill=tcbcol@back,fill opacity=\kvtcb@opacityback,tcb@spec,interior@style},%
  tcb fill title/.style={fill=tcbcol@backtitle,fill opacity=\kvtcb@opacitybacktitle,tcb@spec,title@style},%
}

% fill frame
\def\tcb@drawframe@path{\tcb@pathboundary{tcb fill frame}{\tcb@outerboundary}}
\let\tcb@drawframe@pathfirst=\tcb@drawframe@path
\let\tcb@drawframe@pathmiddle=\tcb@drawframe@path
\let\tcb@drawframe@pathlast=\tcb@drawframe@path


% fill inner box with title
\def\tcb@drawwithtitle@path{\tcb@pathboundary{tcb fill interior}{\tcb@boundaryinterior@title@standard}}

\def\tcb@drawwithtitle@pathfirst{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\let\tcb@drawwithtitle@pathmiddle=\tcb@drawwithtitle@pathfirst

\let\tcb@drawwithtitle@pathlast=\tcb@drawwithtitle@path

% fill inner box without title
\def\tcb@drawwithouttitle@path{\tcb@pathboundary{tcb fill interior}{\tcb@boundaryinterior@notitle@standard}}

\def\tcb@drawwithouttitle@pathfirst{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@ins@NW}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawwithouttitle@pathmiddle{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.east|-frame.north}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawwithouttitle@pathlast{%
  \tcb@pathbase{tcb fill interior}{interior.south west}{interior.east|-frame.north}%
    {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

% draw title box
\def\tcb@drawtitle@path{\tcb@pathboundary{tcb fill title}{\tcb@boundarytitle@standard}}

\let\tcb@drawtitle@pathfirst=\tcb@drawtitle@path

\def\tcb@drawtitle@pathmiddle{%
  \tcb@pathbase{tcb fill title}{title.south west}{title.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\let\tcb@drawtitle@pathlast=\tcb@drawtitle@pathmiddle

% draw segmentation line
\def\tcb@drawlower@path{%
  \iftcb@sidebyside%
    \path[draw=tcbcol@frame,fill opacity=\kvtcb@opacityframe,dash pattern=on 1mm off 1mm,dash phase=0.5mm,tcb@spec,segmentation@style]
    (segmentation.north)--(segmentation.south);%
  \else%
    \path[draw=tcbcol@frame,fill opacity=\kvtcb@opacityframe,dash pattern=on 1mm off 1mm,dash phase=0.5mm,tcb@spec,segmentation@style]
    (segmentation.west)--(segmentation.east);%
  \fi%
}

\def\tcb@draw@pseudo@segmentation#1{%
\begingroup\tcb@shield@externalize\noindent\begin{tikzpicture}%
  \path[use as bounding box] (0,{\the\dimexpr-\kvtcb@middle-\kvtcb@boxsep\relax})
     rectangle (\linewidth,{\the\dimexpr\kvtcb@middle+\kvtcb@boxsep\relax});
  \node[line width=0mm,inner sep=0mm,draw=none,fill=none,rectangle,
        name=segmentation,at={({\the\dimexpr-\kvtcb@boxsep-(#1)\relax},0)},right,%
        minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\kvtcb@middle*2\relax]{};
  \tcb@drawlower@path%
\end{tikzpicture}\endgroup}

\def\tcbline@star#1{%
{\parskip\z@\par\nointerlineskip}%
\xleaders\vbox{\tcb@draw@pseudo@segmentation{#1}}\vskip\dimexpr(\kvtcb@middle+\kvtcb@boxsep)*2\relax%
{\parskip\z@\par\nointerlineskip}}

\def\tcbline@#1{%
{\parskip\z@\par\nointerlineskip}%
\tcb@draw@pseudo@segmentation{#1}%
{\parskip\z@\par\nointerlineskip}}

\def\tcbline{%
  \@ifstar{\iftcb@hasLower\tcbline@star{\kvtcb@leftlower}\else\tcbline@star{\kvtcb@leftupper}\fi}%
  {\iftcb@hasLower\tcbline@{\kvtcb@leftlower+\@totalleftmargin}\else\tcbline@{\kvtcb@leftupper+\@totalleftmargin}\fi}}


% draw special versions
\def\tcb@drawspec@UT{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@UR{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@ins@NW}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@US{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.east|-frame.north}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@LR#1{%
  \tcb@pathbase{#1,segmentation@style}{interior.south west}{[yshift=0.1mm]segmentation.east}%
    {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@LS#1{%
  \tcb@pathbase{#1,segmentation@style}{interior.west|-frame.south}{[yshift=0.1mm]segmentation.east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@A#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@NE}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@sbs@B#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@sbs@C#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@D#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@E#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.east|-frame.north}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@F#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.east|-frame.north}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@T{%
  \tcb@pathbase{top color=tcbcol@frame,bottom color=tcbcol@back,fill opacity=\kvtcb@opacitybacktitle}{[yshift=-0.01pt]interior.north west}{[yshift=0.01pt]title.south east}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawframe@freelance{\tcb@frame@code}
\def\tcb@drawwithtitle@freelance{\tcb@interiortitled@code}
\def\tcb@drawwithouttitle@freelance{\tcb@interior@code}
\def\tcb@drawlower@freelance{\tcb@segmentation@code}
\def\tcb@drawtitle@freelance{\tcb@title@code}


\def\tcb@drawframe@spartan{%
  \begin{pgfscope}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfsetfillcolor{tcbcol@frame}%
  \pgfsetfillopacity{\kvtcb@opacityframe}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawwithtitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight\relax}}%
  \pgfsetfillcolor{tcbcol@back}%
  \pgfsetfillopacity{\kvtcb@opacityback}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawwithouttitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\tcb@height-\kvtcb@top@rule\relax}}%
  \pgfsetfillcolor{tcbcol@back}%
  \pgfsetfillopacity{\kvtcb@opacityback}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawtitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule\relax}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\tcb@height-\kvtcb@top@rule\relax}}%
  \pgfsetfillcolor{tcbcol@backtitle}%
  \pgfsetfillopacity{\kvtcb@opacitybacktitle}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawlower@spartan{%
  \begin{pgfscope}%
  \iftcb@sidebyside%
  \tcbdimto\tcb@seg@pos{\kvtcb@left@rule+\kvtcb@boxsep+\kvtcb@leftupper+\tcb@w@upper+\kvtcb@sbs@gap/2}%
  \pgfpathmoveto{\pgfqpoint{\tcb@seg@pos}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight\relax}}%
  \pgfpathlineto{\pgfqpoint{\tcb@seg@pos}{\kvtcb@bottom@rule}}%
  \else%
  \tcbdimto\tcb@seg@pos{\kvtcb@bottom@rule+\kvtcb@boxsep*2+\tcb@break@bottomsep+\kvtcb@middle+\kvtcb@bottom+\tcb@height@lower}%
  \pgfpathmoveto{\pgfqpoint{\kvtcb@left@rule}{\tcb@seg@pos}}%
  \pgfpathlineto{\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\tcb@seg@pos}}%
  \fi%
  \pgfsetcolor{tcbcol@frame}%
  \pgfsetstrokeopacity{\kvtcb@opacityframe}%
  \pgfusepath{stroke}%
  \end{pgfscope}%
}


\tcbset{%
  frame style/.code={\tikzset{frame@style/.style={#1}}},%
  frame hidden/.style={frame style={draw=none,fill=none}},
  frame engine/path/.style={frame code=\tcb@drawframe@path},
  frame engine/pathfirst/.style={frame code=\tcb@drawframe@pathfirst},
  frame engine/pathmiddle/.style={frame code=\tcb@drawframe@pathmiddle},
  frame engine/pathlast/.style={frame code=\tcb@drawframe@pathlast},
  frame engine/freelance/.style={frame code=\tcb@drawframe@standard},
  frame engine/spartan/.style={frame code=\tcb@drawframe@spartan},
  frame engine/empty/.style={frame code=},
  %
  interior titled engine/path/.style={interior titled code=\tcb@drawwithtitle@path},
  interior titled engine/pathfirst/.style={interior titled code=\tcb@drawwithtitle@pathfirst},
  interior titled engine/pathmiddle/.style={interior titled code=\tcb@drawwithtitle@pathmiddle},
  interior titled engine/pathlast/.style={interior titled code=\tcb@drawwithtitle@pathlast},
  interior titled engine/freelance/.style={interior titled code=\tcb@drawwithtitle@standard},
  interior titled engine/spartan/.style={interior titled code=\tcb@drawwithtitle@spartan},
  interior titled engine/empty/.style={interior titled code=},
  %
  interior engine/path/.style={interior code=\tcb@drawwithouttitle@path},
  interior engine/pathfirst/.style={interior code=\tcb@drawwithouttitle@pathfirst},
  interior engine/pathmiddle/.style={interior code=\tcb@drawwithouttitle@pathmiddle},
  interior engine/pathlast/.style={interior code=\tcb@drawwithouttitle@pathlast},
  interior engine/freelance/.style={interior code=\tcb@drawwithouttitle@standard},
  interior engine/spartan/.style={interior code=\tcb@drawwithouttitle@spartan},
  interior engine/empty/.style={interior code=},
  %
  segmentation engine/path/.style={segmentation code=\tcb@drawlower@path},
  segmentation engine/freelance/.style={segmentation code=\tcb@drawlower@standard},
  segmentation engine/spartan/.style={segmentation code=\tcb@drawlower@spartan},
  segmentation engine/empty/.style={segmentation code=},
  %
  title engine/path/.style={@title code=\tcb@drawtitle@path},
  title engine/pathfirst/.style={@title code=\tcb@drawtitle@pathfirst},
  title engine/pathmiddle/.style={@title code=\tcb@drawtitle@pathmiddle},
  title engine/pathlast/.style={@title code=\tcb@drawtitle@pathlast},
  title engine/freelance/.style={@title code=\tcb@drawtitle@standard},
  title engine/spartan/.style={@title code=\tcb@drawtitle@spartan},
  title engine/empty/.style={@title code=},
  %
  interior style/.code={\tikzset{interior@style/.style={#1}}},%
  interior hidden/.style={interior style={draw=none,fill=none}},
  segmentation style/.code={\tikzset{segmentation@style/.style={#1}}},%
  segmentation hidden/.style={segmentation style={draw=none,fill=none}},
  @title style/.code={\tikzset{title@style/.style={#1}}},%
  title style/.style={title filled,@title style={#1}},
  title hidden/.style={title style={draw=none,fill=none}},
  titlerule style/.style={%
    underlay={\iftcb@hasTitle%
      \path[draw,line width=\kvtcb@title@rule+1000sp,#1]
        ([yshift=-\kvtcb@title@rule/2]title.south west)--([yshift=-\kvtcb@title@rule/2]title.south east);
    \fi}},%
  colbacklower/.colorlet=tcbcol@backlower,%
  clear@spec/.code={\tcb@spec{}},%
  tikz/.code={\appto\tcb@tikz@option@hook{,#1}},%
  tikz reset/.code={\let\tcb@tikz@option@hook\@empty},%
  at begin tikz/.code={\appto\tcb@tikz@begin@hook{#1}},%
  at begin tikz reset/.code={\let\tcb@tikz@begin@hook\@empty},%
  at end tikz/.code={\appto\tcb@tikz@end@hook{#1}},%
  at end tikz reset/.code={\let\tcb@tikz@end@hook\@empty},%
  rotate/.style={tikz={rotate=#1,transform shape}},%
  scale/.style={tikz={scale=#1,transform shape},%
    at begin tikz={%
    \tcbdimto\kvtcb@arc{#1\dimexpr\kvtcb@arc}%
    \tcbdimto\tcb@outer@arc{#1\dimexpr\tcb@outer@arc}%
    \def\tcb@shadow@comp@arc{%
      \tcbdimto\tcb@shadow@ts{#1\dimexpr\tcb@shadow@ts}%
      \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax%
        \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax}%
      \else%
        \let\tcb@shadow@arc=\tcb@zpt%
      \fi%
    }%
    }},%
  remember/.style={tikz={remember picture}},%
  remember as/.style={tikz={remember picture},at end tikz={\pgfnodealias{#1}{frame}}},%
}

\tcbset{%
  base@unbroken/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@standard,%
    shape@of@skin=unbroken,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@unbroken\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@first/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathfirst,%
    shape@of@skin=first,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@first\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@middle/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathmiddle,%
    shape@of@skin=middle,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@middle\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@last/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathlast,%
    shape@of@skin=last,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@last\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
}

\tcb@new@skin{enhanced}{base@unbroken,%
  frame engine=path,interior titled engine=path,interior engine=path,segmentation engine=path,title engine=path,%
  skin first=enhancedfirst,skin middle=enhancedmiddle,skin last=enhancedlast}

\tcb@new@skin{enhancedfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=path,title engine=pathfirst,%
  skin first=enhancedfirst,skin middle=enhancedmiddle,skin last=enhancedmiddle}

\tcb@new@skin{enhancedmiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=path,title engine=pathmiddle,%
  skin first=enhancedmiddle,skin middle=enhancedmiddle,skin last=enhancedmiddle}

\tcb@new@skin{enhancedlast}{base@last,%
  frame engine=pathlast,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=path,title engine=pathlast,%
  skin first=enhancedmiddle,skin middle=enhancedmiddle,skin last=enhancedlast}

\tcbset{enhanced/.style={skin=enhanced},%
  enhanced standard/.style={skin=enhanced,
    skin first=enhanced,skin middle=enhanced,skin last=enhanced},%
  blank/.style={enhanced,frame hidden,interior hidden,segmentation hidden,%
    arc=0pt,outer arc=0pt,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,right=0pt,boxrule=0pt,%
    bottomtitle=6pt,middle=3pt}}

\tcb@new@skin{empty}{base@unbroken,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptyfirst,skin middle=emptymiddle,skin last=emptylast}

\tcb@new@skin{emptyfirst}{base@first,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptyfirst,skin middle=emptymiddle,skin last=emptymiddle}

\tcb@new@skin{emptymiddle}{base@middle,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptymiddle,skin middle=emptymiddle,skin last=emptymiddle}

\tcb@new@skin{emptylast}{base@last,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptymiddle,skin middle=emptymiddle,skin last=emptylast}

\tcbset{empty/.style={skin=empty},%
  blanker/.style={empty,arc=0pt,outer arc=0pt,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,right=0pt,boxrule=0pt,%
    bottomtitle=6pt,middle=3pt},
  blankest/.style={blanker,notitle,
    no shadow,no underlay,no overlay,no finish,no borderline},
  }

\tcb@new@skin{freelance}{base@unbroken,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancefirst,skin middle=freelancemiddle,skin last=freelancelast}%

\tcb@new@skin{freelancefirst}{base@first,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancefirst,skin middle=freelancemiddle,skin last=freelancemiddle}%

\tcb@new@skin{freelancemiddle}{base@middle,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancemiddle,skin middle=freelancemiddle,skin last=freelancemiddle}%

\tcb@new@skin{freelancelast}{base@last,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancemiddle,skin middle=freelancemiddle,skin last=freelancelast}%

\tcbset{freelance/.style={skin=freelance},
  % for backward compatibility:
  extend freelance/.style={#1},%
  extend freelancefirst/.style={skin first is subskin of={freelancefirst}{#1}},%
  extend freelancemiddle/.style={skin middle is subskin of={freelancemiddle}{#1}},%
  extend freelancelast/.style={skin last is subskin of={freelancelast}{#1}}}

\tcb@new@skin{bicolor}{base@unbroken,%
  frame engine=path,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=path,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@path}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@path}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@path}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@path}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@path}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@path}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@B{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@A{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LR{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolorfirst,skin middle=bicolormiddle,skin last=bicolorlast}

\tcbset{bicolor/.style={skin=bicolor}}

\tcb@new@skin{bicolorfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathfirst,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathfirst}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathfirst}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathfirst}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UR%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathfirst}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@D{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@C{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LS{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolorfirst,skin middle=bicolormiddle,skin last=bicolormiddle}

\tcb@new@skin{bicolormiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathmiddle,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathmiddle}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathmiddle}%
    \fi\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathmiddle}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@US%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathmiddle}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@D{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@E{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LS{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolormiddle,skin middle=bicolormiddle,skin last=bicolormiddle}

\tcb@new@skin{bicolorlast}{base@last,%
  frame engine=pathlast,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathlast,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathlast}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathlast}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathlast}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@US%
      \else
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathlast}%
    \fi\tcb@spec{}},%
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@B{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@F{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LR{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolormiddle,skin middle=bicolormiddle,skin last=bicolorlast}

\tcb@new@skin{tile}{skin@bicolor,frame engine=empty,%
  skin first=tilefirst,skin middle=tilemiddle,skin last=tilelast}

\tcbset{tile/.style={skin=tile,boxrule=0pt,sharp corners,title filled,fonttitle=\bfseries}}

\tcb@new@skin{tilefirst}{skin@bicolorfirst,frame engine=empty,%
  skin first=tilefirst,skin middle=tilemiddle,skin last=tilemiddle}

\tcb@new@skin{tilemiddle}{skin@bicolormiddle,frame engine=empty,%
  skin first=tilemiddle,skin middle=tilemiddle,skin last=tilemiddle}

\tcb@new@skin{tilelast}{skin@bicolorlast,frame engine=empty,%
  skin first=tilemiddle,skin middle=tilemiddle,skin last=tilelast}

\tikzset{beamer@color/.style={fill=none,top color=tcbcol@back,bottom color=tcbcol@back!85!black}}

\tcb@new@skin{beamer}{base@unbroken,%
  frame engine=path,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=path,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@path}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@path}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@path}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@path}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LR{beamer@color}\fi\tcb@spec{}},%
  skin first=beamerfirst,skin middle=beamermiddle,skin last=beamerlast}

\tcbset{beamer/.style={skin=beamer,boxrule=0mm,titlerule=1mm,toptitle=0.5mm,arc=2mm,fonttitle=\bfseries,drop fuzzy shadow}}

\tcb@new@skin{beamerfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathfirst,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathfirst}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathfirst}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LS{beamer@color}\fi\tcb@spec{}},%
  skin first=beamerfirst,skin middle=beamermiddle,skin last=beamermiddle}

\tcb@new@skin{beamermiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathmiddle,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathmiddle}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@US%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathmiddle}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LS{beamer@color}\fi\tcb@spec{}},%
  skin first=beamermiddle,skin middle=beamermiddle,skin last=beamermiddle}

\tcb@new@skin{beamerlast}{base@last,%
  frame engine=pathlast,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathlast,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathlast}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@US%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathlast}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LR{beamer@color}\fi\tcb@spec{}},%
  skin first=beamermiddle,skin middle=beamermiddle,skin last=beamerlast}

\def\tcb@drawspec@widgetsegment{%
  \iftcb@sidebyside%
  \tcb@drawlower@path%
  \else%
  \path[left color=tcbcol@frame!75!white,right color=tcbcol@frame!75!white!25!tcbcol@back,segmentation@style]
    ([yshift={-\kvtcb@middle/4}]segmentation.west) rectangle ([yshift={\kvtcb@middle/4}]segmentation.east);
  \fi%
}

\tikzset{widget@color/.style={left color=tcbcol@frame!75!white,right color=tcbcol@frame!75!white!25!tcbcol@back}}

\tcb@new@skin{widget}{base@unbroken,%
  frame engine=path,interior titled engine=path,interior engine=path,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@path}},
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetfirst,skin middle=widgetmiddle,skin last=widgetlast}

\tcbset{widget/.style={skin=widget,arc=0.5mm,fonttitle=\bfseries,titlerule=0mm,toprule at break=0mm}}

\tcb@new@skin{widgetfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathfirst}},%
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetfirst,skin middle=widgetmiddle,skin last=widgetmiddle}

\tcb@new@skin{widgetmiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathmiddle}},%
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetmiddle,skin middle=widgetmiddle,skin last=widgetmiddle}

\tcb@new@skin{widgetlast}{base@last,%
  frame engine=pathlast,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathlast}},
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetmiddle,skin middle=widgetmiddle,skin last=widgetlast}

\tcb@new@skin{spartan}{graphical environment=tikzpicture@tcb@hooked,geometry nodes=true,shape@of@skin=unbroken,%
  set@extensions@preframe=,set@extensions@postframe={\tcb@apply@underlay},set@extensions@final=,%
  frame engine=spartan,interior titled engine=spartan,interior engine=spartan,title engine=spartan,segmentation engine=spartan,%
  set@outerboundary=\tcb@boundaryframe@standard,%
  skin first=spartan,skin middle=spartan,skin last=spartan}

\tcbset{spartan/.style={skin=spartan}}

\tcb@new@skin{draft}{clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,shape@of@skin=unbroken,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=path,title empty,%
  segmentation style={draw=black,dashed},
  set@extensions@postframe=,
  set@extensions@final={\tcb@apply@finish},no finish,%
  colupper=black!50!white,collower=black!50!white,coltitle=black!50!white,
  frame code={%
    \path[draw=blue!10!white,double,line width=1pt,dashed] (current bounding box.south west) rectangle (current bounding box.north east);
    {\tcb@spec{fill=black!15!white,draw=black}\tcb@drawframe@path}%
    \iftcb@hasTitle%
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([xshift={\kvtcb@left@rule},yshift={\kvtcb@bottom@rule}]frame.south west) rectangle
        (interior.north east);
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([yshift={\kvtcb@title@rule}]interior.north west) rectangle
        ([xshift={-\kvtcb@right@rule},yshift={-\kvtcb@top@rule}]frame.north east);
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep}]title.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep}]title.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@lefttitle},yshift={\kvtcb@boxsep+\kvtcb@bottomtitle}]title.south west)
         rectangle node[font=\scriptsize] {title: w=\tcb@w@title, h=\tcb@h@title}
        +(\tcb@w@title,\tcb@h@title);
      \path[draw=red,opacity=0.5] (title.south west) rectangle (title.north east);
    \else%
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([xshift={\kvtcb@left@rule},yshift={\kvtcb@bottom@rule}]frame.south west) rectangle
        ([xshift={-\kvtcb@right@rule},yshift={-\kvtcb@top@rule}]frame.north east);
    \fi%
    \ifcase\tcb@segment@state
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftupper},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle node[font=\scriptsize] {upper: w=\tcb@w@upper, h=\tcb@height@upper}
        +(\tcb@w@upper,\tcb@height@upper);
      \iftcb@sidebyside%
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]segmentation.south east)
        rectangle node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@upper}
        +(\tcb@w@lower,\tcb@height@upper);
      \fi%
    \or%
      \ifdim\wd\tcb@upperbox=0pt\relax
        \path[fill=white,draw,dotted]
          ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
          ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \else
        \path[fill=white,draw,dotted]
          ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
          ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep}]segmentation.east);
        \path[fill=white,draw,dotted]
           ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep}]segmentation.west)
           rectangle ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
        \path[fill=green!20!white,draw=green!75!black,dashed]
          ([xshift={\kvtcb@boxsep+\kvtcb@leftupper},yshift={\kvtcb@boxsep}]segmentation.north west)
           rectangle node[font=\scriptsize] {upper: w=\tcb@w@upper, h=\tcb@height@upper}
           +(\tcb@w@upper,\tcb@height@upper);
      \fi%
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftlower},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle  node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@lower}
        +(\tcb@w@lower,\tcb@height@lower);
      \path[draw=red,opacity=0.5] (segmentation.south west) rectangle (segmentation.north east);
    \else
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftlower},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle  node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@lower}
        +(\tcb@w@lower,\tcb@height@lower);
    \fi%
    \path[draw=red,opacity=0.5] (interior.south west) rectangle (interior.north east);
    \path[draw=red,opacity=0.5] (frame.south west) rectangle (frame.north east);
    \node[above,font=\scriptsize,red!50!black] at (interior.south) {interior: w=\tcb@innerwidth, h=\tcb@innerheight};
    \node[above,font=\scriptsize,red!50!black] at (frame.north) {frame: w=\the\dimexpr\tcb@width\relax, h=\tcb@height};
    \path[draw=blue!10!white,double,line width=1pt,dashed,opacity=0.3] (current bounding box.south west) rectangle (current bounding box.north east);
    \pgfsetfillopacity{0.3}
  },
  skin first=draft,skin middle=draft,skin last=draft}

\tcbset{draft/.style={skin=draft}}

\tikzset{%
  tcb@forced@clip/.code={\tikz@addmode{\tikz@mode@cliptrue}\let\tikz@options=\pgfutil@empty},%
  tcb@invclip/.style={clip,insert path={{[reset cm]\pgfextra{%
    \pgfpathmoveto{\pgfqpoint{-16383.99999pt}{-16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{16383.99999pt}{-16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{16383.99999pt}{16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{-16383.99999pt}{16383.99999pt}}%
    \pgfpathclose}}}}%
}%

\def\tcb@clip@frame{\tcb@pathboundary{clip}{\tcb@outerboundary}}

\def\tcb@invclip@frame{\tcb@pathboundary{tcb@invclip}{\tcb@outerboundary}}

\def\tcb@clip@interior{%
  \begingroup%
  \tcbset{interior hidden}%
  \tcb@spec{tcb@forced@clip}%
  \def\tcb@spec##1{}%
  \iftcb@hasTitle%
    \tcb@interiortitled@code%
  \else%
    \tcb@interior@code%
  \fi%
  \endgroup%
}

\def\tcb@clip@title{%
  \begingroup%
  \tcbset{title hidden}%
  \tcb@spec{tcb@forced@clip}%
  \def\tcb@spec##1{}%
    \iftcb@hasTitle%
      \tcb@title@code%
    \fi%
  \endgroup%
}

\newenvironment{tcbclipframe}{\begin{scope}\tcb@clip@frame}{\end{scope}}
\newenvironment{tcbinvclipframe}{\begin{scope}\tcb@invclip@frame}{\end{scope}}
\newenvironment{tcbclipinterior}{\begin{scope}\tcb@clip@interior}{\end{scope}}
\newenvironment{tcbcliptitle}{\begin{scope}\tcb@clip@title}{\end{scope}}

\def\tcb@apply@underlay{\csname tcb@underlay@\tcb@split@state\endcsname}%
\def\tcb@apply@finish{\csname tcb@finish@\tcb@split@state\endcsname}%

\tcbset{%
  underlay unbroken/.code={\appto\tcb@underlay@unbroken{#1}},%
  underlay first/.code={\appto\tcb@underlay@first{#1}},%
  underlay middle/.code={\appto\tcb@underlay@middle{#1}},%
  underlay last/.code={\appto\tcb@underlay@last{#1}},%
  underlay boxed title/.code={\appto\tcb@underlay@boxedtitle{#1}},%
  underlay/.style={underlay unbroken={#1},underlay first={#1},underlay middle={#1},underlay last={#1}},%
  underlay broken/.style={underlay first={#1},underlay middle={#1},underlay last={#1}},%
  underlay unbroken and first/.style={underlay unbroken={#1},underlay first={#1}},%
  underlay unbroken and last/.style={underlay unbroken={#1},underlay last={#1}},%
  underlay middle and last/.style={underlay middle={#1},underlay last={#1}},%
  underlay first and middle/.style={underlay first={#1},underlay middle={#1}},%
  no underlay unbroken/.code={\let\tcb@underlay@unbroken\@empty},%
  no underlay first/.code={\let\tcb@underlay@first\@empty},%
  no underlay middle/.code={\let\tcb@underlay@middle\@empty},%
  no underlay last/.code={\let\tcb@underlay@last\@empty},%
  no underlay boxed title/.code={\let\tcb@underlay@boxedtitle\@empty},%
  no underlay/.style={no underlay unbroken,no underlay first,no underlay middle,no underlay last,no underlay boxed title},%
  finish unbroken/.code={\appto\tcb@finish@unbroken{#1}},%
  finish first/.code={\appto\tcb@finish@first{#1}},%
  finish middle/.code={\appto\tcb@finish@middle{#1}},%
  finish last/.code={\appto\tcb@finish@last{#1}},%
  finish/.style={finish unbroken={#1},finish first={#1},finish middle={#1},finish last={#1}},%
  finish broken/.style={finish first={#1},finish middle={#1},finish last={#1}},%
  finish unbroken and first/.style={finish unbroken={#1},finish first={#1}},%
  finish unbroken and last/.style={finish unbroken={#1},finish last={#1}},%
  finish middle and last/.style={finish middle={#1},finish last={#1}},%
  finish first and middle/.style={finish first={#1},finish middle={#1}},%
  no finish unbroken/.code={\let\tcb@finish@unbroken\@empty},%
  no finish first/.code={\let\tcb@finish@first\@empty},%
  no finish middle/.code={\let\tcb@finish@middle\@empty},%
  no finish last/.code={\let\tcb@finish@last\@empty},%
  no finish/.style={no finish unbroken,no finish first,no finish middle,no finish last},%
}

\def\tcb@trans@set@boxedsize@copy@top{%
  \begingroup\edef\x{\endgroup\noexpand\def\noexpand\tcb@trans@boxedsize{%
    leftrule=\kvtcb@left@rule,rightrule=\kvtcb@right@rule,
    toprule=\kvtcb@top@rule@stand,bottomrule=\kvtcb@title@rule,
    boxsep=\kvtcb@boxsep,leftupper=\kvtcb@lefttitle,rightupper=\kvtcb@righttitle,
    top=\kvtcb@toptitle,bottom=\kvtcb@bottomtitle,arc=\kvtcb@arc,
    sharp corners=south,
  }}\x}%
\def\tcb@trans@set@boxedsize@copy@bottom{%
  \begingroup\edef\x{\endgroup\noexpand\def\noexpand\tcb@trans@boxedsize{%
    leftrule=\kvtcb@left@rule,rightrule=\kvtcb@right@rule,
    toprule=\kvtcb@title@rule,bottomrule=\kvtcb@bottom@rule@stand,
    boxsep=\kvtcb@boxsep,leftupper=\kvtcb@lefttitle,rightupper=\kvtcb@righttitle,
    top=\kvtcb@toptitle,bottom=\kvtcb@bottomtitle,arc=\kvtcb@arc,
    sharp corners=north,
  }}\x}%

\tcbset{%
  boxed title size/.is choice,
  boxed title size/standard/.code={\def\tcb@trans@set@boxedsize##1{\let\tcb@trans@boxedsize\@empty}},
  boxed title size/title/.code={\def\tcb@trans@set@boxedsize##1{\def\tcb@trans@boxedsize{size=title}}},
  boxed title size/copy/.code={\def\tcb@trans@set@boxedsize##1{%
    \ifstrequal{##1}{top}{\tcb@trans@set@boxedsize@copy@top}{\tcb@trans@set@boxedsize@copy@bottom}}},
  before@boxed@title/.store in=\kvtcb@before@boxedtitle,%
  after@boxed@title/.store in=\kvtcb@after@boxedtitle,%
  boxed title style/.code={\appto\kvtcb@style@boxedtitle{,#1}},%
  no boxed title style/.code={\let\kvtcb@style@boxedtitle\@empty},%
  %
  varwidth boxed title/.style={before@boxed@title={\tcbdimto\tcb@w@title{#1}\begin{varwidth}{\tcb@w@title}},after@boxed@title={\end{varwidth}}},%
  varwidth boxed title/.default={\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)},
  varwidth boxed title*/.style={varwidth boxed title={\kvtcb@width+#1}},
  varwidth boxed title*/.default={0pt-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)},
  %
  minipage boxed title/.style={before@boxed@title={\tcbdimto\tcb@w@title{#1}\begin{minipage}{\tcb@w@title}},after@boxed@title={\end{minipage}}},%
  minipage boxed title/.default={\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)},
  minipage boxed title*/.style={minipage boxed title={\kvtcb@width+#1}},
  minipage boxed title*/.default={0pt-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)},
  %
  tikznode boxed title/.style={before@boxed@title={\centering\tcb@shield@externalize\begin{tikzpicture}\node[align=center,inner sep=0pt,outer sep=0pt,#1]\bgroup},after@boxed@title={\egroup;\end{tikzpicture}}},%
  hbox boxed title/.style={before@boxed@title=,after@boxed@title=},%
  %
  boxtitle/xshift/.dimstore in=\kvtcb@xshift@boxedtitle,%
  boxtitle/yshift/.dimstore in=\kvtcb@yshift@boxedtitle,%
  boxtitle/yshifttext/.dimstore in=\kvtcb@yinnershift@boxedtitle,%
  %
  boxtitle/yshift*@top/.style={yshift*/.code={%
    \tcbdimto\kvtcb@yshift@boxedtitle{##1}%
    \tcbdimto\kvtcb@yinnershift@boxedtitle{\kvtcb@yshift@boxedtitle+\kvtcb@top@rule@stand}%
    \ifdim\dimexpr\kvtcb@yinnershift@boxedtitle>0pt\relax\let\kvtcb@yinnershift@boxedtitle\tcb@zpt\fi%
  }},
  boxtitle/yshift*@bottom/.style={yshift*/.code={%
    \tcbdimto\kvtcb@yshift@boxedtitle{##1}%
    \tcbdimto\kvtcb@yinnershift@boxedtitle{\kvtcb@yshift@boxedtitle-\kvtcb@bottom@rule@stand}%
    \ifdim\dimexpr\kvtcb@yinnershift@boxedtitle<0pt\relax\let\kvtcb@yinnershift@boxedtitle\tcb@zpt\fi%
  }},
  boxtitle/adapt@top/.code={%
    \ifdim\dimexpr\tcboxedtitleheight+\kvtcb@yshift@boxedtitle>0pt\relax
      \tcbdimto\kvtcb@bbtop@stand{\kvtcb@bbtop@stand+\tcboxedtitleheight+\kvtcb@yshift@boxedtitle}%
    \fi%
    \tcbdimto\kvtcb@top{\kvtcb@top-\kvtcb@yinnershift@boxedtitle}%
  },
  boxtitle/adapt@bottom/.code={%
    \ifdim\dimexpr\tcboxedtitleheight-\kvtcb@yshift@boxedtitle>0pt\relax
      \tcbdimto\kvtcb@bbbottom@stand{\kvtcb@bbbottom@stand+\tcboxedtitleheight-\kvtcb@yshift@boxedtitle}%
    \fi%
    \tcbdimto\kvtcb@bottom{\kvtcb@bottom+\kvtcb@yinnershift@boxedtitle}%
  },
  attach@title@boxed/.style n args={5}{%
    detach title,
    code={\def\tcb@specialtitle@hook{%
      \ifx\tcbtitletext\@empty\else%
      \tcb@trans@set@boxedsize{#2}%
      \colorlet{tcbtranscol@frame}{tcbcol@frame}%
      \colorlet{tcbtranscol@back}{tcbcol@backtitle}%
      \let\tcb@trans@skin@current\kvtcb@skin@current%
      \let\tcb@trans@boxedstyle\kvtcb@style@boxedtitle%
      \setbox\tcb@titlebox\color@hbox\bgroup\color{tcbcol@title}\kvtcb@fonttitle\kvtcb@before@boxedtitle\kvtcb@haligntitle\kvtcb@before@title\tcbtitletext\kvtcb@after@title\kvtcb@after@boxedtitle\egroup\color@endbox%
      \setbox\tcb@titlebox\color@hbox\tcbox[skin=\tcb@trans@skin@current,colframe=tcbtranscol@frame,colback=tcbtranscol@back,%
        code={\pgfkeysalsofrom\tcb@trans@boxedsize\pgfkeysalsofrom\tcb@trans@boxedstyle}]{\box\tcb@titlebox}\color@endbox%
      %
      \tcbdimto\tcboxedtitleheight{\ht\tcb@titlebox+\dp\tcb@titlebox}%
      \tcbdimto\tcboxedtitlewidth{\wd\tcb@titlebox}%
      \tcbset{boxtitle/.cd,xshift=0pt,yshift=0pt,yshifttext=0pt,yshift*@#2,#1,adapt@#2}%
      \let\tcb@specialgeonodes@first\relax%
      \let\tcb@specialgeonodes@middle\relax%
      \let\tcb@specialgeonodes@last\relax%
      \def\tcb@specialgeonodes@unbroken{%
        \node[#4,name=title,at={([xshift=\kvtcb@xshift@boxedtitle,yshift=\kvtcb@yshift@boxedtitle]frame.#5)},
                minimum width=\tcboxedtitlewidth,minimum height=\tcboxedtitleheight]{};}%
      \cslet{tcb@specialgeonodes@#3}{\tcb@specialgeonodes@unbroken}%
      \def\tcb@specialgeonodes@hook{\csname tcb@specialgeonodes@\tcb@split@state\endcsname}%
      \preto\tcb@underlay@unbroken{\tcb@underlay@boxedtitle\pgftext[at={\pgfpointanchor{title}{center}}]{\box\tcb@titlebox}}%
      \cspreto{tcb@underlay@#3}{\tcb@underlay@boxedtitle\pgftext[at={\pgfpointanchor{title}{center}}]{\box\tcb@titlebox}}%
      \fi}}%
    },
  attach@title@boxed@top/.style n args={3}{attach@title@boxed={#1}{top}{first}{#2}{#3}},%
  attach@title@boxed@bottom/.style n args={3}{attach@title@boxed={#1}{bottom}{last}{#2}{#3}},%
  %
  attach boxed title to top left/.style={attach@title@boxed@top={#1}{above right}{north west}},
  attach boxed title to top center/.style={attach@title@boxed@top={#1}{above}{north}},
  attach boxed title to top right/.style={attach@title@boxed@top={#1}{above left}{north east}},
  attach boxed title to bottom left/.style={attach@title@boxed@bottom={#1}{below right}{south west}},
  attach boxed title to bottom center/.style={attach@title@boxed@bottom={#1}{below}{south}},
  attach boxed title to bottom right/.style={attach@title@boxed@bottom={#1}{below left}{south east}},
  reduce@vertical@rules/.code={%
    \ifdim\dimexpr\kvtcb@left@rule<\dimexpr\kvtcb@right@rule\relax%
      \tcbdimto\tcb@temp{\kvtcb@left@rule/2}%
    \else%
      \tcbdimto\tcb@temp{\kvtcb@right@rule/2}%
    \fi%
    \tcbset{leftrule/.expanded=\the\dimexpr\kvtcb@left@rule-\tcb@temp\relax,
      rightrule/.expanded=\the\dimexpr\kvtcb@right@rule-\tcb@temp\relax}%
  },
  attach boxed title to bottom/.style={%
    attach boxed title to bottom center={yshift*=\tcboxedtitleheight,#1},
    minipage boxed title,boxed title size=copy,
  },
  attach boxed title to bottom*/.style={%
    attach boxed title to bottom={#1},
    boxed title style={reduce@vertical@rules},
  },
  attach boxed title to top/.style={%
    attach boxed title to top center={yshift*=-\tcboxedtitleheight,#1},
    minipage boxed title,boxed title size=copy,
  },
  attach boxed title to top*/.style={%
    attach boxed title to top={#1},
    boxed title style={reduce@vertical@rules},
  },
  flip title/.style={attach boxed title to bottom,
    boxed title style={reduce@vertical@rules,#1}},
}


\newbox\tcb@waterbox

\def\tcb@setratio#1#2#3{\edef#1{\strip@pt\dimexpr\number\numexpr\number\dimexpr#2\relax*65536/\number\dimexpr#3\relax\relax sp\relax}}

\def\tcb@setratiorobust#1#2#3{\ifdim\dimexpr#3<1pt\tcb@setratio#1{#2}{1pt}\else\tcb@setratio#1{#2}{#3}\fi}

\def\tcb@comp@waterbox@stretch#1#2#3{%
  \tcb@setratiorobust\tcb@scale@x{#1\dimexpr#2}{\wd\tcb@waterbox}%
  \tcb@setratiorobust\tcb@scale@y{#1\dimexpr#3}{\ht\tcb@waterbox+\dp\tcb@waterbox}%
}

\def\tcb@comp@waterbox@zoom#1#2#3{%
  \tcb@comp@waterbox@stretch{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax<\dimexpr\tcb@scale@y pt\relax\let\tcb@scale@y=\tcb@scale@x\else\let\tcb@scale@x=\tcb@scale@y\fi%
}

\def\tcb@comp@waterbox@overzoom#1#2#3{%
  \tcb@comp@waterbox@stretch{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax>\dimexpr\tcb@scale@y pt\relax\let\tcb@scale@y=\tcb@scale@x\else\let\tcb@scale@x=\tcb@scale@y\fi%
}

\def\tcb@comp@waterbox@shrink#1#2#3{%
  \tcb@comp@waterbox@zoom{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax>1pt\relax%
    \edef\tcb@scale@x{1}\edef\tcb@scale@y{1}%
  \fi%
}

\def\tcb@box@scaled@waterbox{\scalebox{\tcb@scale@x}[\tcb@scale@y]{\box\tcb@waterbox}}

\def\tcb@drawspec@watermark@@noclip{%
  \tcb@comp@wm%
  \node[opacity=\kvtcb@watermark@opacity,anchor=center] at (interior) {\tcb@box@scaled@waterbox};%
}

\def\tcb@drawspec@watermark@@clip{%
  \begin{tcbclipinterior}%
  \tcb@drawspec@watermark@@noclip%
  \end{tcbclipinterior}%
}

\def\tcb@drawspec@watermark@tikz#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\pgfsetbaseline{0pt}\begin{tikzpicture}[color=\kvtcb@watermark@color]#1\end{tikzpicture}}\endpgfinterruptpicture\color@endbox%
  \tcb@drawspec@watermark%
}

\def\tcb@drawspec@watermark@graphics#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\includegraphics{#1}}\endpgfinterruptpicture\color@endbox%
  \tcb@drawspec@watermark%
}

\def\tcb@drawspec@watermark@text#1{%
  \tcb@drawspec@watermark@tikz{\node[inner sep=0pt,align=flush center]{#1};}%
}


\tcbset{%
  watermark opacity/.store in=\kvtcb@watermark@opacity,%
  watermark color/.store in=\kvtcb@watermark@color,%
%
  watermark stretch/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@stretch{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark zoom/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@zoom{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark overzoom/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@overzoom{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark shrink/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@shrink{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
%
  watermark tikz/.style={overlay={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark graphics/.style={overlay={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@graphics{#2}}},
  watermark text/.style={overlay={\tcb@drawspec@watermark@text{#1}}},
  watermark text on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@text{#2}}},
  no watermark/.style={no overlay},
  clip watermark/.is choice,
  clip watermark/true/.code={\let\tcb@drawspec@watermark=\tcb@drawspec@watermark@@clip},
  clip watermark/false/.code={\let\tcb@drawspec@watermark=\tcb@drawspec@watermark@@noclip},
  clip watermark/.default=true,
  show bounding box/.style={border@line app={%
    \path[preaction={draw,line width=0.1pt,#1},draw,double=white,line width=1pt,dashed,opacity=0.5,#1]
    (current bounding box.south west) rectangle (current bounding box.north east);}},%
  show bounding box/.default={red},%
}

\def\tcb@tdraw@title@clip{%
  \begin{tcbcliptitle}%
  \tcb@tdraw@title@core%
  \end{tcbcliptitle}%
}

\def\tcb@tdraw@upper@clip{%
  \begin{tcbclipinterior}%
  \tcb@tdraw@upper@core%
  \end{tcbclipinterior}%
}

\def\tcb@tdraw@lower@clip{%
  \begin{tcbclipinterior}%
  \tcb@tdraw@lower@core%
  \end{tcbclipinterior}%
}


\def\tcb@process@ppbb{%
  \pgf@process{\pgfpointanchor{path picture bounding box}{south west}}%
  \pgf@xa\pgf@x\pgf@ya\pgf@y%
  \pgf@process{\pgfpointanchor{path picture bounding box}{north east}}%
  \pgf@xb\pgf@x\pgf@yb\pgf@y%
  \pgfsetfillopacity{\tcb@tikz@fill@graphics@opacity}%
  \pgfsetstrokeopacity{\tcb@tikz@fill@graphics@opacity}%
}

\def\tcb@process@ppbb@wh{%
  \tcb@process@ppbb%
  \tcbdimto\tcb@ppbb@width{\pgf@xb-\pgf@xa}%
  \tcbdimto\tcb@ppbb@height{\pgf@yb-\pgf@ya}%
}

\def\tcb@set@waterbox@to@graphics#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options]{#1}}\endpgfinterruptpicture\color@endbox%
}

\def\tcb@set@waterbox@to@picture#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\pgfsetbaseline{0pt}\begin{tikzpicture}#1\end{tikzpicture}}\endpgfinterruptpicture\color@endbox%
}

\tikzset{%
  fill image opacity/.store in=\tcb@tikz@fill@graphics@opacity,%
  fill image opacity=1,%
  fill image scale/.store in=\tcb@tikz@fill@graphics@scale,%
  fill image scale=1,%
  fill image options/.store in=\tcb@tikz@fill@graphics@options,%
  fill image options=,%
  fill plain image/.style={path picture={%
    \node at (path picture bounding box.center) {\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options]{#1}};
  }},
  fill plain picture/.style={path picture={%
    \tcb@set@waterbox@to@picture{#1}%
    \node at (path picture bounding box.center) {\box\tcb@waterbox};
  }},
  fill stretch image/.style={path picture={%
    \tcb@process@ppbb@wh%
    \node at (path picture bounding box.center) {\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options,%
      width=\the\dimexpr\tcb@tikz@fill@graphics@scale\dimexpr\tcb@ppbb@width\relax,%
      height=\the\dimexpr\tcb@tikz@fill@graphics@scale\dimexpr\tcb@ppbb@height\relax]{#1}};
  }},
  fill stretch picture/.style={path picture={%
    \tcb@process@ppbb@wh%
    \tcb@set@waterbox@to@picture{#1}%
    \tcb@comp@waterbox@stretch{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill@overzoom/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@overzoom{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill overzoom image/.style={fill@overzoom={\tcb@set@waterbox@to@graphics{#1}}},%
  fill overzoom picture/.style={fill@overzoom={\tcb@set@waterbox@to@picture{#1}}},%
  fill@zoom/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@zoom{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill zoom image/.style={fill@zoom={\tcb@set@waterbox@to@graphics{#1}}},%
  fill zoom picture/.style={fill@zoom={\tcb@set@waterbox@to@picture{#1}}},%
  fill@shrink/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@shrink{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill shrink image/.style={fill@shrink={\tcb@set@waterbox@to@graphics{#1}}},%
  fill shrink picture/.style={fill@shrink={\tcb@set@waterbox@to@picture{#1}}},%
  fill@tile/.style={path picture={%
    \tcb@process@ppbb%
    #1%
    \tcbdimto\tcb@ppbb@tilew{\wd\tcb@waterbox}%
    \tcbdimto\tcb@ppbb@tileh{\ht\tcb@waterbox+\dp\tcb@waterbox}%
    \pgf@xc\pgf@xa\pgf@yc\pgf@yb%
    \pgfutil@loop%
      \pgfutil@loop%
        \pgftext[x=\pgf@xc,y=\pgf@yc,left,top]{\copy\tcb@waterbox}%
        \ifdim\pgf@xc<\pgf@xb%
        \advance\pgf@xc\tcb@ppbb@tilew%
      \pgfutil@repeat%
      \ifdim\pgf@yc>\pgf@ya%
      \advance\pgf@yc-\tcb@ppbb@tileh%
      \pgf@xc\pgf@xa%
    \pgfutil@repeat%
  }},%
  fill tile image/.style={fill@tile={\tcb@set@waterbox@to@graphics{#1}}},%
  fill tile picture/.style={fill@tile={\tcb@set@waterbox@to@picture{#1}}},%
  fill tile picture*/.style 2 args={fill@tile={\tcb@set@waterbox@to@picture{#2}%
    \setbox\tcb@waterbox=\color@hbox\scalebox{#1}{\box\tcb@waterbox}\color@endbox}},%
  %
  fill plain image*/.style 2 args={fill image options={#1},fill plain image={#2}},%
  fill stretch image*/.style 2 args={fill image options={#1},fill stretch image={#2}},%
  fill overzoom image*/.style 2 args={fill image options={#1},fill overzoom image={#2}},%
  fill zoom image*/.style 2 args={fill image options={#1},fill zoom image={#2}},%
  fill shrink image*/.style 2 args={fill image options={#1},fill shrink image={#2}},%
  fill tile image*/.style 2 args={fill image options={#1},fill tile image={#2}},%
}

\tcbset{%
  frame style image/.style={frame style={fill=none,fill stretch image={#1}}},
  frame style tile/.style 2 args={frame style={fill=none,fill tile image*={#1}{#2}}},
  interior style image/.style={interior style={fill=none,fill stretch image={#1}}},
  interior style tile/.style 2 args={interior style={fill=none,fill tile image*={#1}{#2}}},
  title style image/.style={title style={fill=none,fill stretch image={#1}}},
  title style tile/.style 2 args={title style={fill=none,fill tile image*={#1}{#2}}},
}

\tcbset{%
  clip title/.is choice,
  clip title/true/.code={\let\tcb@tdraw@title=\tcb@tdraw@title@clip},
  clip title/false/.code={\let\tcb@tdraw@title=\tcb@tdraw@title@core},
  clip title/.default=true,
  clip upper/.is choice,
  clip upper/true/.code={\let\tcb@tdraw@upper=\tcb@tdraw@upper@clip},
  clip upper/false/.code={\let\tcb@tdraw@upper=\tcb@tdraw@upper@core},
  clip upper/.default=true,
  clip lower/.is choice,
  clip lower/true/.code={\let\tcb@tdraw@lower=\tcb@tdraw@lower@clip},
  clip lower/false/.code={\let\tcb@tdraw@lower=\tcb@tdraw@lower@core},
  clip lower/.default=true,
}


\tcbset{marker/.style={%
  skin=enhancedmiddle jigsaw,
  breakable,parbox=false,
  boxrule=0mm,leftrule=5mm,rightrule=5mm,boxsep=0mm,
  left=3mm,right=3mm,top=1mm,bottom=1mm,
  toptitle=1mm,bottomtitle=1mm,fonttitle=\bfseries,
  arc=0mm,outer arc=0mm,
  colback=yellow!10!white,colframe=red,
  watermark color=yellow!75!red!25!white,
  enlarge left by=-8mm,
  enlarge right by=-8mm,
  enlarge top by=0mm,
  enlarge bottom by=0mm,
  width=\the\dimexpr\linewidth+1.6cm\relax,
  frame style={top color=tcbcol@frame,bottom color=tcbcol@frame,middle color=yellow!75!tcbcol@frame},
  title style={left color=tcbcol@frame,right color=tcbcol@frame,middle color=yellow!75!tcbcol@frame},
  watermark tikz={\draw[line width=2mm] circle (1cm) node{\fontfamily{ptm}\fontseries{b}\fontsize{20mm}{20mm}\selectfont!};},
  watermark zoom=0.75,
}}


\def\tcb@arc@bor{\pgfsetcornersarced{\pgfqpoint{\tcb@border@arc}{\tcb@border@arc}}}%

\def\tcb@arc@bor@NW{\csname tcb@arc@bor@NW@\tcb@corner@mode@NW\endcsname}
\def\tcb@arc@bor@NE{\csname tcb@arc@bor@NE@\tcb@corner@mode@NE\endcsname}
\def\tcb@arc@bor@SW{\csname tcb@arc@bor@SW@\tcb@corner@mode@SW\endcsname}
\def\tcb@arc@bor@SE{\csname tcb@arc@bor@SE@\tcb@corner@mode@SE\endcsname}

\let\tcb@arc@bor@NW@sharp\tcb@arc@zpt
\let\tcb@arc@bor@NE@sharp\tcb@arc@zpt
\let\tcb@arc@bor@SW@sharp\tcb@arc@zpt
\let\tcb@arc@bor@SE@sharp\tcb@arc@zpt

\let\tcb@arc@bor@NW@rounded\tcb@arc@bor
\let\tcb@arc@bor@NE@rounded\tcb@arc@bor
\let\tcb@arc@bor@SW@rounded\tcb@arc@bor
\let\tcb@arc@bor@SE@rounded\tcb@arc@bor

\def\tcb@border@prepare#1#2{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@border@ts\relax%
    \tcbdimto\tcb@border@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@border@ts\relax}%
  \else%
    \let\tcb@border@arc=\tcb@zpt%
  \fi%
}

\def\tcb@border@unbroken#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathbase{draw,line width=#1,#3}{[xshift=\tcb@border@ts,yshift=\tcb@border@ts]frame.south west}%
    {[xshift=-\tcb@border@ts,yshift=-\tcb@border@ts]frame.north east}%
    {\tcb@arc@bor@SW}{\tcb@arc@bor@NW}{\tcb@arc@bor@NE}{\tcb@arc@bor@SE}%
}

\def\tcb@border@first#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathboundary{draw,line width=#1,#3}{%
    \tcb@gettikzxy{([xshift=\tcb@border@ts]frame.south west)}{\tcb@xa}{\tcb@ya}%
    \tcb@gettikzxy{([xshift=-\tcb@border@ts,yshift=-\tcb@border@ts]frame.north east)}{\tcb@xb}{\tcb@yb}%
    \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
    \tcb@arc@bor@NW\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
    \tcb@arc@bor@NE\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
    \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  }%
}

\def\tcb@border@middle#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \draw[line width=#1,#3]
    ([xshift=\tcb@border@ts]frame.north west) -- ([xshift=\tcb@border@ts]frame.south west);%
  \draw[line width=#1,#3]
    ([xshift=-\tcb@border@ts]frame.north east) -- ([xshift=-\tcb@border@ts]frame.south east);%
}

\def\tcb@border@last#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathboundary{draw,line width=#1,#3}{%
    \tcb@gettikzxy{([xshift=\tcb@border@ts,yshift=\tcb@border@ts]frame.south west)}{\tcb@xa}{\tcb@ya}%
    \tcb@gettikzxy{([xshift=-\tcb@border@ts]frame.north east)}{\tcb@xb}{\tcb@yb}%
    \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
    \tcb@arc@bor@SW\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
    \tcb@arc@bor@SE\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
    \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  }%
}

\def\tcb@draw@border@unbroken{%
  \let\tcb@border=\tcb@border@unbroken%
  \kvtcb@borderline%
}

\def\tcb@draw@border@first{%
  \let\tcb@border=\tcb@border@first%
  \kvtcb@borderline%
}

\def\tcb@draw@border@middle{%
  \let\tcb@border=\tcb@border@middle%
  \kvtcb@borderline%
}

\def\tcb@draw@border@last{%
  \let\tcb@border=\tcb@border@last%
  \kvtcb@borderline%
}

\def\tcb@bordernorth@draw#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([yshift=-\tcb@border@ts]frame.north west) -- ([yshift=-\tcb@border@ts]frame.north east);%
}

\def\tcb@bordernorth{%
  \ifdefstring{\tcb@split@state}{unbroken}{\tcb@bordernorth@draw}{%
    \ifdefstring{\tcb@split@state}{first}{\tcb@bordernorth@draw}{}}%
}

\def\tcb@bordersouth@draw#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([yshift=\tcb@border@ts]frame.south west) -- ([yshift=\tcb@border@ts]frame.south east);%
}

\def\tcb@bordersouth{%
  \ifdefstring{\tcb@split@state}{unbroken}{\tcb@bordersouth@draw}{%
    \ifdefstring{\tcb@split@state}{last}{\tcb@bordersouth@draw}{}}%
}

\def\tcb@borderwest#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([xshift=\tcb@border@ts]frame.north west) -- ([xshift=\tcb@border@ts]frame.south west);%
}

\def\tcb@bordereast#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([xshift=-\tcb@border@ts]frame.north east) -- ([xshift=-\tcb@border@ts]frame.south east);%
}

\tcbset{%
  border@line app/.code={\appto\kvtcb@borderline{#1}},%
  borderline/.style args={#1#2#3}{border@line app={\tcb@border{#1}{#2}{#3}}},%
  no borderline/.code={\def\kvtcb@borderline{}},%
  borderline north/.style args={#1#2#3}{border@line app={\tcb@bordernorth{#1}{#2}{#3}}},%
  borderline south/.style args={#1#2#3}{border@line app={\tcb@bordersouth{#1}{#2}{#3}}},%
  borderline west/.style args={#1#2#3}{border@line app={\tcb@borderwest{#1}{#2}{#3}}},%
  borderline east/.style args={#1#2#3}{border@line app={\tcb@bordereast{#1}{#2}{#3}}},%
  borderline horizontal/.style args={#1#2#3}{borderline north={#1}{#2}{#3},borderline south={#1}{#2}{#3}},%
  borderline vertical/.style args={#1#2#3}{borderline west={#1}{#2}{#3},borderline east={#1}{#2}{#3}},%
}


\def\tcb@shadow@comp@ts@smart#1#2{%
  \ifdim#2>0pt\relax\tcbdimto\tcb@shadow@ts{#1-#2/2}%%
  \else\tcbdimto\tcb@shadow@ts{#1+#2/2}\fi%
}

\def\tcb@shadow@comp@ts@copy#1#2{%
  \tcbdimto\tcb@shadow@ts{#1}%
}

\def\tcb@shadow@comp@arc{%
  \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax%
    \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax}%
  \else%
    \let\tcb@shadow@arc=\tcb@zpt%
  \fi%
}

\def\tcb@arc@sha{\pgfsetcornersarced{\pgfqpoint{\tcb@shadow@arc}{\tcb@shadow@arc}}}%

\def\tcb@arc@sha@NW{\csname tcb@arc@sha@NW@\tcb@corner@mode@NW\endcsname}
\def\tcb@arc@sha@NE{\csname tcb@arc@sha@NE@\tcb@corner@mode@NE\endcsname}
\def\tcb@arc@sha@SW{\csname tcb@arc@sha@SW@\tcb@corner@mode@SW\endcsname}
\def\tcb@arc@sha@SE{\csname tcb@arc@sha@SE@\tcb@corner@mode@SE\endcsname}

\let\tcb@arc@sha@NW@sharp\tcb@arc@zpt
\let\tcb@arc@sha@NE@sharp\tcb@arc@zpt
\let\tcb@arc@sha@SW@sharp\tcb@arc@zpt
\let\tcb@arc@sha@SE@sharp\tcb@arc@zpt

\let\tcb@arc@sha@NW@rounded\tcb@arc@sha
\let\tcb@arc@sha@NE@rounded\tcb@arc@sha
\let\tcb@arc@sha@SW@rounded\tcb@arc@sha
\let\tcb@arc@sha@SE@rounded\tcb@arc@sha

\def\tcb@shadow@unbroken#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@sha@SE}%
}

\def\tcb@shadow@first#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@zpt}%
}

\def\tcb@shadow@middle#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@shadow@last#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@sha@SE}%
}


\tcbset{%
  shad@w app/.code={\appto\kvtcb@shadow{#1}},%
  shadow/.style args={#1#2#3#4}{shad@w app={\csuse{tcb@shadow@\tcb@shapeofskin}{#1}{#2}{#3}{#4}}},%
  no shadow/.code={\def\kvtcb@shadow{}},%
  fuzzy shadow/.style args={#1#2#3#4#5}{shad@w app={%
    \begin{scope}[#5]%
      \letcs\tcb@shadow{tcb@shadow@\tcb@shapeofskin}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-4\dimexpr#4\relax}{opacity=0.01}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-3\dimexpr#4\relax}{opacity=0.02}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-2\dimexpr#4\relax}{opacity=0.04}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-#4\relax}{opacity=0.07}%
      \tcb@shadow{#1}{#2}{#3}{opacity=0.11}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+#4\relax}{opacity=0.11}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+2\dimexpr#4\relax}{opacity=0.07}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+3\dimexpr#4\relax}{opacity=0.04}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+4\dimexpr#4\relax}{opacity=0.02}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+5\dimexpr#4\relax}{opacity=0.01}%
  \end{scope}}},%
  %
  drop shadow/.style={shadow={0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},
  drop shadow/.default={black!50!white},%
  drop midday shadow/.style={shadow={0mm}{-0.8mm}{-0.4mm}{opacity=0.5,#1}},
  drop midday shadow/.default={black!50!white},%
  halo/.style args={#1 with #2}{shadow={0mm}{0mm}{-#1}{opacity=0.5,#2}},
  halo/.default={0.9mm with yellow},%
  drop fuzzy shadow/.style={fuzzy shadow={1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow/.default={black!50!white},%
  drop fuzzy midday shadow/.style={fuzzy shadow={0mm}{-1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy midday shadow/.default={black!50!white},%
  fuzzy halo/.style args={#1 with #2}{fuzzy shadow={0mm}{0mm}{-#1}{0.12mm}{#2}},
  fuzzy halo/.default={1.0mm with yellow},%
  %
  drop shadow southeast/.style={shadow={0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow southeast/.default={black!50!white},%
  drop shadow south/.style={shadow={0mm}{-0.8mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow south/.default={black!50!white},%
  drop shadow southwest/.style={shadow={-0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow southwest/.default={black!50!white},%
  drop shadow west/.style={shadow={-0.8mm}{0mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow west/.default={black!50!white},%
  drop shadow northwest/.style={shadow={-0.9mm}{0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow northwest/.default={black!50!white},%
  drop shadow north/.style={shadow={0mm}{0.8mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow north/.default={black!50!white},%
  drop shadow northeast/.style={shadow={0.9mm}{0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow northeast/.default={black!50!white},%
  drop shadow east/.style={shadow={0.8mm}{0mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow east/.default={black!50!white},%
  drop fuzzy shadow southeast/.style={fuzzy shadow={1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow southeast/.default={black!50!white},%
  drop fuzzy shadow south/.style={fuzzy shadow={0mm}{-1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow south/.default={black!50!white},%
  drop fuzzy shadow southwest/.style={fuzzy shadow={-1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow southwest/.default={black!50!white},%
  drop fuzzy shadow west/.style={fuzzy shadow={-1.0mm}{0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow west/.default={black!50!white},%
  drop fuzzy shadow northwest/.style={fuzzy shadow={-1.0mm}{1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow northwest/.default={black!50!white},%
  drop fuzzy shadow north/.style={fuzzy shadow={0mm}{1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow north/.default={black!50!white},%
  drop fuzzy shadow northeast/.style={fuzzy shadow={1.0mm}{1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow northeast/.default={black!50!white},%
  drop fuzzy shadow east/.style={fuzzy shadow={1.0mm}{0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow east/.default={black!50!white},%
  %
  smart shadow arc/.is choice,
  smart shadow arc/true/.code={\let\tcb@shadow@comp@ts=\tcb@shadow@comp@ts@smart},
  smart shadow arc/false/.code={\let\tcb@shadow@comp@ts=\tcb@shadow@comp@ts@copy},
  smart shadow arc/.default=true,
}

\def\tcb@boundary@tikzbendedbase#1#2#3#4#5#6#7#8{%
  \tcb@gettikzxy{(#1)}{\tcb@xa}{\tcb@ya}%
  \tcb@gettikzxy{(#2)}{\tcb@xb}{\tcb@yb}%
  \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
  #5\pgfpathquadraticcurveto{\pgfqpoint{\dimexpr0.5\dimexpr\tcb@xa+\tcb@xb\relax}{\dimexpr\tcb@yb+#8}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  #6\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  #3\pgfpathquadraticcurveto{\pgfqpoint{\dimexpr0.5\dimexpr\tcb@xa+\tcb@xb\relax}{\dimexpr\tcb@ya+#7}}{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  #4\pgfpathclose%
}

\def\tcb@pathbendedbase#1#2#3#4#5#6#7#8#9{\tcb@pathboundary{#1}{\tcb@boundary@tikzbendedbase{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}}

\def\tcb@shadowbended@prepare#1{%
  \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr#1\relax}%
  \ifdim\dimexpr\tcb@shadow@arc<0pt\relax%
    \let\tcb@shadow@arc=\tcb@zpt%
  \fi%
}

\def\tcb@shadowlifted@unbroken#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@sha@SE}{#4}{0pt}%
}

\def\tcb@shadowlifted@first#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@zpt}{#4}{0pt}%
}

\def\tcb@shadowlifted@middle#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{#4}{0pt}%
}

\def\tcb@shadowlifted@last#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@sha@SE}{#4}{0pt}%
}

\tcbset{
  lifted shadow/.style n args={5}{shad@w app={%
    \begin{scope}[#5]%
      \letcs\tcb@shadowlifted{tcb@shadowlifted@\tcb@shapeofskin}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-4\dimexpr#4}{#3}{opacity=0.01}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-3\dimexpr#4}{#3}{opacity=0.02}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-2\dimexpr#4}{#3}{opacity=0.04}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-#4}{#3}{opacity=0.07}%
      \tcb@shadowlifted{#1}{#2}{0pt}{#3}{opacity=0.11}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+#4}{#3}{opacity=0.11}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+2\dimexpr#4}{#3}{opacity=0.07}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+3\dimexpr#4}{#3}{opacity=0.04}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+4\dimexpr#4}{#3}{opacity=0.02}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+5\dimexpr#4}{#3}{opacity=0.01}%
  \end{scope}}},%
  drop small lifted shadow/.style={lifted shadow={1mm}{-0.75mm}{1.3mm}{0.1mm}{#1}},
  drop small lifted shadow/.default={black!50!white},%
  drop lifted shadow/.style={lifted shadow={1.5mm}{-1.5mm}{2.7mm}{0.12mm}{#1}},
  drop lifted shadow/.default={black!50!white},%
  drop large lifted shadow/.style={lifted shadow={2mm}{-3mm}{5.7mm}{0.16mm}{#1}},
  drop large lifted shadow/.default={black!50!white},%
}

\newif\iftcb@isindraft
\def\tcb@draftmode{\tcbset{spartan,spartan@fit}}
\def\tcbstartdraftmode{\let\tcb@afteroptions@hook=\tcb@draftmode\tcb@isindrafttrue}
\def\tcbstopdraftmode{\let\tcb@afteroptions@hook=\@empty\tcb@isindraftfalse}

\def\tcbinterruptdraftmode{%
  \iftcb@isindraft%
    \tcbstopdraftmode%
    \let\tcbcontinuedraftmode=\tcbstartdraftmode%
  \else%
    \let\tcbcontinuedraftmode=\@empty%
  \fi}

\tcbset{%
  draftmode/.is choice,%
  draftmode/.default=true,%
  draftmode/true/.code=\tcbstartdraftmode,%
  draftmode/false/.code=\tcbstopdraftmode,%
}


\def\tcb@include@graphics{%
  \ifdefstring{\kvtcb@capture}{hbox}{%
    \tcbox{%
      \begingroup\edef\x{\endgroup\noexpand\includegraphics[\expandonce\kvtcb@graphics@options]}%
      \x{\imagepath}%
    }%
  }{%
    \iftcb@fixedheight%
      \begin{tcolorbox}%
        \begingroup\edef\x{\endgroup\noexpand\includegraphics[\expandonce\kvtcb@graphics@options,width=\linewidth,height=\tcbtextheight,keepaspectratio]}%
        \x{\imagepath}%
      \end{tcolorbox}%
    \else%
      \begin{tcolorbox}%
        \begingroup\edef\x{\endgroup\noexpand\includegraphics[\expandonce\kvtcb@graphics@options,width=\linewidth]}%
        \x{\imagepath}%
      \end{tcolorbox}%
    \fi%
  }%
}

\def\tcb@scanfilename#1#2{%
  \begingroup%
    \everyeof{\noexpand}%
    \endlinechar -1%
    \catcode`\_=11%
    \catcode`\~=11%
    \edef\x{\scantokens\expandafter{#2}}%
  \expandafter\endgroup%
  \expandafter\def\expandafter #1\expandafter{\x}%
}%


\def\tcb@include@graphics@preparefile#1{%
  \tcb@scanfilename\tcb@temp{#1}%
  \filename@parse{\tcb@temp}%
  \ifx\filename@ext\relax%
    \let\imagename\filename@base%
  \else%
    \def\imagename{\filename@base\Gin@sepdefault\filename@ext}%
  \fi%
  \ifdefined\grffile@Ginclude@graphics%
    % grffile package loaded
    \ifx\kvtcb@graphics@directory\@empty%
      \def\imagepath{#1}%
    \else%
      \def\imagepath{\kvtcb@graphics@directory/#1}%
    \fi%
  \else%
    \ifx\kvtcb@graphics@directory\@empty%
      \edef\imagepath{#1}%
    \else%
      \edef\imagepath{\kvtcb@graphics@directory/#1}%
    \fi%
  \fi%
}

\newcommand{\tcbincludegraphics}[2][]{%
  \begingroup%
  \tcb@layer@pushup%
  \tcb@apply@box@options{enhanced,clip upper=true,valign=center,center upper,#1}%
  \tcb@include@graphics@preparefile{#2}%
  \edef\imagepage{1}%
  \tcb@include@graphics%
  \endgroup%
}

\def\tcb@set@pdfpages#1#2{%
  \IfFileExists{#2}{%
    \ifdef{\pdfximage}{%
      \pdfximage{#2}%
      \edef#1{\the\pdflastximagepages}%
    }{%
      \ifdef{\XeTeXpdfpagecount}{%
        \edef#1{\the\XeTeXpdfpagecount #2 }%
        \ifnum#1=0 %
          \edef#1{1}%
        \fi%
      }{\tcb@error{For PDF support run pdflatex, xelatex, or lualatex}{%
        Your compiler seems not to support PDF include files.}}%
    }%
  }{\tcb@error{PDF file `#2' not found}{The PDF file `#2' was not found}}%
  \relax%
}

\newcommand{\tcbincludepdf}[2][]{%
  \begingroup%
  \tcb@layer@pushup%
  \tcb@apply@box@options{enhanced,clip upper=true,valign=center,center upper,#1}%
  \appto\kvtcb@graphics@options{,page=\imagepage}%
  \tcb@include@graphics@preparefile{#2}%
  \tcb@set@pdfpages\pdfpages{\imagepath}%
  \foreach \imagepage in \kvtcb@graphics@pages%
  {%
    \tcb@include@graphics%
  }%
  \endgroup%
}

\tcbset{%
  graphics options/.store in=\kvtcb@graphics@options,
  graphics pages/.store in=\kvtcb@graphics@pages,
  graphics directory/.store in=\kvtcb@graphics@directory,
}


\tcbset{%
  reset@skins/.style={%
    frame style=,interior style=,segmentation style=,@title style=,%
    colbacklower=black!15!white,%
    extend freelance=,extend freelancefirst=,extend freelancemiddle=,extend freelancelast=,%
    clear@spec,%
    watermark opacity=1.00,watermark color=tcbcol@back!85!tcbcol@frame,%
    watermark zoom=0.75,clip watermark,%
    clip title=false,clip upper=false,clip lower=false,%
    no borderline,smart shadow arc,no shadow,no underlay,no finish,tikz reset,at begin tikz reset,at end tikz reset,%
    boxed title size=title,no boxed title style,hbox boxed title,code={\let\tcb@specialgeonodes@hook\relax},%
    graphics options=,graphics pages={1,...,\pdfpages},graphics directory=,%
  },
  initialize@reset=reset@skins,
}

\tcbuselibrary{skins@jigsaw}


==> tcbskinsjigsaw.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcbskinsjigsaw.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.94}

\tcbuselibrary{skins}

\def\tcb@drawframe@pathjigsaw{%
  \tcb@pathboundary{tcb fill frame}{\tcb@boundaryframe@standardjigsaw}%
}

\def\tcb@boundary@pathfirstjigsaw@A{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\tcb@height-\kvtcb@top@rule}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@out@NW\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \tcb@arc@out@NE\pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \tcb@arc@ins@NE\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \tcb@arc@ins@NW\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@boundary@pathfirstjigsaw@B{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@out@NW\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \tcb@arc@out@NE\pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@drawframe@pathfirstjigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundary@pathfirstjigsaw@B%
          \tcb@boundarytitle@standard%
        \else%
          \tcb@boundary@pathfirstjigsaw@A%
        \fi%
      \else%
        \tcb@boundary@pathfirstjigsaw@B%
      \fi%
    \else%
      \tcb@boundary@pathfirstjigsaw@A%
    \fi%
  }%
}

\def\tcb@boundary@pathmiddlejigsaw@A{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{\kvtcb@left@rule}{\tcb@height}}%
  \pgfpathrectangle{\pgfqpoint{\tcb@xa}{0pt}}{\pgfqpoint{\kvtcb@right@rule}{\tcb@height}}%
}

\def\tcb@boundary@pathmiddlejigsaw@B{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\tcb@height-\kvtcb@top@rule}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@boundary@pathmiddlejigsaw@C{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@drawframe@pathmiddlejigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundary@pathmiddlejigsaw@C%
          \tcb@arc@zpt%
          \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule}%
          \tcbdimto\tcb@xb{\tcb@width-\kvtcb@right@rule}%
          \tcbdimto\tcb@yb{\tcb@height-\kvtcb@top@rule}%
          \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
        \else%
          \tcb@boundary@pathmiddlejigsaw@B%
        \fi%
      \else%
        \tcb@boundary@pathmiddlejigsaw@C%
      \fi%
    \else%
      \tcb@boundary@pathmiddlejigsaw@A%
    \fi%
  }%
}

\def\tcb@drawframe@pathlastjigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundaryframe@pathlast%
          \tcb@arc@zpt%
          \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule}%
          \tcbdimto\tcb@xb{\tcb@width-\kvtcb@right@rule}%
          \tcbdimto\tcb@yb{\tcb@height-\kvtcb@top@rule}%
          \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
          \tcb@boundaryinterior@title@standard%
        \else%
          \tcb@boundaryframe@pathlast%
          \tcb@boundary@base{\kvtcb@left@rule}{\kvtcb@bottom@rule}%
            {\tcb@width-\kvtcb@right@rule}{\tcb@height-\kvtcb@top@rule}%
            {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
        \fi%
      \else%
        \tcb@boundaryframe@pathlast%
      \fi%
    \else%
      \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
      \pgfpathmoveto{\pgfpointorigin}%
      \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
      \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@height}}%
      \tcb@arc@ins@SW\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
      \tcb@arc@ins@SE\pgfpathlineto{\pgfqpoint{\tcb@xa}{\kvtcb@bottom@rule}}%
      \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@height}}%
      \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
      \tcb@arc@out@SE\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
      \tcb@arc@out@SW\pgfpathclose%
    \fi%
  }%
}


\def\tcb@draw@shadowjigsaw@unbroken{%
  \let\tcb@shadow=\tcb@shadow@unbroken%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@first{%
  \let\tcb@shadow=\tcb@shadow@first%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@middle{%
  \let\tcb@shadow=\tcb@shadow@middle%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@last{%
  \let\tcb@shadow=\tcb@shadow@last%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\tcb@new@skin{enhanced jigsaw}{base@unbroken,%
  frame engine=pathjigsaw,interior titled engine=path,interior engine=path,segmentation engine=path,title engine=path,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@unbroken},%
  skin first=enhancedfirst jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedlast jigsaw}

\tcb@new@skin{enhancedfirst jigsaw}{base@first,%
  frame engine=pathfirstjigsaw,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=path,title engine=pathfirst,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@first},%
  skin first=enhancedfirst jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedmiddle jigsaw}

\tcb@new@skin{enhancedmiddle jigsaw}{base@middle,%
  frame engine=pathmiddlejigsaw,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=path,title engine=pathmiddle,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@middle},%
  skin first=enhancedmiddle jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedmiddle jigsaw}

\tcb@new@skin{enhancedlast jigsaw}{base@last,%
  frame engine=pathlastjigsaw,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=path,title engine=pathlast,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@last},%
  skin first=enhancedmiddle jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedlast jigsaw}

\tcbset{%
  enhanced jigsaw/.style={skin=enhanced jigsaw},%
  frame engine/pathjigsaw/.style={frame code=\tcb@drawframe@pathjigsaw},
  frame engine/pathfirstjigsaw/.style={frame code=\tcb@drawframe@pathfirstjigsaw},
  frame engine/pathmiddlejigsaw/.style={frame code=\tcb@drawframe@pathmiddlejigsaw},
  frame engine/pathlastjigsaw/.style={frame code=\tcb@drawframe@pathlastjigsaw},
}



==> tcbtheorems.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcbtheorems.code.tex: Code for theorems in colorboxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.94}

\RequirePackage{amsmath}

\def\tcb@hack@amsmath{\tcb@hack@currenvir\vskip-\abovedisplayskip}

\def\tcb@theo@form@namenumber#1#2{\hbox{#1~#2}}
\def\tcb@theo@form@numbername#1#2{\hbox{#2~#1}}
\def\tcb@theo@form@name#1#2{\hbox{#1}}

\def\tcb@theo@desc@form@std#1{\tcb@desc@col\kvtcb@desc@font\kvtcb@desc@delim@left#1\kvtcb@desc@delim@right}

\def\tcb@theo@title#1#2#3{%
  \ifdefempty{#2}{\setbox\z@=\color@hbox#1\color@endbox}{\setbox\z@=\tcb@theo@form{#1}{#2}}%
  \def\temp@a{#3}%
  \ifx\temp@a\@empty\relax%
    \unhbox\z@\kvtcb@terminatorsign%
  \else%
    \setbox\z@=\hbox{\unhbox\z@\kvtcb@separatorsign\ }%
    \hangindent\wd\z@%
    \hangafter=1%
    \mbox{\unhbox\z@}{\tcb@theo@desc@form{#3}}\kvtcb@terminatorsign%
  \fi%
}

\def\tcb@theo@listentry#1#2#3{%
  \def\kvtcb@listentry{\protect\numberline{#2}#3}%
}

\def\tcb@theo@label#1#2{%
  \def\temp@a{#2}%
  \ifx\temp@a\@empty%
  \else%
    \tcbset{label={#1\kvtcb@label@sep#2}}%
  \fi%
}

\if@fleqn%
\tcbset{%
  ams equation upper/.style={before upper=\tcb@hack@amsmath\equation,after upper=\endequation},%
  ams equation lower/.style={before lower=\tcb@hack@amsmath\equation,after lower=\endequation},%
  ams equation* upper/.style={before upper=\tcb@hack@amsmath\csname equation*\endcsname,after upper=\endequation},%
  ams equation* lower/.style={before lower=\tcb@hack@amsmath\csname equation*\endcsname,after lower=\endequation}%
}%
\else%
\tcbset{%
  ams equation upper/.style={before upper=\tcb@hack@currenvir\equation,after upper=\endequation},%
  ams equation lower/.style={before lower=\tcb@hack@currenvir\equation,after lower=\endequation},%
  ams equation* upper/.style={before upper=\tcb@hack@currenvir\csname equation*\endcsname,after upper=\endequation},%
  ams equation* lower/.style={before lower=\tcb@hack@currenvir\csname equation*\endcsname,after lower=\endequation},%
}%
\fi

\tcbset{
  theorem/.style args={#1#2#3#4}{%
    step and label={#2}{#4},%
    title={\letcs\tcb@temp{the#2}\tcb@theo@title{#1}{\tcb@temp}{#3}}},%
  math upper/.style={before upper=$\displaystyle,after upper=$},%
  math lower/.style={before lower=$\displaystyle,after lower=$},%
  math/.style={math upper,math lower},%
  ams equation/.style={ams equation upper,ams equation lower},%
  ams equation*/.style={ams equation* upper,ams equation* lower},%
  ams align upper/.style={before upper=\tcb@hack@amsmath\align,after upper=\endalign},%
  ams align lower/.style={before lower=\tcb@hack@amsmath\align,after lower=\endalign},%
  ams align/.style={ams align upper,ams align lower},%
  ams align* upper/.style={before upper=\tcb@hack@amsmath\csname align*\endcsname,after upper=\endalign},%
  ams align* lower/.style={before lower=\tcb@hack@amsmath\csname align*\endcsname,after lower=\endalign},%
  ams align*/.style={ams align* upper,ams align* lower},%
  ams gather upper/.style={before upper=\tcb@hack@amsmath\gather,after upper=\endgather},%
  ams gather lower/.style={before lower=\tcb@hack@amsmath\gather,after lower=\endgather},%
  ams gather/.style={ams gather upper,ams gather lower},%
  ams gather* upper/.style={before upper=\tcb@hack@amsmath\csname gather*\endcsname,after upper=\endgather},%
  ams gather* lower/.style={before lower=\tcb@hack@amsmath\csname gather*\endcsname,after lower=\endgather},%
  ams gather*/.style={ams gather* upper,ams gather* lower},%
  ams nodisplayskip upper/.style={before upper=\vskip-\abovedisplayskip},%
  ams nodisplayskip lower/.style={before lower=\vskip-\abovedisplayskip},%
  ams nodisplayskip/.style={ams nodisplayskip upper,ams nodisplayskip lower},%
  highlight math style/.style={highlight math/.style={notitle,nophantom,#1}},%
  separator sign/.store in=\kvtcb@separatorsign,%
  separator sign colon/.style={separator sign={:}},%
  separator sign dash/.style={separator sign={\ --}},%
  separator sign none/.style={separator sign=},%
  terminator sign/.store in=\kvtcb@terminatorsign,%
  terminator sign colon/.style={terminator sign={:}},%
  terminator sign dash/.style={terminator sign={\ --}},%
  terminator sign none/.style={terminator sign=},%
  label separator/.store in=\kvtcb@label@sep,%
  description delimiters/.code 2 args={\def\kvtcb@desc@delim@left{#1}\def\kvtcb@desc@delim@right{#2}},%
  description delimiters parenthesis/.style={description delimiters=()},
  description delimiters none/.style={description delimiters={}{}},
  description color/.code={\def\temp@a{#1}\ifx\temp@a\@empty\relax%
    \def\tcb@desc@col{}\else\def\tcb@desc@col{\color{#1}}\fi},%
  description color/.default=,
  description font/.store in=\kvtcb@desc@font,
  description font/.default=,
  description formatter/.code={\let\tcb@theo@desc@form=#1},%
  description formatter/.default={\tcb@theo@desc@form@std},%
  theorem name and number/.code={\let\tcb@theo@form=\tcb@theo@form@namenumber},
  theorem number and name/.code={\let\tcb@theo@form=\tcb@theo@form@numbername},
  theorem name/.code={\let\tcb@theo@form=\tcb@theo@form@name},
  theorem style/.is choice,
  theorem style/standard/.style={separator sign colon,description delimiters none,
    terminator sign none,theorem name and number,attach title},
  theorem style/change standard/.style={theorem style=standard,theorem number and name},
  theorem style/plain/.style={separator sign none,description delimiters parenthesis,
    terminator sign colon,theorem name and number,attach title to upper={\ }},
  theorem style/plain apart/.style={separator sign none,description delimiters parenthesis,
    terminator sign none,theorem name and number,attach title},
  theorem style/break/.style={theorem style=plain,attach title to upper={\par}},
  theorem style/change/.style={theorem style=plain,theorem number and name},
  theorem style/change apart/.style={theorem style=plain apart,theorem number and name},
  theorem style/change break/.style={theorem style=break,theorem number and name},
  theorem style/margin/.style={theorem style=plain,theorem name,before title=\makebox[0pt][r]{\thetcbcounter\ }},
  theorem style/margin apart/.style={theorem style=margin,attach title,terminator sign none},
  theorem style/margin break/.style={theorem style=margin,attach title to upper={\par}},
}

\newcommand{\new@tcbtheorem}[5][]{%
  \@@newtcolorbox[auto counter,#1]{#2}[3][]{#4,%
    title={\tcb@theo@title{#3}{\thetcbcounter}{##2}},%
    list entry={\protect\numberline{\thetcbcounter}##2},%
    nameref={##2},%
    code={\tcb@theo@label{#5}{##3}},%
    ##1}%
  \@@newtcolorbox[#1,no counter,list inside=]{#2*}[2][]{#4,%
    title={\tcb@theo@title{#3}{\@empty}{##2}},%
    ##1}%
}

\def\newtcbtheorem{\let\@@newtcolorbox\newtcolorbox%
  \new@tcbtheorem}

\def\renewtcbtheorem{\let\@@newtcolorbox\renewtcolorbox%
  \new@tcbtheorem}

\newcommand{\tcbmaketheorem}[5]{%
  \newtcolorbox{#1}[3][]{#3,theorem={#2}{#4}{##2}{#5\kvtcb@label@sep##3},##1}%
}

\newtcbox{\tcboxmath}[1][]{nobeforeafter,math upper,tcbox raise base,#1}
\newtcbox{\tcbhighmath}[1][]{highlight math,nobeforeafter,math upper,tcbox raise base,#1}

\tcbset{%
  reset@theorems/.style={%
    description formatter,description color,description font,
    highlight math style={colframe=red,colback=yellow!25!white},%
    theorem style=standard,label separator=:,%
  },
  initialize@reset=reset@theorems,
}



==> tcbvignette.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcbvignette.code.tex: Code for ornamental frames
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.94}

\tcbuselibrary{skins}

\usetikzlibrary{fadings}

\pgfdeclarehorizontalshading{tcb@fade@east}{100bp}
{color(0bp)=(pgftransparent!50); color(25bp)=(pgftransparent!50);
 color(75bp)=(pgftransparent!100); color(100bp)=(pgftransparent!100)}

\pgfdeclarehorizontalshading{tcb@fade@west}{100bp}
{color(0bp)=(pgftransparent!100); color(25bp)=(pgftransparent!100);
 color(75bp)=(pgftransparent!50); color(100bp)=(pgftransparent!50)}

\pgfdeclareverticalshading{tcb@fade@north}{100bp}
{color(0bp)=(pgftransparent!50); color(25bp)=(pgftransparent!50);
 color(75bp)=(pgftransparent!100); color(100bp)=(pgftransparent!100)}

\pgfdeclareverticalshading{tcb@fade@south}{100bp}
{color(0bp)=(pgftransparent!100); color(25bp)=(pgftransparent!100);
 color(75bp)=(pgftransparent!50); color(100bp)=(pgftransparent!50)}

\pgfdeclarefading{semi east}{\pgfuseshading{tcb@fade@east}}
\pgfdeclarefading{semi west}{\pgfuseshading{tcb@fade@west}}
\pgfdeclarefading{semi north}{\pgfuseshading{tcb@fade@north}}
\pgfdeclarefading{semi south}{\pgfuseshading{tcb@fade@south}}

\def\tcb@vig@draw@north#1{\path[#1]\pgfextra{%
  \pgfpathmoveto{\pgfqpoint{\tcb@vig@xA}{\tcb@vig@yB}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xB}{\tcb@vig@yB}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xb}{\tcb@vig@yb}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xa}{\tcb@vig@yb}}%
  \pgfpathclose};}

\def\tcb@vig@draw@east#1{\path[#1]\pgfextra{%
  \pgfpathmoveto{\pgfqpoint{\tcb@vig@xB}{\tcb@vig@yB}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xB}{\tcb@vig@yA}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xb}{\tcb@vig@ya}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xb}{\tcb@vig@yb}}%
  \pgfpathclose};}

\def\tcb@vig@draw@south#1{\path[#1]\pgfextra{%
  \pgfpathmoveto{\pgfqpoint{\tcb@vig@xB}{\tcb@vig@yA}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xA}{\tcb@vig@yA}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xa}{\tcb@vig@ya}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xb}{\tcb@vig@ya}}%
  \pgfpathclose};}

\def\tcb@vig@draw@west#1{\path[#1]\pgfextra{%
  \pgfpathmoveto{\pgfqpoint{\tcb@vig@xA}{\tcb@vig@yA}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xA}{\tcb@vig@yB}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xa}{\tcb@vig@yb}}%
  \pgfpathlineto{\pgfqpoint{\tcb@vig@xa}{\tcb@vig@ya}}%
  \pgfpathclose};}

\def\tcb@vig@draw@direct{%
  \ifdim\tcb@vig@yB>\tcb@vig@yb\relax%
    \begingroup\edef\x{\endgroup\noexpand\tcb@vig@draw@north{fill,draw=none,\expandonce\tcb@vig@style@north}}\x%
  \fi%
  \ifdim\tcb@vig@xB>\tcb@vig@xb\relax%
    \begingroup\edef\x{\endgroup\noexpand\tcb@vig@draw@east{fill,draw=none,\expandonce\tcb@vig@style@east}}\x%
  \fi%
  \ifdim\tcb@vig@yA<\tcb@vig@ya\relax%
    \begingroup\edef\x{\endgroup\noexpand\tcb@vig@draw@south{fill,draw=none,\expandonce\tcb@vig@style@south}}\x%
  \fi%
  \ifdim\tcb@vig@xA<\tcb@vig@xa\relax%
    \begingroup\edef\x{\endgroup\noexpand\tcb@vig@draw@west{fill,draw=none,\expandonce\tcb@vig@style@west}}\x%
  \fi%
}

\def\tcb@vig@draw@clipped{%
  \ifdim\tcb@vig@yB>\tcb@vig@yb\relax%
    \begin{scope}
    \tcb@vig@draw@north{clip}%
    \begingroup\edef\x{\endgroup\noexpand\path[fill,\expandonce\tcb@vig@style@north]}%
    \x\pgfextra{\pgfpathrectanglecorners{\pgfpoint{\tcb@vig@xA-1mm}{\tcb@vig@yb}}%
        {\pgfpoint{\tcb@vig@xB+1mm}{\tcb@vig@yB}}};
    \end{scope}
  \fi%
  \ifdim\tcb@vig@xB>\tcb@vig@xb\relax%
    \begin{scope}
    \tcb@vig@draw@east{clip}%
    \begingroup\edef\x{\endgroup\noexpand\path[fill,\expandonce\tcb@vig@style@east]}%
    \x\pgfextra{\pgfpathrectanglecorners{\pgfpoint{\tcb@vig@xb}{\tcb@vig@yA-1mm}}%
          {\pgfpoint{\tcb@vig@xB}{\tcb@vig@yB+1mm}}};
    \end{scope}
  \fi%
  \ifdim\tcb@vig@yA<\tcb@vig@ya\relax%
    \begin{scope}
    \tcb@vig@draw@south{clip}%
    \begingroup\edef\x{\endgroup\noexpand\path[fill,\expandonce\tcb@vig@style@south]}%
    \x\pgfextra{\pgfpathrectanglecorners{\pgfpoint{\tcb@vig@xA-1mm}{\tcb@vig@yA}}%
        {\pgfpoint{\tcb@vig@xB+1mm}{\tcb@vig@ya}}};
    \end{scope}
  \fi%
  \ifdim\tcb@vig@xA<\tcb@vig@xa\relax%
    \begin{scope}
    \tcb@vig@draw@west{clip}%
    \begingroup\edef\x{\endgroup\noexpand\path[fill,\expandonce\tcb@vig@style@west]}%
    \x\pgfextra{%
      \pgfpathrectanglecorners{\pgfpoint{\tcb@vig@xA}{\tcb@vig@yA-1mm}}%
        {\pgfpoint{\tcb@vig@xa}{\tcb@vig@yB+1mm}}};
    \end{scope}
  \fi%
}

\newcommand{\tcbvignette}[1]{%
  \ifdefined\pgfpictureid%
    \begingroup%
    \tcbset{vig/.cd,#1}%
    \tcbdimto\tcb@vig@xA{\tcb@vig@xmin}%
    \tcbdimto\tcb@vig@xB{\tcb@vig@xmax}%
    \tcbdimto\tcb@vig@yA{\tcb@vig@ymin}%
    \tcbdimto\tcb@vig@yB{\tcb@vig@ymax}%
    \tcbdimto\tcb@vig@xa{\tcb@vig@xA+\tcb@vig@size@west}%
    \tcbdimto\tcb@vig@xb{\tcb@vig@xB-(\tcb@vig@size@east)}%
    \tcbdimto\tcb@vig@ya{\tcb@vig@yA+\tcb@vig@size@south}%
    \tcbdimto\tcb@vig@yb{\tcb@vig@yB-(\tcb@vig@size@north)}%
    \begin{scope}[tcb@vig@scope]%
    \tcb@vig@draw%
    \end{scope}
    \endgroup%
  \else%
    \tcb@warning{'tcbvignette' was found outside a 'tikzpicture' environment and is ignored}%
  \fi%
}

\tcbset{%
  vig/.cd,
  xmin/.store in=\tcb@vig@xmin,
  xmax/.store in=\tcb@vig@xmax,
  ymin/.store in=\tcb@vig@ymin,
  ymax/.store in=\tcb@vig@ymax,
  lower left corner/.code={\tcb@gettikzxy{(#1)}{\tcb@vig@xmin}{\tcb@vig@ymin}},
  upper right corner/.code={\tcb@gettikzxy{(#1)}{\tcb@vig@xmax}{\tcb@vig@ymax}},
  %
  inside node/.style={lower left corner={#1.south west},upper right corner={#1.north east}},
  outside node/.style={lower left corner={[xshift=-\tcb@vig@size@west,yshift=-\tcb@vig@size@south]#1.south west},
    upper right corner={[xshift=\tcb@vig@size@east,yshift=\tcb@vig@size@north]#1.north east}},
  %
  on node/.style={lower left corner={#1.south west},upper right corner={#1.north east}},
  over node offset/.store in=\tcb@vig@onoffset,%
  over node/.style={lower left corner={[xshift=-\tcb@vig@onoffset,yshift=-\tcb@vig@onoffset]#1.south west},
    upper right corner={[xshift=\tcb@vig@onoffset,yshift=\tcb@vig@onoffset]#1.north east}},
  north size/.store in=\tcb@vig@size@north,
  south size/.store in=\tcb@vig@size@south,
  east size/.store in=\tcb@vig@size@east,
  west size/.store in=\tcb@vig@size@west,
  vertical size/.style={north size=#1,south size=#1},
  horizontal size/.style={east size=#1,west size=#1},
  size/.style={north size=#1,south size=#1,east size=#1,west size=#1},
  north style/.store in=\tcb@vig@style@north,
  south style/.store in=\tcb@vig@style@south,
  east style/.store in=\tcb@vig@style@east,
  west style/.store in=\tcb@vig@style@west,
  scope/.code={\tikzset{tcb@vig@scope/.style={#1}}},
  draw method/.is choice,
  draw method/direct/.code={\let\tcb@vig@draw\tcb@vig@draw@direct},%
  draw method/clipped/.code={\let\tcb@vig@draw\tcb@vig@draw@clipped},%
  base color/.colorlet=tcbcol@vig@base,
  raised color/.style={%
    base color=#1,
    north style={tcbcol@vig@base!50!white},
    east style={tcbcol@vig@base!75!black},
    south style={tcbcol@vig@base!50!black},
    west style={tcbcol@vig@base!75!white},
  },
  lowered color/.style={%
    base color=#1,
    north style={tcbcol@vig@base!50!black},
    east style={tcbcol@vig@base!75!white},
    south style={tcbcol@vig@base!50!white},
    west style={tcbcol@vig@base!75!black},
  },
  color from/.style args={#1 to #2}{%
    north style={bottom color=#1,top color=#2},
    east style={left color=#1,right color=#2},
    south style={top color=#1,bottom color=#2},
    west style={right color=#1,left color=#2},
  },
  fade in/.style={%
    north style={#1,path fading=south},
    east style={#1,path fading=west},
    south style={#1,path fading=north},
    west style={#1,path fading=east},
  },
  fade in/.default=white,
  fade out/.style={%
    north style={#1,path fading=north},
    east style={#1,path fading=east},
    south style={#1,path fading=south},
    west style={#1,path fading=west},
  },
  fade out/.default=white,
  semi fade in/.style={%
    north style={#1,path fading=semi south},
    east style={#1,path fading=semi west},
    south style={#1,path fading=semi north},
    west style={#1,path fading=semi east},
  },
  semi fade in/.default=white,
  semi fade out/.style={%
    north style={#1,path fading=semi north},
    east style={#1,path fading=semi east},
    south style={#1,path fading=semi south},
    west style={#1,path fading=semi west},
  },
  semi fade out/.default=white,
  %
  scope=,
  draw method=direct,
  xmin=0pt,
  xmax=1cm,
  ymin=0pt,
  ymax=1cm,
  size=2mm,
  over node offset=0.1mm,
  raised color=red,
}

\tcbset{%
  finish@vignette/.style 2 args={finish #1={%
    \begin{tcbclipframe}\tcbvignette{%
      scope={transparency group,opacity=0.25},
      north style=white,
      east style=black!75,
      south style=black,
      west style=black!25,#2,inside node=frame
      }\end{tcbclipframe}}},
  finish vignette/.style={%
    finish@vignette={unbroken}{#1},%
    finish@vignette={first}{#1,south size=0pt},%
    finish@vignette={middle}{#1,north size=0pt,south size=0pt},%
    finish@vignette={last}{#1,north size=0pt}%
  },
%
  finish@raised@vignette/.style 2 args={finish #1={%
    \begin{tcbclipframe}\tcbvignette{%
      draw method=clipped,
      north style={white,path fading=semi south},
      east style={black!75,path fading=semi west},
      south style={black,path fading=semi north},
      west style={black!25,path fading=semi east},#2,inside node=frame
      }\end{tcbclipframe}}},
  finish raised fading vignette/.style={%
    finish@raised@vignette={unbroken}{#1},%
    finish@raised@vignette={first}{#1,south size=0pt},%
    finish@raised@vignette={middle}{#1,north size=0pt,south size=0pt},%
    finish@raised@vignette={last}{#1,north size=0pt}%
  },
%
  finish@fading@vignette/.style 2 args={finish #1={%
    \tcbvignette{%
      draw method=clipped,fade in=tcbcol@vig@base,#2,over node=frame}}},
  finish fading vignette/.style={%
    finish@fading@vignette={unbroken}{base color=white,#1},%
    finish@fading@vignette={first}{base color=white,#1,south size=0pt},%
    finish@fading@vignette={middle}{base color=white,#1,north size=0pt,south size=0pt},%
    finish@fading@vignette={last}{base color=white,#1,north size=0pt}%
  },
%
  underlay@vignette/.style 2 args={underlay #1={%
    \begin{tcbclipframe}\tcbvignette{%
      raised color=tcbcol@frame,
      north size=\kvtcb@top@rule@stand,
      south size=\kvtcb@bottom@rule@stand,
      west size=\kvtcb@left@rule,
      east size=\kvtcb@right@rule,#2,inside node=frame
      }\end{tcbclipframe}}},
  underlay vignette/.style={%
    underlay@vignette={unbroken}{#1},%
    underlay@vignette={first}{#1,south size=0pt},%
    underlay@vignette={middle}{#1,north size=0pt,south size=0pt},%
    underlay@vignette={last}{#1,north size=0pt}%
  },
%
  underlay@fading@vignette/.style 2 args={underlay #1={%
    \begin{tcbclipframe}\tcbvignette{%
      draw method=clipped,
      north style={white,path fading=semi south},
      east style={black!75,path fading=semi west},
      south style={black,path fading=semi north},
      west style={black!25,path fading=semi east},#2,inside node=frame,
      }\end{tcbclipframe}}},
  underlay raised fading vignette/.style={%
    underlay@fading@vignette={unbroken}{#1},%
    underlay@fading@vignette={first}{#1,south size=0pt},%
    underlay@fading@vignette={middle}{#1,north size=0pt,south size=0pt},%
    underlay@fading@vignette={last}{#1,north size=0pt}%
  },
  %
  underlay raised shading vignette/.style={%
    underlay vignette={draw method=clipped,
      north style={bottom color=tcbcol@frame,top color=tcbcol@frame!33!white},
      east style={left color=tcbcol@frame,right color=tcbcol@frame!66!black},
      south style={top color=tcbcol@frame,bottom color=tcbcol@frame!33!black},
      west style={right color=tcbcol@frame,left color=tcbcol@frame!66!white},#1}},
  %
  underlay shade in vignette/.style={%
    underlay vignette={draw method=clipped,color from=tcbcol@back to tcbcol@frame,#1}},
}


==> tcbxparse.code.tex <==
%% The LaTeX package tcolorbox - version 3.94 (2016/07/14)
%% tcbxparse.code.tex: Code for xparse features
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2016 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.94}

\RequirePackage{xparse}[2013/12/31]

\tcbset{%
  IfNoValueTF/.code args={#1#2#3}{\IfNoValueTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  IfValueTF/.code args={#1#2#3}{\IfValueTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  IfBooleanTF/.code args={#1#2#3}{\IfBooleanTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  verbatim/.style={fontupper=\ttfamily,nobeforeafter,tcbox raise base,top=0pt,bottom=0pt,left=1mm,right=1mm,boxrule=0.3mm}
}

%-- tcolorbox --
\long\def\tcb@New@TColorBox#1#2#3{%
  \tcb@newenvironment{#1}{#2}{\tcolorbox[#3,options@for=#1]}{\endtcolorbox}}

\def\DeclareTColorBox{%
  \let\tcb@newenvironment\DeclareDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\NewTColorBox{%
  \let\tcb@newenvironment\NewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\RenewTColorBox{%
  \let\tcb@newenvironment\RenewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\ProvideTColorBox{%
  \let\tcb@newenvironment\ProvideDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

%-- tcolorbox (total) --
\long\def\tcb@New@TotalTColorBox#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\begin{tcolorbox}[#3,options@for=#1]#4\end{tcolorbox}}}

\def\DeclareTotalTColorBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\NewTotalTColorBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\RenewTotalTColorBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\ProvideTotalTColorBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

%-- tcbox --
\long\def\tcb@New@TCBox#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbox[#3,options@for=#1]}}

\def\DeclareTCBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\NewTCBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\RenewTCBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\ProvideTCBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

%-- tcbox (total) --
\long\def\tcb@New@TotalTCBox#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbox[#3,options@for=#1]{#4}}}

\def\DeclareTotalTCBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\NewTotalTCBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\RenewTotalTCBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\ProvideTotalTCBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\DeclareTotalTCBox{\tcboxverb}{ O{} v }{verbatim,#1}{#2}

%-- tcboxfit --
\long\def\tcb@New@TCBoxFit#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcboxfit[#3,options@for=#1]}}

\def\DeclareTCBoxFit{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\NewTCBoxFit{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\RenewTCBoxFit{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\ProvideTCBoxFit{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\long\def\tcb@New@TotalTCBoxFit#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcboxfit[#3,options@for=#1]{#4}}}

\def\DeclareTotalTCBoxFit{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\NewTotalTCBoxFit{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\RenewTotalTCBoxFit{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\ProvideTotalTCBoxFit{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}


%-- tcblisting --
\long\def\tcb@New@TCBListing#1#2#3{%
  \tcb@newenvironment{#1}{#2}{\tcblisting{#3,options@for=#1}}{\endtcblisting}}

\def\DeclareTCBListing{%
  \let\tcb@newenvironment\DeclareDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\NewTCBListing{%
  \let\tcb@newenvironment\NewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\RenewTCBListing{%
  \let\tcb@newenvironment\RenewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\ProvideTCBListing{%
  \let\tcb@newenvironment\ProvideDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

%-- tcbinputlisting --
\long\def\tcb@New@TCBInputListing#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbinputlisting{#3,options@for=#1}}%
}

\def\DeclareTCBInputListing{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\NewTCBInputListing{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\RenewTCBInputListing{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\ProvideTCBInputListing{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}


%-- sidebyside --

\def\tcb@sbs@content@none{\tcb@sbs@text@left\tcblower\tcb@sbs@text@right}
\def\tcb@sbs@content@left{\box\tcb@upperbox\tcblower\tcb@sbs@text@right}
\def\tcb@sbs@content@right{\tcb@sbs@text@left\tcblower\box\tcb@lowerbox}
\def\tcb@sbs@content@both{\box\tcb@upperbox\tcblower\box\tcb@lowerbox}

\tcbset{%
  sidebyside adapt/.is choice,
  sidebyside adapt/none/.style={%
    sidebyside@adapt@process/.style={%
      code={\let\tcb@sbs@content\tcb@sbs@content@none},
    }%
  },
  sidebyside adapt/left/.style={%
    sidebyside@adapt@process/.style={%
      code={\sbox{\tcb@upperbox}{\tcb@sbs@text@left}\let\tcb@sbs@content\tcb@sbs@content@left},
      lefthand width=\wd\tcb@upperbox,
    }%
  },
  sidebyside adapt/right/.style={%
    sidebyside@adapt@process/.style={%
      code={\sbox{\tcb@lowerbox}{\tcb@sbs@text@right}\let\tcb@sbs@content\tcb@sbs@content@right},
      righthand width=\wd\tcb@lowerbox,
    }%
  },
  sidebyside adapt/both/.style={%
    sidebyside@adapt@process/.style={%
      code={\sbox{\tcb@upperbox}{\tcb@sbs@text@left}\sbox{\tcb@lowerbox}{\tcb@sbs@text@right}\let\tcb@sbs@content\tcb@sbs@content@both},
      text width=\wd\tcb@upperbox+\kvtcb@sbs@gap+\wd\tcb@lowerbox,
      lefthand width=\wd\tcb@upperbox,
    }%
  },
  %
  sidebyside switch/.is choice,
  sidebyside switch/true/.style={%
    sidebyside@switch/.code={%
      \tcb@swap{\tcb@sbs@text@left}{\tcb@sbs@text@right}
    }%
  },
  sidebyside switch/false/.style={%
    sidebyside@switch/.style=%
  },
  sidebyside switch/.default=true
}


\DeclareTotalTColorBox{\tcbsidebyside}{ +O{} +m +m }{%
  code={\long\def\tcb@sbs@text@left{#2}\long\def\tcb@sbs@text@right{#3}},%
  #1,%
  sidebyside,%
  sidebyside@switch,sidebyside@adapt@process%
}{\tcb@sbs@content}


\tcbset{%
  reset@xparse/.style={%
    sidebyside adapt=none,sidebyside switch=false,%
  },
  initialize@reset=reset@xparse,
}

